Hardness of Approximate Diameter: Now for Undirected Graphs

Approximating the graph diameter is a basic task of both theoretical and practical interest. A simple folklore algorithm can output a 2-approximation to the diameter in linear time by running BFS from an arbitrary vertex. It has been open whether a better approximation is possible in near-linear time. A series of papers on fine-grained complexity have led to strong hardness results for diameter in directed graphs, culminating in a recent tradeoff curve independently discovered by [Li, STOC'21] and [Dalirrooyfard and Wein, STOC'21], showing that under the Strong Exponential Time Hypothesis (SETH), for any integer $k\ge 2$ and $\delta>0$, a $2-\frac{1}{k}-\delta$ approximation for diameter in directed $m$-edge graphs requires $mn^{1+1/(k-1)-o(1)}$ time. In particular, the simple linear time $2$-approximation algorithm is optimal for directed graphs. In this paper we prove that the same tradeoff lower bound curve is possible for undirected graphs as well, extending results of [Roditty and Vassilevska W., STOC'13], [Li'20] and [Bonnet, ICALP'21] who proved the first few cases of the curve, $k=2,3$ and $4$, respectively. Our result shows in particular that the simple linear time $2$-approximation algorithm is also optimal for undirected graphs. To obtain our result we develop new tools for fine-grained reductions that could be useful for proving SETH-based hardness for other problems in undirected graphs related to distance computation.

==> backup/proofsketch_old.tex <==
\section{Overview of the general $k$ reduction}
\label{sec:proofsketch}

We now sketch the ideas of the proof of Theorem~\ref{thm:main} for general $k$.

\subsection{The basic setup}
\label{ssec:proofsketch-0}
%\mina{motivation for our ideas. for example: why we can't have a coordinate change edge. why we need more than two stacks.}
%\mina{The story of how we got our ideas: (I'm just writing this to help us explain our ideas later in a better way)} 

%We now highlight some of the ideas used to extend the above Diameter reduction to general $k$.
%We point out that our proof for general $k$ is not a direct generalization of the proofs for $k=4$ and $k=5$.
%Above, for $k=4$ and $k=5$, we did not present the general construction restricted to $k=4$ and $k=5$, because the $k=4$ and $k=5$ cases had simpler constructions that still highlighted some of the ideas we used.

For our general reduction, we start with a $k$-OV instance $A\subset\{0,1\}^{\mathbb{d}}$ with size $|A|=n_{OV}$ and would like to construct a graph $G$ on $\tilde O(n_{OV}^{k-1})$ vertices and edges such that, if the set $A$ has $k$ orthogonal vectors (Yes case), the diameter of $G$ is at least $2k-1$, and otherwise (No case) the diameter of $G$ is at most $k$.
Throughout, we refer to elements of $A$ as \emph{vectors} and elements of $[\mathbb{d}]$ as \emph{coordinates}.
We may assume without loss of generality that the all ones vector $\mathbf{1}$ is in the set $A$.
We may also assume without loss of generality that no $k-1$ vectors of $A$ are orthogonal, as this can be checked in $\tilde O(n_{OV}^{k-1})$ time, and if there were then we already know we have $k$ orthogonal vectors (these assumptions help in motivating the construction).
Like in the prior constructions for $k=2,3,4$, the graph $G$ contains an ``endpoint vertex'' for each element of $A^{k-1}$, as well as some ``internal vertices'', identified by at most $k-2$ vectors in $A$, and some constant (in terms of $k$) number of \emph{coordinates} in $[\mathbb{d}]$.
Accordingly, we think each vertex of $G$ as a \emph{configuration} $H$ of vectors (in $A$) and coordinates (in $[\mathbb{d}]$).
Some configurations $H$ are \emph{valid}, meaning vectors in $H$ have 1s in specified coordinates of $H$, and there is one vertex of $G$ for each valid configuration.
Edges between vertices (configurations) of $G$ change up to one vector of a configuration and/or some of the coordinates of the configuration, and we think of edges as performing \emph{operations} on configurations.
To ensure the graph is undirected, we need to choose operations that always have an inverse operation.

\subsection{The vectors in a configuration}
\label{ssec:proofsketch-1}
The reduction graph $G$ has the property that, for any two vertices $v$ and $v'$ identified by vectors $a_1,\dots,a_s$ and $a_1',\dots,a_{s'}'$, respectively, for $s,s'\le k-1$, (and possibly some coordinates), if any subset of $k$ vectors from $a_1,\dots,a_s,a_1',\dots,a_{s'}'$ are not orthogonal (No case), then vertices $v$ and $v'$ are at distance at most $k$.
Furthermore, in the Yes case, if $a_1,\dots,a_k$ are $k$ orthogonal vectors, then the endpoint vertices $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ should be at distance $2k-1$.
Already, these requirements impose the following structure on the construction:

\paragraph{In the Yes case, a path of length at most $k-2$ from endpoint vertex $(a_1,\dots,a_{k-1})$ should not drop vector $a_1$.}
That is, after taking $k-2$ edges from the endpoint vertex $v=(a_1,\dots,a_{k-1})$, one cannot arrive at a configuration $u=(b_1,\dots,b_s, \bar x)$ of vectors $b_1,\dots,b_s$ and coordinates $\bar x$ where $a_1$ is not among vectors $b_1,\dots,b_s$.
Suppose not for contradiction, and suppose $a_1,a_2,\dots,a_k$ form the orthogonal $k$-tuple in the Yes case.
If all of the ``new'' vectors added are the all ones vector $\mathbf{1}$, then the vectors $\{b_1,\dots,b_s\}$ contain only vectors from $(a_2,\dots,a_{k-1},\mathbf{1})$.
Then among $b_1,\dots,b_s, a_k,a_{k-1},\dots,a_2,\mathbf{1}$, any $k$ vectors are orthogonal, so vertex $(b_1,\dots,b_s,\bar x)$ should be distance at most $k$ from endpoint vertex $v'=(a_k,\dots,a_2)$ by our requirement for the No case.
Hence, if $d(v,u)\le k-2$, then by the triangle inequality, we have $d(v,v')\le d(v,u)+d(u,v')\le 2k-2$, which contradicts our large diameter requirement for the Yes case.

For the same reason, a path of length at most $k-2$ from endpoint vertex $(a_k,\dots,a_2)$ should not drop vector $a_k$.
This idea leads to our next idea.

\paragraph{Using ``stacks''}
Here, stacks refer to the ``first-in-last-out'' data structure.
We identify a configuration by several ``stacks'' $S_1,\dots,S_t$, where each stack $S_i$ is simply a tuple of a nonnegative number of vectors of $A$ (the configuration may also be identified by some coordinates).
The endpoint vertices of the Diameter instance are configurations with a single stack of size $k-1$.
We think of these tuples of vectors as ``stacks'' so that operations consist of popping a vector from one stack and pushing a vector onto another stack.
In particular, an operation can only touch the ``top'' vector of any given stack.
This ensures that in the Yes case, for the endpoint vertices with stacks $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$, it takes $k-1$ operations to delete the vectors $a_1$ and $a_k$ from their respective stacks, because each operation can remove at most one vector from the top of the stack.
We point out that our constructions for $k=4$ and $k=5$ are written in this stack language.

\paragraph{More than two stacks}
For $k=4$ and $k=5$, it suffices to construct our Diameter instance with vertices that are configurations with at most two stacks, but for general $k$, more stacks seem necessary: if $k$ is large, and there were two configurations $H$ and $H'$ each with two stacks $S_1,S_2$ and $S_1',S_2'$ each of size roughly $k/2$, if one is constrained to only having two stacks, one needs around $3k/2$ vector insertion+vector deletion operations to reach configuration $S_1',S_2'$ from $S_1,S_2$, which is too much in the No case.

\paragraph{A general operation} (Definition~\ref{def:op})
For general $k$, to accommodate for more than two stacks, we define operations (edges of the Diameter instance) as follows.
Operations on configurations consist of one ``insertion'' \emph{half-operation} and one ``deletion'' half-operation.
An insertion half-operation either pushes a vector onto some stack or creates a new empty stack (along with some coordinates), and a deletion half-operation either deletes (pops) a vector from some stack or deletes an empty stack.\footnote{For technical reasons, in the final construction, we require that operations that do the insertion half-operation before the deletion half-operation, which contrasts with the $k=4$ and $k=5$ case where the deletions are done first. Roughly, this change saves a +1 in the Yes case.}\footnote{Also for technical reasons, in specific cases of the general $k$ construction, we also allow a operation to perform a ``flip'' operation between the insertion and deletion, which changes some of the ``meta-data'' of a configuration.}

Conveniently, \emph{all} edges of our generalized construction can be described by such operations.
In the $k=4$ and $k=5$ case, the edges that apply a vector insertion followed by a vector deletion cover all of the edges in the graph, except for (1) the edges from endpoint vertices with one stack to internal vertices with two stacks, and (2) the edges that change the coordinates (``coordinate change edges'').
However, for our general $k$ construction, we do not use the coordinate change edges from (2) (intuition for why is given below), this generalized definition of an operation now includes edges from (1): for example, in the $k=4$ case, the edge from $(a,b,c)\in A^3$ to $(\{(a,b),()\},x,y)\in A^2\times ([\mathbb{d}]^3)^2$ can be seen as the operation of inserting an empty stack $()$ and coordinates $x$ and $y$, and then deleting the vector $c$ from the top of the stack $(a,b,c)$.
Furthermore, these operations are invertible (e.g., a vector insertion plus stack deletion can be inverted by applying a stack insertion plus a vector deletion), so our Diameter instance is indeed undirected.


\paragraph{Size: how big are configurations?} (Definition~\ref{def:size})
We also need to specify how many vectors (and stacks) we can have in a configuration.
We note that the total number of vectors plus the total number of stacks is invariant under our defined operations: each ``insertion'' (of a vector or a stack) increases this quantity by 1, and each ``deletion'' (of a vector or a stack) decreases this quantity by 1.
Accordingly, we give this quantity a special name, calling it the \emph{size} of a configuration. 
The endpoint vertices have 1 stack and $k-1$ vectors, so the size of configurations at endpoint vertices is $k$.
Since operations preserve size, we therefore require that all configurations (vertices) in our Diameter instance have size $k$.
The size definition also has the property that, if we ignore coordinates, it is always possible to reach one size $k$ configuration from any other size $k$ configuration with $k$ operations, giving us hope that we can achieve Diameter $k$ in the No case.


%It is possible to view the above constructions for $k=4$ and $k=5$ in this stack language:
%In the reduction for $k=4$, the vertex subset $L_1$ has configurations with a single stack of three vectors, the vertex subset $L_2$ consists of configurations with two stacks, one with two vectors and one empty stack, and the subset $L_3$ consists of configurations with two stacks, each with one vector.
%The $L_1-L_2$ edges can be seen as an operation of deleting a vector and then inserting a stack, the $L_2$ to $L_3$ edges and the $L_3$ to $L_3$ vector change edges can be seen as operations of deleting and then inserting a vector.
%In the reduction for $k=5$, the vertex subset $L_1$ has configurations with a single stack of four vectors, the vertex subset $L_2$ consists of configurations with two stacks, one with three vectors and one empty stack, and the subset $L_3$ consists of configurations with two stacks, one with two vectors and one with one vector.
%Again, all of the vector change edges can be seen as an operation consisting of a vector/stack deletion followed by a vector/stack insertion. 
%For technical reasons, in the final construction, we require that operations that do the insertion half-operation before the deletion half-operation, which contrasts with the $k=4$ and $k=5$ case where the deletions could be done first.













\subsection{The coordinates in a configuration}
\label{ssec:proofsketch-2}
We have specified the structure of vectors in the configurations, namely, that we place them in first-in-last-out stacks so that the total size (number of stacks plus number of vectors in stacks) is $k$, and operations push and pop vectors from stacks and add and delete empty stacks.
Now, we need to specify the coordinates in the configurations.
In particular, we need to specify how the operations change the coordinates, and which coordinates constrain (need to be satisfied by) which stacks.

As argued above, we expect that for general $k$, our configurations need more than two stacks, and the main challenge that remains is specifying how the coordinates in configurations constrain the vectors in those stacks.
The constraints must be strong enough that in the Yes case, the 1-stack configurations $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ are not too close, but loose enough that any two configurations can reach each other in $k$ steps in the No case.
Conveniently for our construction, we only need to specify when configurations are valid vertices of our graph: we let an operation give a valid edge as long as the incident configurations are valid.
We now describe the additional ideas needed to specify the coordinates of configurations, starting with the most concrete ones.


\paragraph{Coordinate arrays}
A key abstraction that was implicit in prior constructions but that we explicitly use is something we call \emph{coordinate arrays}.
For a $k$-OV instance $A\subset\{0,1\}^{\mathbb{d}}$, a coordinate array is simply an element of $[\mathbb{d}]^{k-1}$ (Definition~\ref{def:coord-1}).
With this notion, we define what it means for a stack $S=(a_1,\dots,a_{|S|})$ to \emph{satisfy} a coordinate array $x$, which requries the vectors $a_1,\dots,a_{|S|}$ in the stacks have ones in certain coordinates of the array (Definition~\ref{def:coord-2}).
With these definitions, coordinate arrays become a useful primitive because of the following nice properties, which are helpful for achieving the balance we need between the Yes case having large diameter and the No case having small diameter.
\begin{enumerate}
\item (Lemma~\ref{lem:stack-2}, useful for the No case) Let $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$ be stacks with at most $k-1$ vectors such that any $k$ vectors from among $a_1,\dots,a_s,b_1,\dots,b_{s'}$ are orthogonal.
Then there exists a coordinate array satisfied by both $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$.
\item (Lemma~\ref{lem:yes-1}, useful for the Yes case) If $a_1,\dots,a_k$ are orthogonal, and $x$ is a coordinate array, then the stacks $(a_1,\dots,a_j)$ and $(a_k,\dots,a_{j+1})$ cannot satisfy $x$ simultaneously,
\end{enumerate}

%For $k=5$ and our simplified proof for $k=4$, we only need to consider configurations with one or two stacks of vectors from $A$, and accordingly it makes sense to have coordinate arrays that constrain the two stacks.
%We have no coordinates for one stack configurations (like in previous constructions for $k=2,3,4,5$), and for two stack configurations, we have some (two) coordinate arrays that constrain the two stacks.
At this point, we have described all of the ideas that are common to our general $k$ construction and the small case constructions for $k=4$ and $k=5$ (Section~\ref{sec:k4} and Appendix~\ref{app:k5}).
Coordinate arrays are also used as primitives in our simplified proofs for $k=4$ and $k=5$.
However, because we optimized the presentation of the $k=4$ and $k=5$ constructions for brevity and simplicity and not for generalizability, the ways the coordinate arrays constrain the stacks is slightly different from the way the coordinates constrain the stacks in the general construction.
The remaining ideas specific are to the general $k$ construction.


%As a starting point, consider the following definition of a configuration (which does not give a working Diameter construction).
%Recall that a coordinate array $x$ is an element of $[d]^{k-1}$ a stack $S$ \emph{satisfies} a coordinate array $x$ if it either left- or right-satisfies $x$, where the definition of left- and right-satisfy is given in Definition~\ref{def:satisfy}.
%A configuration $H$ consists of stacks $S_1,\dots,S_t$ and coordinate arrays $x^{i,j}$ for $1\le i\le j\le t$, such that stacks $S_i$ and $S_j$ satisfy coordinate array $x^{i,j}$.
%We can think of the configuration as a complete graph with each node labeled by a stack and each edge labeled by a coordinate array that constrains the stacks on the endpoints (note now, there are two types of graphs, the Diameter instance, and the configuration graphs).
%Each operation inserts a vector or node, and then deletes a vector or node.
%The vector insertions/deletions push or pop a vector from the top of a stack.
%Stack insertions add a node with an empty stack and edges labeled with coordinate arrays to all the other vertices, and stack deletions delete a node from the configuration graph.


%Given the constructions for $k=4$ and $k=5$, a natural place to start is to specify several coordinate arrays $x\subset[d]^{k-1}$, and require certain stacks to satisfy certain coordinate arrays.
%\textbf{Idea 3: Make coordinate changes costly}
%
%In a configuration with vectors in $A$ and coordinates in $[d]$, the coordinates need to constrain the vectors enough that the 


\paragraph{No case: Coordinate arrays constrain at most two stacks.} (See Definition~\ref{def:edge} and Table~\ref{tab:edgesatisfying})
The next two ideas may or may not be necessary but are at least convenient.
In the No case, for any two configurations $H$ and $H'$, we need to construct a path $H_0=H,H_1,\dots,H_k=H'$ from $H$ to $H'$, such that configuration $H_i$ is obtained by applying some operation to $H_{i-1}$ for all $i=1,\dots,k$.
Since configurations $H$ and $H'$ have size $k$, in each of the $k$ operations on the path, the insertion operation must add a vector or stack ``belonging to'' $H'$ and the deletion operation must delete a vector or stack ``belonging to'' $H$ (the notion that some configurations ``share'' stacks can be formalized by assigning labels to stacks, see Definition~\ref{def:configuration}).
Hence, each intermediate configuration $H_i$ contains some stacks and coordinate arrays ``belonging to'' $H$, some stacks and coordinate arrays ``belonging to'' $H'$, and possibly some additional coordinate arrays. 
However, it is possible that none of the vectors in $H$ have ones in any of the coordinates in $H'$, and vise versa.
Thus, it is important that for each $H_i$, none of the coordinate arrays ``belonging to'' $H$ constrain any of the stacks ``belonging to'' $H'$, and vise versa.
This is easiest to guarantee if at most two stacks are ever required to satisfy any coordinate array, and we found this assumption not make the Yes case much harder.
By similar reasoning, we also have the following idea.

\paragraph{No case: Require every configuration has a stack with at least $\ceil{(k-2)/2}$ vectors.} (Definition~\ref{def:valid})
Without this constraint, there could be two size-$k$ configurations $H$ and $H'$ with $\Omega(k)$ stacks of $O(1)$ vectors each such that none of the coordinate arrays from $H$ are satisfied by stacks in $H'$ and vise versa.
In the No case, these two configurations $H$ and $H'$ must be connected by a length $k$ path $H_0=H,H_1,\dots,H_k=H'$.
Then, the intermediate configuration $H_{k/2}$ must have $\Omega(k)$ stacks from $H$ and also $\Omega(k)$ stacks from $H'$.
It is easily possible that configuration $H_{k/2}$ has at least one coordinate array for every pair of stacks (in fact, below we show that having only one coordinate array for each pair of stacks is not enough for the Yes case), so we likely have $\Omega(k^2)$ coordinate arrays in $H_{k/2}$ that belong to neither $H$ or $H'$ but constrain some stack in $H$ and another stack in $H'$.
All $\Omega(k^2)$ must be all inserted and then deleted on the path from $H$ to $H'$, giving a lot of ``extra'' coordinate arrays to keep track of.

Requiring that every configuration has a stack with at least $\ceil{(k-2)/2}$ vectors means that, in the No case, we can find a path $H_0=H,H_1,\dots,H_k=H'$ between two configurations $H$ and $H'$, such that in each intermediate configuration $H_i$, there is either only \emph{one} stack from $H$ or only \emph{one} stack from $H'$, giving only $O(k)$ ``extra'' coordinate arrays to keep track of, an improvement from $\Omega(k^2)$ such coordinate arrays.
Furthermore, this requirement does not seem to affect the Yes case, and our Yes case proof does not seem to use this assumption.








\paragraph{Yes case: No coordinate change edge.}
In the $k=4$ and $k=5$ constructions in this work, at every vertex, there is an edge that changes \emph{all} the coordinates of an edge, e.g., from $(a,b,x,y)_{L_2}\in A^2\times ([\mathbb{d}]^3)^2$ to $(a,b,x',y')_{L_2}$ in the case of $k=4$.
However, these ``coordinate-change edges'' cannot exist in the general construction.
Indeed, if such edges existed, then in the Yes case, configurations $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ would be at distance only $3k/2+O(1)$.
From $(a_1,\dots,a_{k-1})$, we could (i) reach a configuration with stacks $(a_1,\dots,a_{k/2-O(1)}), (\mathbf{1},\dots,\mathbf{1})$ in roughly $k/2$ operations, (ii) apply a coordinate change edge, (iii) reach a configuration with stacks $(a_k,\dots,a_{k/2+O(1)}),(\mathbf{1},\dots,\mathbf{1})$ in roughly $k/2$ operations, (iv) apply a coordinate change edge, and (v) reach configuration $(a_k,\dots,a_{2})$ in roughly $k/2$ operations.
Indeed, the coordinate change edges divide the path into three subpaths, and in each subpath we never ``see'' all of the vectors $a_1,\dots,a_k$ in the stacks, so we can choose the coordinate arrays so that the stacks always satisfy the coordinate arrays, hence giving a valid path (we assumed without loss of generality that no $k-1$ vectors are orthogonal).
Thus, for the Yes case, changing coordinates needs to be more expensive that one edge.



\paragraph{Yes case: Remembering coordinate arrays (a.k.a. coordinate arrays constraining phantom stacks)} (See comments after Definition~\ref{def:edge})
One natural (but incorrect) way of implementing the above ideas is, in a configuration with stacks $S_1,\dots,S_t$, have $\binom{t}{2}$ coordinate arrays, $x^{i,j}$ for $1\le i<j\le t$, and require that stacks $S_i$ and $S_j$ satisfy coordinate array $x^{i,j}$.
Adding an empty stack $S_{t+1}$ to a configuration with $t$ stacks adds $t$ coordinate arrays $x^{i,t+1}$, one for each pair of stacks $(S_i,S_{t+1})$, and deleting a stack $S_{t}$ deletes the $t-1$ coordinate arrays that constrain it.
This construction does not work, because in the Yes case, as in the previous paragraph, it is again possible for the 1-stack configuration $(a_1,\dots,a_{k-1})$ to reach the 1-stack configuration $(a_k,\dots,a_2)$ in $3k/2+O(1)$ steps, by passing through the two stack configurations with stacks $(a_1,\dots,a_{k/2-O(1)}), (\mathbf{1},\dots,\mathbf{1})$ and $(a_k,\dots,a_{k/2+O(1)}),(\mathbf{1},\dots,\mathbf{1})$.

%With the same counterexample in the Yes case, we also rule out the following simpler construction:
%The Diameter instance again has a vertex for every ``configuration'' of vectors and coordinates, and edges of the Diameter instance correspond to operations on configurations.
%In a configuration, 
%\begin{itemize}
%\item A configuration $H$ consists of stacks $S_1,\dots,S_t$ and coordinate arrays $x^{i,j}$ for $1\le i\le j\le t$, such that stacks $S_i$ and $S_j$ satisfy coordinate array $x^{i,j}$. We can think of the configuration as a complete graph with each node labeled by a stack and each edge labeled by a coordinate array that constrains the stacks on the endpoints (note now, there are two types of graphs, the Diameter instance, and the configuration graphs).
%\item Each operation inserts a vector or node, and then deletes a vector or node.
%The vector insertions/deletions push or pop a vector from the top of a stack.
%Stack insertions add a node with an empty stack and edges labeled with coordinate arrays to all the other vertices, and stack deletions delete a node from the configuration graph.
%\end{itemize}
%Indeed, let $S=(a_1,\dots,a_{(k-2)/2}), S'=(a_{k},\dots,a_{(k+4)/2})$ be stacks of length $\floor{(k-2)/2}$, and let $\vec{\mathbf{1}} = (\mathbf{1},\dots,\mathbf{1})$ be a stack of length $\ceil{(k-2)/2}$.
%Then the configuration $H$ with stacks $S$ and $\vec{\mathbf{1}}$ can reach the configuration $H'$ with stacks $S'$ and $\vec{\mathbf{1}}$, by creating a new node, and using the fact that any $k-1$ vectors are orthogonal. \TODO{picture}
%($S\xleftrightarrow{X}\mathbf{1}$, $S'\xleftrightarrow{Y}\mathbf{1}$, and $S\xleftrightarrow{Z}\mathbf{1}$)

%The above attempt is a natural attempt when each coordinate array constrains a pair of stacks.
To work around this problem we have configurations $H$ ``remember'' some coordinate arrays that constrain deleted stacks.
That is, if an operation on configuration $H$ deletes a stack $S$ to obtain configuration $H'$, some of the coordinate arrays of $H$ that $S$ needed to satisfy are still coordinate arrays of configuration $H'$.
In this way, some coordinate arrays of a configuration constrain two stacks and other coordinate arrays only constrain one stack (such coordinate arrays can be thought of as constraining a real stack and a ``phantom'' stack).
This works, but one needs to be careful in how many coordinate arrays are ``remembered'', or else the No case might have large diameter.

\paragraph{Balancing the No case and Yes case: a tree and an ordering $\prec_H$ on the stacks.} (Definition~\ref{def:configuration})
The Yes case, particularly the $3k/2+O(1)$-path counterexample, encourages us to remember more constraints, but having Diameter $k$ in the No case keeps us from remembering too many constraints.
In the final construction, to help with this balance, we add two additional structures to configurations: 
\begin{enumerate}
\item Put an ordering $\prec_H$ on the stacks of a configuration $H$, so that we have a list of stacks, rather than simply a set of stacks.
Whether a stack is constrained by a certain coordinate array then depends on the location of the stack in the ordering. 

\item We place the stacks $S_1,\dots,S_t$ of a configuration $H$ at the vertices of a tree on $t$ vertices (in particular, a star graph on $t$ vertices). Coordinate arrays are attached to the edges of the tree so that a coordinate array is added to (deleted from) the configuration exactly when the corresponding edge is added to (deleted from) the configuration.
For clarity, we emphasize that there are now two types of graphs: the tree graphs $H$ that define a configuration, and the Diameter instance $G$, whose vertices are configurations $H$.

With this tree, we remember some, but not too many, coordinate arrays that constrained deleted vertices (Lemma~\ref{lem:yes-3}).
In particular, for an edge connecting stacks $S_i$ and $S_j$, we keep track of the coordinate arrays that constrain $S_i$ and some other (possibly non-existent) stack, and also the coordinate arrays that constrain $S_j$ and some other (possibly non-existent) stack.
Somewhat subtly, the coordinate arrays attached to an edge may constrain stacks not incident to the edge.
For the coordinate arrays constraining $S_i$, whether the coordinate arrays constrain another real stack or a non-existent stack depends on the ordering $\prec_H$.
\end{enumerate}


%In the cases $k=4$ and $k=5$, it is useful
%Consider, the Yes case when, for example, $k=100$.









%Can start with $k=6$, illustrate the ST construction, say that we just need half of the layers cause we are in the undirected case: layers would be $L_1:(a_1,\ldots,a_5)$, $L_2:(a_1,\ldots,a_4,X)$, $L_3:(a_1,a_2,a_3,b_1,X)$, $L_4:(a_1,a_2,b_1,b_2)$. First we can treat $L_1$ as one stack and the other layers as having two stacks: $a$s and $b$s. Then we can say how a path from $(a_1,\ldots,a_5)$ to $(b_1,\ldots,b_5)$ looks like: we define a new stack, then we empty the first stack and add to the second stack one by one. Now if we want to go from $L_1:(a_1,\ldots,a_5)$ to $L_4:(a_1',a_2',b_1,b_2,Y)$, we can go to $(a_1,a_2,b_1,b_2,X)$, then need to be able to change $a_1$ and $a_2$, i.e. change the $a$ stack in $L_4$. Our first idea comes here. We basically can treat changing this stack as a $k=3$ instance. So in order to change it, we create an empty stack, and change the vectors one by one. We also need to change the coordinate array $Y$ to $X$. If we just put a coordinate array change edge inside $L_4$, that can be problematic in the yes case (say why) so we need to change $Y$ "gradually". That's why when adding the third stack, we keep $X$, but we also introduce the $Y$ stack, and we define certain constraint among the stacks and the coordinate arrays. 

%
%\ryl{Another thing we can say: for the No case, from configuration $H$ to configuration $H'$, we need to ``forget'' all the constraints of configuration $H$ and ``add'' all the constraints of configuration $H'$. 
%We found this easiest to guarantee by assuming some stack in each configuration has at least $\floor{(k-2)/2}$ nodes, so that in the middle of the path, we can be dealing with only two stacks.
%The ordering $\prec_H$ is used because it is possible that none of the stacks in $H$ satisfy any of the coordinate arrays in any of the edge-constraints in $H'$, so the path in the No case can never have a stack in $H$ constrained by an ``added'' coordinate array of $H'$, and similarlyl any ``added'' stack of $H'$ can never be constrained by one of hte original coordinate arrays of $H$.}




==> backup/simplified_old.tex <==
\section{The main theorem for general $k$}
\label{sec:all}


%\ryl{Cleaned up this section a bit, added some more structure (paragraph headings) to the configuration definition, added some English in between the definitions and added some references to the proof overview}
We describe below a reduction from $k$-OV to $2k-1$ vs. $k$ Diameter with time $O(n^{k/(k-1)})$ on graphs with edges of weight 1 or 0.
This immediately gives a reduction from $k$-OV to $2k-1$ vs. $k$ Diameter with time $O(n^{k/(k-1)})$ on unweighted graphs, by contracting the edges of weight 0.
For clarity of exposition, we describe the reduction to the 0/1-weighted graph.


Throughout the construction, fix $k'=\floor{k/2}+1$.
Throughout the construction, all coordinate arrays are $k$-coordinate arrays.
Let $\Phi$ be a $k$-OV instance given by a set $A$ of $n$ vectors of length $O(\log{n})$. We create a graph $G$ using this instance.
First we need a few definitions.


\subsection{Configurations}


\paragraph{Edge constraints.}
The vertices of our construction are ``configurations" which we are going to define formally later. 
Each configuration is a small graph, in which each vertex is assigned a stack and each edge puts constraints between those stacks. 
These \emph{edge-constraints} on edges are of the following form.
Recall that a coordinate array is an element of $[\mathbb{d}]^{k-1}$. 
\begin{definition}[Edge-constraint]
In a graph with an edge connecting vertices $v$ and $v'$, a \emph{$(v,v')$-edge-constraint $X$} (or \emph{edge-constraint} when $(v,v')$ is implicit) is a tuple of $2k'+1$ coordinate-arrays: $X_{v,i}$ and $X_{v',i}$ for $i\in[k']$, and $X_{*}$.
\end{definition}
We later define how these $2k'+1$ coordinate arrays of a $(v,v')$-edge-constraint relate with the stacks assigned to $v$ and $v'$, as well as the stacks of other vertices. 



\paragraph{Configurations.}
With these edge-constraints defined, we can now define a configuration.
\begin{definition}[Configuration]
  A \emph{configuration} $H$ is an undirected star\footnote{Recall a star graph is a tree with a \emph{center} vertex adjacent to all other vertices. We expect that a similar construction works even if the configurations are constrained to be trees, and not specifically stars. However, we restrict configurations to be star graphs to simplify the presentation.} graph $H$ with nodes $V(H)$ labeled by distinct elements of $[2k']$, such that 
  \begin{enumerate}
  \item The center node, denoted $\rho(H)$, of the star graph $H$ is called the \emph{root} (if the graph has two nodes, either one could be the root),
  \item $H$ is equipped with a total order $\prec_H$ on the vertices of $H$ such that the root is the smallest node of $\prec_H$,
  \item Each node $v$ of $H$ is assigned a stack $S_v(H)$, and
  \item Each edge $(v,v')$ of $H$ is labeled with an $(v,v')$-edge constraint $X^{v,v'}$. As graph $H$ is undirected, we equivalently denote $X^{v,v'}$ by $X^{v',v}$.
  \end{enumerate}
  \label{def:configuration}
\end{definition}
Again, we emphasize that there are now two types of graphs, the configuration graph, and the Diameter instance, whose vertices are identified by configuration graphs.
We say configuration $H$ is a \emph{$t$-stack} configuration if $H$ has $t$ vertices. %\mina{I don't think we use $t$-stack anywhere}\ryl{it's used a few times}
The vertices of our Diameter instance are identified with configurations. 
We use the following definition to specify how many nodes and vectors are in these configuration (Section~\ref{ssec:proofsketch-1} motivates this definition).
As we specify later, the vertices of our Diameter instance are identified by configurations of size $k$.
\begin{definition}[Size of a configuration]
  The \emph{size} of a configuration $H$ is the integer $\sum_{v\in V(H)}^{} (1+|S_v(H)|)$; i.e. the number of stacks plus the total number of vectors in all the stacks. 
  \label{def:size}
\end{definition}


\paragraph{Equivalent configurations.}
The node labels of a configuration $H$ in $[2k']$ are irrelevant except so that we can reason about operations on configurations (defined later) in a well defined way.
Accordingly, we say two configurations are \emph{equivalent} if, informally, one can be obtained by permuting the node labels of the other.
Formally, we have the following definition.
\begin{definition}[Equivalence of configurations]
\label{def:equiv}
We say two configurations $H$ and $H'$ are \emph{equivalent} if there is some permutation $\pi:[2k']\to [2k']$ such that, 
\begin{itemize}
\item Configuration $H'$ contains node $\pi(v)$ for each node $v$ of $H$, and an edge $(\pi(v),\pi(v'))$ with $(\pi(v),\pi(v'))$-edge constraint $Y^{\pi(v),\pi(v')}$ for each edge $(v,v')$ of $H$ with $(v,v')$-edge-constraint $X^{v,v'}$, such that $Y^{\pi(v),\pi(v')}_{\pi(v),j}=X^{v,v'}_{v,j}$ and $Y^{\pi(v),\pi(v')}_{\pi(v'),j}=X^{v,v'}_{v',j}$ for all $j\in[k']$, and $Y^{\pi(v),\pi(v')}_* = X^{v,v'}_*$.
\item The stacks satisfy $S_{\pi(v)}(\pi(H))=S_v(H)$ for every node $v$ of $H$.
\item The ordering $\prec_{H'}$ on $H'$  has $\pi(v)\prec_{H'} \pi(v')$ if and only if $v\prec_{H'} v'$.
\item The root $\rho(\pi(H))$ of $\pi(H)$ satisfies $\rho(\pi(H))=\pi(\rho(H))$.
%$v$ is the root of $H$, then $\pi(v)$ is the root of $H'$.
\end{itemize}
In this case, we write $H'=\pi(H)$.
\end{definition}
It is easy to check the following fact from Definition~\ref{def:equiv}.
\begin{lemma}
  For two permutations $\pi$ and $\pi'$, we have $\pi(\pi'(H)) = (\pi\circ\pi')(H)$, so taking $\pi'=\pi^{-1}$ verifies that the equivalence in Definition~\ref{def:equiv} is indeed an equivalence relation.
\label{lem:perm-0}
\end{lemma}


\paragraph{Edge-satisfying and valid configurations.}
For a configuration to be a valid vertex of our diameter instance, the stacks of a configuration need to satisfy particular coordinate arrays in the configuration. 
We now make precise how we want the coordinate arrays to constrain the stacks.
This is the most technical definition in the construction.
\begin{definition}[Edge-satisfying and $\mathcal{X}_v(H)$]
  \label{def:edge}
  A configuration $H$ with $s\ge 1$ vertices $v_1\prec_H\cdots\prec_H v_s$ is \emph{edge-satisfying} if and only if for every $i\in[s]$, the stack $S_{v_i}(H)$ satisfies each coordinate array in the following set $\mathcal{X}_{v_i}(H)$ of coordinate arrays.
  \begin{enumerate}
  \item For every neighbor $v'$ of $v_i$, and every index $j\in[k']$, set $\mathcal{X}_{v_i}(H)$ includes the coordinate array $X^{v_i,v'}_{v_i,j}$ and $X^{v_i,v'}_*$. Note that either $v'$ or $v_i$ is the root.
  \item For every $i' > i$, set $\mathcal{X}_{v_i}(H)$ includes the coordinate array $X^{v_{i'},v_1}_{v_{i'},i}$, where recall that $v_1$ is the root $\rho(H)$. See Figure \ref{fig:edgesatisfying}. %\vvw{Btw, we might want to say something about this bullet here since the $i$th stack now needs to satisfy coordinates that are not on edges incident to $v_i$; this can be confusing.}
  \end{enumerate}
 %\mina{todo: a figure/table }
 %\mina{another possible wording of this (for my understanding/can be used for clarification/figures,etc): to see which stacks satisfy which parts of $X^{v_1,v_i}$: fix $j$. only $v_1$ satisfies $X^{v_1,v_i}_{v_1,j}$. for $X^{v_1,v_i}_{v_i,j}$, $v_i$ satisfies it and if $j<i$, $v_j$ satisfies it as well.}
% \ryl{Yeah, I originally wrote it that way. The current wording, where you list the coordinates that $S_{v_i}$ needs to satisfy, makes Lemma~\ref{lem:op-4} and Lemma~\ref{lem:no-4} easier to write, since it's easier to make statements like ``we already know stack $S_v(H')$ satisfies some coordinate arrays because some other configuration is valid, so there's only a few coordinate arrays we need to check''}\vvw{How about we add Mina's wording as intuition?}
\end{definition}

\begin{figure}
    \centering
    \includegraphics{edgesatisfying.pdf}
    \caption{The coordinate arrays $\mathcal{X}_{v_i}(H)$ that stack $S_{v_i}(H)$ satisfies, for $i\ge 2$. The relevant edges are colored red, and the coordinate array that is satisfied by $S_{v_i}(H)$ is written on them. the edge $v_1v_i$ is shown in bold since many coordinate arrays on this edge-constraint are satisfied by $S_{v_i}(H)$.
    }
    \label{fig:edgesatisfying}
\end{figure}

We highlight the subtle detail that the edge constraint $X^{v_1,v_i}$ belonging to the edge $v_1v_i$ where $v_1=\rho(H)$ might hold coordinate arrays constraining the stacks of the nodes other than its endpoints $v_1$ and $v_i$. %\ryl{Updated this sentence}
To get more intuition, the coordinate arrays a given stack $S_{v_i}$ needs to satisfy are illustrated in Figure~\ref{fig:edgesatisfying}, and for an edge $v_1v_i$ in configuration $H$ the stacks that must satisfy each coordinate array in $X^{v_1,v_i}$ are illustrated in Table~\ref{tab:edgesatisfying}. 
As we motivated in the overview (Section~\ref{ssec:proofsketch-2}), Table~\ref{tab:edgesatisfying} shows that every coordinate array in the edge-constraint $X$ constrains at most two stacks.
Furthermore, some coordinate arrays only constrain one stack, corresponding to coordinate arrays that need to be ``remembered'' for the Yes case (Section~\ref{ssec:proofsketch-2}).

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
         & $*$& 1&$\ldots$ &$j$ & $\ldots$ & $i-1$ & $i$ & $\ldots$ & $k'$ \\ \hline
         $*$& $S_{v_1},S_{v_i}$&$-$ &$\ldots$ & $-$ & $\ldots$ & $-$ & $-$ & $\ldots$ & $-$ \\ \hline
         $v_1$ & $-$& $S_{v_1}$&$\ldots$& $S_{v_1}$ & $\ldots$ & $S_{v_1}$ & $S_{v_1}$ &$\ldots$& $S_{v_1}$ \\ \hline
         $v_i$ & $-$&$S_{v_1},S_{v_i}$ &$\ldots$ &$S_{v_j},S_{v_i}$ & $\ldots$ & $S_{v_{i-1}},S_{v_i}$ & $S_{v_i}$ &$\ldots$& $S_{v_i}$ \\ \hline
    \end{tabular}
    \caption{Edge satisfying constraints for $X^{v_1,v_i}$ in a configuration $H$. The entry in row $u$ and column $t$ represent the stacks satisfying $X^{v_1,v_i}_{u,t}$. The entry in row $*$ and column $*$ represent the stacks satisfying $X^{v_1,v_i}_*$. We drop $H$ in $S_{u}(H)$ for space constraints.}
    \label{tab:edgesatisfying}
\end{table}

\begin{definition}[Valid configuration]
\label{def:valid}
  The configuration $H$ is \emph{valid} if it is edge-satisfying and the stack of the root node  satisfies $|S_{\rho(H)}(H)|\ge (k-2)/2$. Here, $k$ is the parameter of our reduction. We use this definition even when the size of configuration $H$ is not $k$. 
  %\ryl{$k$ is overloaded.} %\mina{todo: check if this condition is fine with flip edges}\ryl{I think this is okay, because the flip is the middle operation of a full operation. We only need it in the ``middle'' of the No case, so the operation is always insert, flip, delete.}
\end{definition}
%\TODO{Some examples of configurations.
%Example of a configuration, a the half operations, and flips
%}

%\vvw{What do you mean by "by definition" below. I didn't see anywhere that the sum of stack sizes in a configuration should be $\ceil{(k-2)/2}$. This doesn't appear until the definition of valid configuration below.}\ryl{Sorry this paragraph was in the wrong place}
The requirement that the root node stack has size $(k-2)/2$ is motivated in Section~\ref{ssec:proofsketch-2}.
The choice of our global constant $k'$ is motivated by this definition: Since all valid configurations have a stack with at least $(k-2)/2$ vectors, all valid size-$k$ configurations, and hence all configurations at vertices of our Diameter instance, have at most $k-\ceil{(k-2)/2} = k'$ nodes. Now we relate edge-constraints with the nodes of a configuration.

\paragraph{Operations on configurations.}
As mentioned earlier, our final construction consists of configurations. To relate different configurations to each other, we define operations as follows.

%\vvw{I suggest that we have a special variable for the root, e.g. $\rho(H)$.}\ryl{Good idea}

\begin{definition}[Operations on configurations]
  We define the following \emph{half-operations} on configurations $H$, that produce a resulting configuration $H'$.
  \begin{enumerate}
  \item \textbf{Vector insertion}. $H'$ has the same nodes, root node, edges, stacks, and ordering as $H$, except that $S_v(H') = S_v(H) + b$ for some vector $b\in A$ and some node $v$.
  \item \textbf{Vector deletion}. $H'$ has the same nodes, root node, edges, stacks, and ordering as $H$, except that $S_v(H') = popped(S_v(H))$ for some node $v$.
  \item \textbf{Node insertion}. $H'$ has the same nodes, root node, edges, stacks as $H$, except that $H'$ also contains a node $v$ labeled in $[2k']\setminus V(H)$, assigned with an empty stack $S_v(H')=\emptyset$, and an edge from node $v$ to the root node $\rho(H')=\rho(H)$ with a $(v,\rho(H'))$-edge constraint $X$, and such that the total order $\prec_{H'}$ is a total order consistent with $\prec_H$ on the nodes of $H$ and the new node $v$ as either the largest or second largest node of $\prec_H$.\footnote{This requirement that the new node $v$ is either the largest or second largest node of $\prec_H$ is not necessary, but makes the rest of the proof, especially Lemma~\ref{lem:op-4}, easier to write. Similarly, for node deletions, the deleted node does not need to be the largest or second-largest node of $\prec_H$.}
  \item \textbf{Node deletion}. $H'$ has the same nodes, root node, edges, stacks as $H$, except that for some non-root (leaf) node $v$ with $S_v(H)=\emptyset$ that is either the second-largest or largest node of $\prec_H$, $H'$ does not contain node $v$ or the edge incident to it, and the order $\prec_{H'}$ is the order $\prec_H$ restricted to the nodes of $H'$
  \item \textbf{Flip}. This half-operation is ``only" defined when $H$ has \emph{exactly two} nodes $v$ and $v'$ with $v=\rho(H)$ as the root and $|S_v(H)|=|S_{v'}(H)|$. Then $H'$ has the same nodes, edges, and stacks as $H$, but $v'=\rho(H')$ is the root of $H'$ and the ordering $\prec_{H'}$ of the nodes of $H'$ is switched accordingly, so that $v'\prec_{H'} v$.
  \end{enumerate}
  Call such a half-operation \emph{valid} if configurations $H$ and $H'$ are both valid.  %\mina{but in flip one of them is not going to be valid. Maybe we just need the two endpoints of a "full operation" be valid (probably the easiest fix)? or maybe we need to relax the validity definition for root to be for when we have at least 3 nodes?}
 % \ryl{In this construction, the flips only occur when the stacks are roughly the same size (so e.g., if the stacks are size $k-2$ and $0$, you can't use the flip edge).
  %I realized it is easier to write this way.
 
  %Also, we actually need that the full operation is valid iff both half operations are valid, because otherwise we only get diameter $2k-2$ in the Yes case. In particular, in the yes case, when we go from $H_i\to H_{i+0.5}\to H_{i+1}$, we sometimes use that $H_{i+0.5}$ is valid.}
    
  A \emph{full operation} is obtained by applying a vector or node insertion, possibly applying a flip (if applicable), and then applying a vector or node deletion.
  We say a full operation from $H$ to $H'$ is \emph{valid} if each of the two (or three, if there is a flip) participating half-operations is valid, and if at least one of $H$ or $H'$ has at least two nodes.
  \label{def:op}
\end{definition}

%Note that a half operation might create a configuration $H'$ of size $k+1$, but this configuration is valid because it has $(k-2)/2$ vectors in the stack $S_{\rho(H')}$. \ryl{Was this added? I deleted it}
By combining a ``delete" (node or vector) half operation to an insert (node or vector) half operation, we make sure that the endpoints of a full-operation have the same size. For examples of full operations, see Figure \ref{fig:conf-ex1} and Figure \ref{fig:conf-ex2}. Full operations have the following useful properties.

\begin{figure}
    \centering
    \includegraphics{conf-ex1.pdf}
    \caption{Example of a full operation consisting of a node insertion ($v_4$) and a vector deletion (from $v_2$). We assume that $k=7$ in this example. The root in all three configurations is colored purple.}
    \label{fig:conf-ex1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{conf-ex2.pdf}
    \caption{Example of a full operation consisting of a vector insertion (in $ v_2$), a flip and a vector deletion (from $v_1$). We assume that $k=7$ in this example. Note that when the flip operation happens, the two nodes have the same number of vectors in their stacks. The root in all four configurations is colored purple.}
    \label{fig:conf-ex2}
\end{figure}


\begin{lemma}[Properties of half and full operations]
  Let $H$ and $H'$ be configurations.
  \begin{itemize}
  \item If applying a vector insertion to $H$ gives $H'$, it is possible to apply a vector deletion to $H'$ to get $H$.
  \item If applying a vector deletion to $H$ gives $H'$, it is possible to apply a vector insertion to $H'$ to get $H$.
  \item If applying a node insertion to $H$ gives $H'$, it is possible to apply node deletion to $H'$ to get $H$.
  \item If applying a node deletion to $H$ gives $H'$, it is possible to apply node insertion to $H'$ to get $H$.
  \item Applying two flip operations to a 2-stack configuration gives the same configuration.
  \item If applying a valid full operation to $H$ gives $H'$, it is possible to apply a valid full operation to $H'$ to get $H$. 
  \end{itemize}
  \label{lem:op-1}
\end{lemma}
\begin{proof}
  For the first item, if $H'$ is obtained from a vector insertion at node $v$ in $H$, then $H$ is obtained by a vector deletion at node $v$ in $H$.
  The second, third, and fourth items are similar.
  For the fifth item, flip operations do not change the 2-node graph, and two flips preserve the root node and the ordering of the two nodes.

  For the sixth item, note that the first five items imply that every half-operation has an inverse.
  If $H'$ is obtained by applying two half-operations to $H$ that give $H''$ then $H'$, and both half operations are valid, then configurations $H,H'',H'$ are all valid configurations. 
  Then the full operation $H'\to H''\to H$ is a valid full operation.
  Similarly if $H'$ is obtained with a valid full operation including a flip, having intermediate configurations $H\to H''\to H'''\to H'$, then all the intermediate configurations are valid, and $H'\to H'''\to H''\to H$ is a valid full operation.
\end{proof}


\subsection{Defining the Diameter graph $G$}
We are now ready to define our graph $G$.
The vertex set of $G$ is the set of valid size-$k$ configurations. Recall that for all size-$k$ configurations, the number of stacks plus the total number of vectors in all stacks is $k$, and a configuration is valid if it is edge-satisfying (Definition~\ref{def:edge}) and the root stack has at least $(k-2)/2$ vectors in it. 
The edge-set of $G$ includes the following types of edges:
\begin{itemize}
\item edges $(H,H')$ such that configuration $H$ can be obtained from configuration $H'$ by a valid full operation. 
We call these edges \emph{operation edges}.
By the last part of Lemma~\ref{lem:op-1}, $(H,H')$ are connected by an operation edge \emph{if and only if} $H$ can be obtained from $H'$ by a valid full operation, so these edges can indeed by undirected.

\item weight-0 edges $(H,\pi(H))$ for all valid size-$k$ configurations $H$ and all permutations $\pi:[2k']\to [2k']$ (recall $\pi(H)$ is defined in Definition~\ref{def:equiv}).
We call these edges \emph{permutation edges}.

\item (if $k$ is even) weight-0 edges $(H,H')$ if $H'$ can be obtained by applying a flip to $H$. 
We call these edges \emph{flip edges}.
\end{itemize}
For disambiguation, we always refer to vertices of configurations as \emph{nodes}, and vertices of the Diameter instance $G$ as \emph{vertices} or \emph{configurations}.





\paragraph{Runtime analysis.}
We first show that the graph $G$ can be constructed in time $O_k(n_{OV}^{k-1}\mathbb{d}^{O(k^2)})$.
One can construct the vertices of $G$ by enumerating over all possible star graphs labeled by $[2k']$, of which there are at most $O_k(1)$, and then enumerating over all possible orderings $\prec$ of the nodes of star graphs, of which there are at most $O_k(1)$, and then enumerating over all possible stacks for each star graph, of which there are at most $O_k(n_{OV}^{k-1})$ (each configuration is size-$k$, meaning the total number of nodes (stacks) plus the total number of vectors equals $k$, and since there is always at least one node (stack), the total number of vectors is at most $k-1$), and enumerating over all possible edge-constraints, of which there are at most $O_k(\mathbb{d}^{(k'-1)\cdot (2k'+1)}) \le O_k(\mathbb{d}^{2k^2})$.
Hence, there are at most $O_k(n_{OV}^{k-1}\mathbb{d}^{2k^2})$ vertices of $G$.
Furthermore, for $t\ge 2$, there are at most $O_k(n_{OV}^{k-2}\mathbb{d}^{2k^2})$ many $t$-stack configurations of $G$.

For any configuration, there are $O_k(n_{OV})$ vector insertions possible, $O_k(1)$ vector deletions possible, $O_k(\mathbb{d}^{2k'+1})$ node insertions possible, and $O_k(1)$ node deletions possible.
Hence, each configuration of $G$ has at most $O_k(n_{OV}+\mathbb{d}^{2k'+1})$ neighbors.
Every edge of $G$ has at least one endpoint that has $t\ge 2$ stacks (by definition of valid full operation), so the total number of edges of $G$ is at most $O_k(n_{OV}+\mathbb{d}^{2k'+1})\cdot O_k(n_{OV}^{k-2}\mathbb{d}^{2k^2})\le O_k(n_{OV}^{k-1}\mathbb{d}^{4k^2})$.

Hence, $G$ has $\tilde O(n_{OV}^{k-1})$ vertices (configurations) and edges.
Checking whether any half-operation is valid takes time $O_k(\mathbb{d}) = \tilde O_k(1)$. 
Hence enumeration of vertices (configurations) and edges of the Diameter graph $G$ is standard and can be done in time near-linear in the number of vertices and edges, so the construction of $G$ takes time $\tilde O(n_{OV}^{k-1})$.


\subsection{Some useful properties of configurations}

We now move on to proving the correctness of our configurations, showing that the Diameter is at least $2k-1$ when the $k$-OV instance $\Phi$ has a solution (Yes case), and the Diameter is at most $k$ when $\Phi$ has no solution (No case).
We begin with some useful lemmas about configurations.
%\ryl{Added some preamble}

\paragraph{Lemma for the No case.}
In the No case, we need to construct length $k$ paths between every pair of nodes and verify that those paths are valid paths in the Diameter instance.
The following natural lemma facilitates these verifications.
Call $H'$ a  \emph{subconfiguration} of $H$ if $H'$ can be obtained from $H$ by vector deletions and node deletions.
\begin{lemma}
  If $H'$ is a subconfiguration of $H$ and $H$ is edge-satisfying, then $H'$ is also edge-satisfying.
  \label{lem:op-4}
\end{lemma}
\begin{proof}
  It suffices to prove that if $H'$ is obtained by applying a single vector deletion or node deletion to $H$, and $H$ is valid, then $H'$ is valid.
  The full lemma follows from induction of the number of deletions needed to obtain $H'$ from $H$.
  Let $H$ have vertices $v_1\prec_H\cdots\prec_H v_s$.

  Suppose $H'$ is obtained from $H$ by a vector deletion.
  Then $H$ and $H'$ have the same node set and edge set.
  Let $i\in[s]$.
  In the Definition~\ref{def:edge}, the set of coordinate arrays $\mathcal{X}_{v_i}(H')$ is the same as the set of coordinate arrays $\mathcal{X}_{v_i}(H)$, because $H$ and $H'$ are the same graph with the same edge-constraints.
  Since we assume $H$ is edge-satisfying, we have that $S_{v_i}(H)$ satisfies all the coordinate arrays in $\mathcal{X}_{v_i}(H)=\mathcal{X}_{v_i}(H')$, so $S_{v_i}(H')$ does as well, by Lemma~\ref{lem:stack-1}.
  This holds for all $i\in[s]$, so we have that $H'$ is edge-satisfying.

  Now suppose $H'$ is obtained from $H$ by a node deletion, so that the graph $H'$ is a subgraph of the graph $H$ with a leaf node deleted.
  We claim that, for all $i$ such that node $v_i$ is in $H'$, we have $\mathcal{X}_{v_i}(H')\subseteq\mathcal{X}_{v_i}(H)$.
  First, suppose $v_s$ is deleted from $H$ to give $H'$.
  Then, for each $i=1,\dots,s-1$, by Definition~\ref{def:edge}, the set $\mathcal{X}_{v_i}(H')$ is the same as the set of coordinate arrays $\mathcal{X}_{v_i}(H)$, except with $X^{v_s,v_1}_{v_s,i}$ deleted, and, if $v_i$ is a neighbor of $v_s$ (only true for $i=1$), with coordinate arrays $X^{v_s,v_i}_{v_i, j}$ deleted for $j\in[k']$, so indeed $\mathcal{X}_{v_i}(H')\subset\mathcal{X}_{v_i}(H)$.
  Now suppose $v_{s-1}$ is deleted from $H$ to give $H'$.
  For $1\le i\le s-2$, we have $\mathcal{X}_{v_i}(H')\subset\mathcal{X}_{v_i}(H)$ by the same reasoning as when $v_s$ is deleted.
  Additionally, we can show $\mathcal{X}_{v_s}(H')=\mathcal{X}_{v_s}(H)$: nodes $v_s$ and $v_{s-1}$ are not adjacent in $H$ (node deletions can only delete non-root nodes so $v_{s-1}$ is not the root) so all of the coordinate arrays of $\mathcal{X}_{v_s}(H)$ and $\mathcal{X}_{v_s}(H')$ in part 1 of Definition~\ref{def:edge} are the same, and $\mathcal{X}_{v_s}(H)$ and $\mathcal{X}_{v_s}(H')$ have no coordinate arrays in part 2 of Definition~\ref{def:edge} since $v_s$ is the largest node each of $\prec_{H}$ and $\prec_{H'}$.

  Thus, we have that $\mathcal{X}_{v_i}(H')\subseteq\mathcal{X}_{v_i}(H)$ for all nodes $v_i$ in $H'$.
  For all nodes $v_i$ in $H'$, we have the stacks $S_{v_i}(H')$ and $S_{v_i}(H)$ are the same, since no vector insertions/deletions were applied.
  Thus, since stack $S_{v_i}(H)$ satisfies all the coordinate arrays in $\mathcal{X}_{v_i}(H)$, we have $S_{v_i}(H')$ satisfies all the coordinate arrays in $\mathcal{X}_{v_i}(H')$, as desired.

  We have shown that if $H'$ is obtained by applying a single vector deletion or node deletion to $H$, and $H$ is valid, then $H'$ is valid.
  By the first paragraph of the proof, this completes the proof.
\end{proof}

%\begin{lemma}
%  Suppose $k$ is odd.
%  Let $H$ and $H'$ be configurations such that $H$ is obtained from applying a valid full operation consisting of a vector insertion at some node $v$, followed by a flip, followed by a vector deletion at some node $v'\neq v$. Then the full operation is valid if and only if both $H$ and $H'$ are valid.
%\end{lemma}
%\begin{proof}
%  The only if direction follows from the definition of a full operation.
%  By definition of a flip, $H$ and $H'$ each have two nodes $v$
%\end{proof}




\paragraph{Lemma for the Yes case}
The next lemma, illustrated in Figure~\ref{fig:yes-lemma}, shows why the tree structure of configurations keeps us from ``forgetting'' coordinate arrays too quickly, which is useful for the Yes case (see Section~\ref{ssec:proofsketch-2} in the overview).
%\ryl{Added some preamble and figure}
%\ryl{This lemma might be a nice one to have a picture for if it's not too hard. If you have tikz files for these eps images I can try to draw it. All I have in mind is a configuration, with a vertex $v'$, and a loop around all other nodes saying they need to be deleted before $v'$.}\mina{I'm using ipe, uploaded all source files in "figure sources" folder.}\ryl{Figure added}
\begin{figure}
    \centering
    \includegraphics{yes-lemma.pdf}
    \caption{Lemma~\ref{lem:yes-3}. In the example configuration of size $k=7$, to delete the root node $v'=\rho(H)$ (purple) without deleting $v$, one needs to delete all the red vectors and red nodes. This requires 3 node deletions and 3 vectors deletions for a total of $6=k-1$ deletions.}
    \label{fig:yes-lemma}
\end{figure}
\begin{lemma}
  Suppose $H$ is a size-$k$ configuration containing a non-root leaf node $v$ with $S_v(H)=\emptyset$ and edge $(v,v')$ where $v'=\rho(H)$.
  Suppose that one applies $c$ full operations among which node $v'$ is deleted but node $v$ is never deleted.
  Then $c\ge k-1$.
\label{lem:yes-3}
\end{lemma}
\begin{proof}
  Let $H_0=H,H_1,\dots,H_c$ be the sequence of configurations such that $H_i$ is the result of applying a valid full operation to $H_{i-1}$ for $i=1,\dots,c$.
  Let $v''\notin \{v,v'\}$ be an arbitrary node in $H$.
  We claim that node $v''$ must be deleted before node $v'$.
  Let $i\in\{0,\dots,c\}$ be the largest index such that $v''$ and $v$ are both in configuration $H_i$.
  Node $v'$ is on the path from node $v''$ to node $v$ in configuration graph $H_0$.
  Only leaf nodes can be deleted in a node deletion.
  Thus, as $v$ and $v''$ are both in $H_0,\dots,H_i$, all the nodes on the path from $v$ to $v''$ are also nodes in $H_0,\dots,H_i$.
  In particular, node $v'$ is in $H_0,\dots,H_i$, so node $v''$ must be deleted before $v'$. %\ryl{Added some more detail here.}%\mina{another potential explanation: $v'$ is the root, it should not be the root when we delete it, so at some point we flip, hence at that point we should have only two nodes.}
  
  Hence, the only way to delete node $v'$ without deleting node $v$ is to first delete all nodes other than $v'$ (by first deleting the vectors in their stacks and then the node) and then deleting $v'$.
  This results in deleting all nodes other than $v$, which takes at least $\sum_{u\in V(H)}^{} (1+|S_u(H)|) - (1+|S_v(H)|) = k-(1+0)$ deletions.
  Since each full operation applies at most one deletion, the number of full operations needed to delete $v'$ without deleting $v$ is at least $k-1$.
\end{proof}


\paragraph{Permutations commute with valid full operations}

The next few lemmas justify the informal statement that ``permutations commute with valid full operations''. 
This statement is convenient in the Yes case because it allows us to assume that all permutation edges are at the end of a path.
Intuitively, we expect this lemma to be true because changing the node labels of a configuration gives essentially the same configuration.
\begin{lemma}
  \label{lem:perm-1}
  Let $\pi:[2k']\to [2k']$ be a permutation.
  Let $H$ be a configuration, and suppose that applying a vector insertion (vector deletion, node insertion, node deletion, flip) on $H$ gives configuration $H'$.
  Then there exists a vector insertion (vector deletion, node insertion, node deletion, flip) that, applied to $\pi(H)$, gives $\pi(H')$.
\end{lemma}
\begin{proof}
  A vector $b\in A$ is inserted at node $v$ in $H$ ($v$ is a node label in $[2k']$) to give a configuration $H'$. 
  Suppose that inserting vector $b$ at node $\pi(v)$ in $\pi(H)$ gives a configuration $H''$.
  We claim $H''=\pi(H')$.
  By definition of vector insertion, $H''$ has the same nodes, edges, edge-constraints, root node, and ordering as configuration $\pi(H)$.
  Furthermore, since $H$ has the same nodes, edges, edge-constraints, root node, and ordering as configuration $H'$, we have $\pi(H)$ and $\pi(H')$, and thus $H''$ and $\pi(H')$ have the nodes, edges, edge-constraints, root node, and ordering.
  Furthermore, the stacks $S_{\pi(v)}(H'')$ and $S_{\pi(v)}(\pi(H'))$ are both equal to $S_v(H) + b$, and the stacks $S_{\pi(v')}(H'')$ and $S_{\pi(v')}(\pi(H'))$ are both equal to $S_{v'}(H)$ for nodes $v'\neq v$ in $H$, so we indeed have $H''=\pi(H')$.

  This proves the lemma for vector insertions.
  The proofs for vector deletions, node insertions, node deletions, and flips are similar.
\end{proof}
\begin{lemma}
  Let $\pi:[2k']\to [2k']$ be a permutation.
  If configuration $H$ is valid, then configuration $\pi(H)$ is valid.
\label{lem:perm-2}
\end{lemma}
\begin{proof}
  The root node $\rho(\pi(H))$ of $\pi(H)$ has the same stack as the root node $\rho(H)$ of $H$, which has at least $(k-2)/2$ vectors. %\mina{might not be needed after resolving the conflict between validity and flip edges}
  By definition of $\pi(H)$, for each node $v\in V(H)$, the set of coordinate arrays $\mathcal{X}_{\pi(v)}(H)$ is the same as $\mathcal{X}_{v}(H)$.
  Since $H$ is valid, $S_v(H)$ satisfies every coordinate array in $\mathcal{X}_v(H)$, so $S_{\pi(v)}(\pi(H))=S_v(H)$ satisfies every coordinate array in $\mathcal{X}_{\pi(v)}(\pi(H))=\mathcal{X}_v(H)$.
  This holds for all $v$, so $\pi(H)$ is edge-satisfying and thus valid.
\end{proof}
As a corollary of Lemmas~\ref{lem:perm-1} and \ref{lem:perm-2}, we have that permutations commute with valid full operations.
\begin{corollary}
  Let $\pi:[2k']\to [2k']$ be a permutation.
  Let $H$ be a configuration, and suppose that applying some valid full operation on $H$ gives configuration $H'$.
  Then applying some valid full operation on $\pi(H)$ gives $\pi(H')$.
  \label{cor:perm-3}
\end{corollary}






\subsection{No case.}
We now prove that when $\Phi$ has no solution, our Diameter instance has diameter at most $k$.
To do so, we find a length $k$ path between any two configurations $H$ and $H'$.
As sketched in the overview, we apply $k$ full operations to get $H'$ from $H$, and each operation inserts a vector or node ``from $H'$'' and deletes a vector or node ``from $H$''.
For an example of such a path when $k=7$, see Figure~\ref{fig:no-case}.
%\ryl{Added some preamble and moved the figure up}

\begin{figure}
    \centering
    \includegraphics{no-case-ex.pdf}
    \caption{The path of length $7$ between $H$ and $H'$ for $k=7$. Full operations are indicated by red arrows and roots are indicated by purple.
    The ``extra'' edge-constraint $Z$ that belongs to neither $H$ nor $H'$ is labeled in orange.
    %\ryl{Another nitpick, should the middle edge red text also have a ``flip''} \ryl{Also, it may help to label the edge constaint $Z$ in the diagram? either with an explicit label or just highlighting it}
   % \ryl{Updated figure.}
    }
    \label{fig:no-case}
\end{figure}




Let $H$ be an arbitrary size-$k$ configuration with vertices $v_1\prec_H\cdots\prec_H v_s$ for some $s\ge 1$, where $v_1=\rho(H)$ is the root, and with edges $v_1v_i$ with edge-constraint $X^{v_1,v_i}$ for $2\le i\le s$.
Let $H'$ be an arbitrary size-$k$ configuration with vertices $v'_1\prec_{H'}\dots\prec_{H'}v'_{s'}$ for some $s'\ge 1$, where $v'_1=\rho(H')$ is the root, and with edges $v'_1v'_i$ with edge-constraint $Y^{v_1',v_i'}$ for $2\le i\le s$.
By taking a permutation edge (of weight 0) from vertex $H'$ in the Diameter instance $G$ to obtain an equivalent configuration, we may assume without loss of generality that the set of node labels $\{v_1,\dots,v_s\}$ of $H$ are disjoint from the node labels $\{v_1',\dots,v_{s'}'\}$ of $H'$.

We now define an edge-constraint $Z$, containing the only ``extra'' coordinate arrays we need in the path from $H$ to $H'$.
Let $Z$ be a $(v_1,v_1')$-edge constraint such that, 
\begin{itemize}
\item For $i\in[k']$, coordinate array $Z_{v_1,i}$ is satisfied by stack $S_{v_1}(H)$ and, if $i\le s'$, by stack $S_{v'_i}(H')$, 
\item For $i\in[k']$, coordinate array $Z_{v'_1,i}$ is satisfied by stack $S_{v'_1}(H')$ and, if $i\le s$, by stack $S_{v_i}(H)$, and
\item $Z_{*}$ is satisfied by $S_{v_1}(H)$ and $S_{v_1'}(H')$.
\end{itemize}
As configurations $H$ and $H'$ are size-$k$ and have at least 1 stack, any stack of $H$ or $H'$ has at most $k-1$ vectors.
Hence, the coordinate arrays of $Z$ all exist by Lemma~\ref{lem:stack-2}.
Note that the definition of $Z$ is symmetric with respect to $H$ and $H'$, in the sense that if we switch $H$ with $H'$ (and $s$ with $s'$ and $(v_1,\dots,v_s)$ with $(v_1',\dots,v_s')$), the definition of $Z$ stays the same.

We now define two intermediate nodes $H_{mid}$ and $H_{mid}'$, which are on our desired path from $H$ to $H'$.
Let $H_{mid}$ be the configuration with nodes $v_1$ and $v'_1$, with the connecting edge having $(v_1,v_1')$-edge constraint $Z$, where 
\begin{itemize}
    \item $v_1=\rho(H_{mid})$ is the root, 
    \item $S_{v_1}(H_{mid})$ is the bottom $\ceil{(k-2)/2}$ elements of $S_{v_1}(H)$, and 
    \item $S_{v'_1}(H_{mid})$ is the bottom $\floor{(k-2)/2}$ elements of $S_{v'_1}(H')$. 
\end{itemize}

Let $H_{mid}'$ be the configuration with nodes $v_1$ and $v'_1$, with the connecting edge having $(v_1,v_1')$-edge constraint $Z$, where 
\begin{itemize}
    \item $v'_1=\rho(H_{mid}')$ is the root, 
    \item $S_{v'_1}(H_{mid}')$ is the bottom $\ceil{(k-2)/2}$ elements of $S_{v'_1}(H')$, and 
    \item $S_{v_1}(H_{mid}')$ is the bottom $\floor{(k-2)/2}$ elements of $S_{v_1}(H)$. 
\end{itemize}

We have that $H_{mid}$ and $H_{mid}'$ are valid: by the definition of the edge-constraint $Z$, we have that $S_{v_1}(H)$ and thus $S_{v_1}(H_{mid})$ satisfies $Z_{v_1,j}$ for all $j\in[k']$, and also satisfies coordinate array $Z_{v_1',1}$ and $Z_{*}$.
Similarly, $S_{v'_1}(H')$ and thus $S_{v'_1}(H_{mid})$ satisfies $Z_{v_1',j}$ for all $j\in[k']$, and also satisfies coordinate arrays $Z_{*}$.
Thus, $H_{mid}$ is edge-satisfying and thus valid.
By a symmetric argument, $H_{mid}'$ is also valid.
Note that $H_{mid}$ and $H_{mid}'$ are symmetric with respect to $H$ and $H'$, in the sense that if we switched $H$ and $H'$, then $H_{mid}$ becomes $H_{mid}'$ and vise-versa.

\begin{figure}
    \centering
    \includegraphics{no-case-tildeH.pdf}
    \caption{Claim~\ref{lem:no-4}, the configuration $\tilde H$ for Figure~\ref{fig:no-case}: all configurations on the path from $H$ to $H_{mid}$ are subconfigurations of $\tilde H$. By Lemma~\ref{lem:op-4}, showing $\tilde H$ is valid implies that the path from $H$ to $H_{mid}$ is valid.
    }
    \label{fig:no-case-tildeH}
\end{figure}



\begin{claim}
  One can apply $\floor{k/2}$ valid full operations on $H$ to obtain $H_{mid}$, and $\floor{k/2}$ valid full operations on $H'$ to obtain $H_{mid}'$.
\label{lem:no-4}
\end{claim}
\begin{proof}
  We prove this for $H$ and $H_{mid}$, and the result for $H'$ and $H_{mid}'$ follows from a symmetric argument (the symmetry holds because the definition of $Z$ and the definitions of $H_{mid}$ and $H_{mid}'$ are symmetric with respect to $H$ and $H'$). 
  Let $\tilde H$ be the configuration obtained by adding node $v'_1$ to $H$ with stack $S_{v'_1}(H_{mid}')$ (of size $\floor{(k-2)/2}$), with an edge $(v_1,v_1')$ having edge constraint $Z$, and such that the ordering $\prec_{\tilde H}$ agrees with $\prec_H$ on the nodes of $H$, and $v'_1$ is the largest node of $\prec_{\tilde H}$ (see Figure~\ref{fig:no-case-tildeH}).
  Note that $\tilde H$ has size larger than $k$ (to be precise, it has size $k+\floor{k/2}$).

  We first prove that $\tilde H$ is edge-satisfying.
  First, the set $\mathcal{X}_{v_1'}(\tilde H)$ has coordinate arrays $Z_*$ and $Z_{v_1',j}$ for $j\in[k']$, by part 1 of Definition~\ref{def:edge}, and has no coordinate arrays from part 2 of Definition~\ref{def:edge} as $v'_1$ is the largest node of $\prec_H$.
  By definition of $Z$, stack $S_{v'_1}(H')$ satisfies all these coordinate arrays, and thus by Lemma~\ref{lem:stack-2} stack $S_{v'_1}(H_{mid})$ does as well,   satisfying the requirement of Definition~\ref{def:edge} for node $v_1'$.
  For $i\in [s]$, the set of coordinate arrays in $\mathcal{X}_{v_i}(\tilde H)$ is the same as the set of coordinate arrays $\mathcal{X}_{v_i}(H)$ plus the coordinate array $Z_{v_1',i}$, and, if $i=1$, plus the coordinate arrays $Z_*$ and $Z^{v_1', v_1}_{v_1,j}$ for $j\in[k']$.
  By definition of $Z$, we have that $S_{v_i}(\tilde H) = S_{v_i}(H)$ satisfies coordinate array $Z_{v_1',i}$.
  Furthermore, $S_{v_1}(\tilde H)=S_{v_1}(H)$ satisfies coordinate arrays $Z_*$ and $Z_{v_1,j}$ for $j\in[k']$.
  Since configuration $H$ is edge-satisfying and the above coordinate arrays are satisfied, we conclude that configuration $\tilde H$ is edge-satisfying.

  We now note that $H_{mid}$ can be obtained from $H$ by applying the following half-operations
  \begin{itemize}
  \item Insert node $v_1'$ as the largest node in the ordering
  \item Insert vectors into $v_1'$ $\floor{(k-2)/2}$ times.
  \item For each $i=s,s-1,\dots,2$, delete vectors from $S_{v_i}$ until the stack is empty, and then delete node $v_i$.
  \item Delete vectors from $S_{v_1}$ until the stack has size $\ceil{(k-2)/2}$.
  \end{itemize}
  We can check that there are $\floor{k/2}$ insertions and $\sum_{i=1}^{s} (1+|S_{v_i}|) - (1+\ceil{k-2}/2) = k-\ceil{k/2}=\floor{k/2}$ deletions.
  We can obtain $H$ from $H_{mid}$ by alternating applying these insertions and deletions, giving a configurations $H=H_0,H_{0.5},H_1,\dots,H_{\floor{k/2}-0.5},H_{\floor{k/2}}=H_{mid}$, so that applying the $i$th insertion to $H_{i-1}$ gives the size-$k+1$ configuration $H_{i-0.5}$, and applying the $i$th deletion to $H_{i-0.5}$ gives the size-$k$ configuration $H_i$.
  These half-operations indeed satisfy the definition of half-operations: all the vector insertions/deletions are legal, the single node insertion is legal as $v_1'$ is inserted as the largest node, and all the node deletions are legal as the deleted nodes are always the second-largest node in the ordering.
  Furthermore, if we perform only the insertions, we obtain configuration $\tilde H$.
  Hence, any $i=0,0.5,\dots,\floor{k/2}$, we can obtain configuration $H_i$ from configuration $\tilde H$ by applying vector deletions at node $v_1'$ until stack $S_{v_1'}$ is the right size, and then applying the first $\floor{i}$ node/vector deletions above (at nodes $v_s,v_{s-1},\dots$).
  Thus, for $i=0,0.5,\dots,\floor{k/2}$ configuration $H_i$ is a subconfiguration of configuration $\tilde H$. 
  Since configuration $\tilde H$ is valid, by Lemma~\ref{lem:op-4}, each $H_i$ and $H_{i+0.5}$ is valid, so we have a sequence of $\floor{k/2}$ valid full operations that gives $H_{mid}$ from $H$.
%
  %By a symmteric argument, there is a sequence of $\floor{k/2}$ valid full operations that gives $H_{mid}'$ from $H'$.
\end{proof}

With Claim~\ref{lem:no-4}, we have nearly proved the No case.
It remains to show that $H_{mid}$ and $H_{mid}'$ are at distance either 0 or 1, depending on the parity of $k$.

If $k$ is even, then $H_{mid}$ can be obtained by applying a flip to $H_{mid}'$, and thus the two configurations are at distance 0 in the Diameter graph $G$.
Thus, there is a length $2\cdot \floor{k/2} = k$ path from $H$ to $H'$ through $H_{mid}$ and $H_{mid}'$ by Claim~\ref{lem:no-4}.

If $k$ is odd, then $H_{mid}$ is distance 1 from $H_{mid}'$:
$H_{mid}'$ is obtained from $H_{mid}$ by applying a vector insertion at node $v_1'$, giving a configuration $H_{mid,+}$, followed by a flip, giving a configuration $H_{mid,+}'$, followed by a vector deletion at node $v_1$, giving configuration $H_{mid}$.
The flip can be done because $H_{mid,+}$ and $H_{mid,+}'$ both have two nodes, each of which has a stack of size $\ceil{(k-2)/2}$.
We now check these half-operations are all valid operations, by checking that configurations $H_{mid,+}$ and $H_{mid,+}'$ are valid configurations.
Since no vectors are deleted at node $v_1'$ from $H_{mid,+}$ to $H_{mid}'$, we have $S_{v_1'}(H_{mid,+}) = S_{v_1'}(H_{mid}')$ is a substack of $S_{v_1'}(H')$, and similarly $S_{v_1}(H_{mid,+})=S_{v_1}(H_{mid})$ is a substack of $S_{v_1}(H)$.
Hence, by construction of $Z$ and Lemma~\ref{lem:stack-1}, stack $S_{v_1'}(H_{mid,+}) = S_{v_1'}(H_{mid}')$ satisfies coordinate array $Z_{v_1',j}$ for all $j\in[k']$ and also satisfies coordinate array $Z_*$, and the stack $S_{v_1}(H_{mid,+}) = S_{v_1}(H_{mid})$ at the root node of $H_{mid,+}$ satisfies $Z_{v_1,j}$ for all $j\in[k']$ and also satisfies coordinate arrays $Z_{v_1',1}$ and $Z_*$.
Hence, configuration $H_{mid,+}$ is edge-satisfying, and thus a valid configuration.
By a symmetric argument, configuration $H_{mid,+}'$ is valid.
Hence, configurations $H_{mid}$ and $H_{mid}'$ are adjacent in the diameter instance with an edge of weight 1, and we have a path from $H$ to $H'$ through $H_{mid}$ and $H_{mid}'$ of length $1+2\cdot \floor{k/2} = k$ by Claim~\ref{lem:no-4}. 

In either case, we have shown that, when $A$ has no $k$ orthogonal vectors, then for any two configurations $H$ and $H'$, there is a length $k$ path from $H$ to $H'$.
This completes the proof of the no case.






\subsection{Yes case.}
We now prove that the Diameter of $G$ is at least $2k-1$ in the Yes case.
Suppose $A$ has an orthogonal $k$-tuple $(a_1,\dots,a_k)$.
Throughout this section fix $v\in[2k']$ to be an arbitrary edge label (say $v=1$).
Let $H$ be the 1-stack configuration with a single node $v$ assigned with a stack $S_v(H)=(a_1,\dots,a_{k-1})$ (and a trivial ordering).
Let $H'$ be the 1-stack configuration with a single node labeled $v$ assigned with a stack $S_{v}(H')=(a_k,\dots,a_2)$. 
We claim configurations $H$ and $H'$ are at distance $2k-1$ in the Diameter graph $G$.


Consider a path $H_0=H,H_1,\dots,H_{r+1}=H'$ from $H$ to $H'$ using edges of $G$, and assume for contradiction this path has length $2k-2$ (if it has length less than $2k-2$, we may assume without loss of generality that in one of the $t$-stack vertices for $t\ge 2$, there are trivial valid full operations (e.g., node insertion followed by node deletion), which give self loop edges of weight 1, increasing the path length to $2k-2$).
This path contains some valid full operation edges, possibly some weight-0 flip edges if $k$ is even, and possibly some weight-0 permutation edges between equivalent configurations.
By Corollary~\ref{cor:perm-3}, we may assume without loss of generality that all weight-0 permutation edges are at the end of the path, and furthermore if there are multiple permutations $\pi_1,\dots,\pi_\ell:[2k']\to[2k']$, we may replace them by a single permutation $\pi=\pi_1\circ\cdots\pi_\ell$ by Lemma~\ref{lem:perm-0}.
Hence, we may assume that our path has $2k-2$ valid full operation edges, followed by a single weight-0 edge applying a permutation $\pi$.

Thus, we may assume that $r=2k-2$, and configuration $H'$ is $\pi(H_{2k-2})$ for some $\pi:[2k']\to[2k']$, so that configuration $H_{2k-2}$ contains a single stack at node $v'\defeq \pi^{-1}(v)$, and so that for $i=1,\dots,2k-2$, configuration $H_i$ can be reached from $H_{i-1}$ by an operation edge, and possibly a flip edge.
For each $i=0,\dots,2k-3$, the valid full operation on $H_i$ has one valid vector/node insertion, possibly followed by a flip operation, followed by one valid vector/node deletion, possibly followed by a flip, so we can let $H_{i+0.5}$ denote the result of only applying the insertion and possibly a flip to $H_i$, so that $H_{i+1}$ is the result of applying a deletion, possibly followed by a flip, to $H_{i+0.5}$.
By definition of a valid half-operation, configuration $H_{i+0.5}$ is valid (and has size $k+1$).

The following two claims reason about the stacks and the edge-constraints that must be on the path.
\begin{claim}
  If an edge $(w,w')$ appears in configuration $H_i$ for some integer $i=1,\dots,2k-3$, it also appears (with the corresponding edge-constraint) in configurations $H_{i-0.5}$ and $H_{i+0.5}$. 
\label{lem:yes-1.6}
\end{claim}
\begin{proof}
  Configuration $H_{i+0.5}$ is obtained by applying a vector or node insertion to $H_i$, possibly followed by a flip, so no node, and thus no edge is deleted from $H_i$ to $H_{i+0.5}$.
  Configuration $H_{i}$ is obtained by applying a vector or node deletion to $H_{i-0.5}$, possibly followed by a flip, so $H_{i-0.5}$ is obtained by possibly applying a flip to $H_i$, followed by a node or vector insertion, and again no edge is deleted.
\end{proof}

\begin{claim}
  For $0\le s\le k-1$, we have $S_v(H_s)$ and $S_v(H_{s+0.5})$ both contain $(a_1,\dots,a_{k-1-s})$ as a substack.
  For $k-1\le s\le 2k-2$, we have $S_{v'}(H_{s})$ and $S_{v'}(H_{s-0.5})$ both contain $(a_k,\dots,a_{2k-s})$ as a substack.
\label{lem:yes-2}
\end{claim}
\begin{proof}
  For the first item, we have $S_v(H_0)=(a_1,\dots,a_{k-1})$, and each of the first $s$ full operations deletes at most one vector from this stack, so stack $S_v(H_s)$ has $(a_1,\dots,a_{k-1-s})$ as a substack.
  By Claim~\ref{lem:yes-1.6}, $S_v(H_{i+0.5})$ does as well.
  Similarly, we have stack $S_v(H_{2k-2})=(a_k,\dots,a_2)$.
  Applying $2k-2-s$ full operations from $H_{2k-2}$ gives $H_{s}$, but each operation deletes at most one vector from the starting stack $S_{v'}(H_{2k-2})=(a_k,\dots,a_2)$.
  Hence, stack $S_v(H_{s})$ has $(a_k,\dots,a_{2k-s})$ as a substack, and by Claim~\ref{lem:yes-1.6}, stack $S_v(H_{s-0.5})$ does as well.
\end{proof}

Let $s$ be the largest index such that node $v$ is in configurations $H_0,\dots,H_s$ ($s$ exists because $H_0$ contains node $v$).
Let $s'$ be the smallest index such that node $v'$ is in configurations  $H_{s'},\dots,H_{2k-2}$ (again $s'$ exists because $H_{2k-2}$ contains node $v'$).
By the maximality of $s$ (and since we assume no permutation edges are used in $H_0,\dots,H_{2k-2}$), node $v$ has an empty stack in configuration graph $H_s$.
Node $v$ also has a size $k-1$ stack in $H_0$.
Since each valid full operation can delete at most one vector from some stack, we have that $s\ge k-1$.
Similarly, we have that $s'\le k-1$, so $s'\le s$.
Thus, nodes $v$ and $v'$ both appear in each of the configurations $H_{s'},\dots,H_s$.
We have three cases, and in each case, we show that our path contradicts Lemma~\ref{lem:yes-1}.

\textbf{Case 1. $v=v'$.}
This implies that $s'=0$ and $s=r$, and node $v$ appears in every configuration $H_0,\dots,H_{2k-2}$.
We have that the stack $S_v(H_0)=(a_1,\dots,a_{k-1})$, and $S_v(H_{2k-2})=(a_k,\dots,a_2)$.
Thus, to obtain $S_v(H_{r})$ from $S_v(H_0)$, one needs to apply $k-1$ vector deletions followed by $k-1$ vector insertions.
Since each valid full operation applies at most one vector insertion followed by at most one vector deletion, the first $k-1$ full operations of our path must include a vector deletion at node $v$, and the last $k-1$ edges must include a vector insertion at node $v$, inserting the vectors $a_k,\dots,a_2$ in that order.
In particular, we have $S_v(H_k) = (a_k)$.

Because valid full operations must have one endpoint with at least two nodes, $H_0$ to $H_1$ operation must include a node insertion of some node $w\neq v$ with an edge $(v,w)$.
By Claim~\ref{lem:yes-1.6} the edge $(v,w)$ with an edge constraint $X^{v,w}$ appears in configuration $H_{0.5}$, so stack $S_v(H_{0.5}) = (a_1,\dots,a_{k-1})$ satisfies coordinate array $X^{v,w}_{*}$.
Furthermore, since there are no node-deletions in the first $k-1$ valid full operations (because each full operation deletes either a vector or node, not both), we know the edge $(v,w)$ exists in each of $H_1,\dots,H_{k-1}$. 
By Claim~\ref{lem:yes-1.6} the edge $(v,w)$ labeled with the edge constraint $X^{v,w}$ also exist in configuration $H_{k-0.5}$.
Additionally, as we reasoned earlier, $S_v(H_{k-0.5})=(a_k)$, so stack $(a_k)$ satisfies coordinate array $X^{v,w}_*$.
However, this means that stacks $(a_1,\dots,a_{k-1})$ and $(a_k)$ both satisfy $X^{v,w}_*$, which is a contradiction of Lemma~\ref{lem:yes-1}.


\textbf{Case 2. $v\neq v'$ and nodes $v$ and $v'$ are adjacent in configuration $H_{s'}$.}
Clearly we have $s'\ge 1$ and $s\le 2k-3$ in this case.
In configuration $H_{s'}$, node $v'$ is a non-root leaf node with an empty stack $S_{v'}(H_{s'})=\emptyset$ and incident edge $(v,v')$.
Furthermore, from configuration $H_{s'}$ to $H_{s+1}$, node $v$ is deleted, but node $v'$ is in configurations $H_{s'},\dots,H_{s+1}$.
Hence, by Lemma~\ref{lem:yes-3}, we have $(s+1)-s'\ge k-1$.

By Claim~\ref{lem:yes-1.6}, both configurations $H_{s'-0.5}$ and $H_{s+0.5}$ contain the edge $(v,v')$ with edge-constraint $X^{v,v'}$.
By Claim~\ref{lem:yes-2}, in configuration $H_{s'-0.5}$, node $v$ is labeled with a stack that contains $(a_1,\dots,a_{k-s'})$ as a substack, so by Lemma~\ref{lem:stack-1}, stack $(a_1,\dots,a_{k-s'})$ satisfies coordinate array $X^{v,v'}_*$.
Similarly, by Claim~\ref{lem:yes-2}, in configuration $H_{s+0.5}$, node $v'$ is labeled with a stack that contains $(a_k,\dots,a_{2k-1-s})$ as a substack, so stack $(a_k,\dots,a_{2k-1-s})$ satisfies coordinate array $X^{v,v'}_*$.
Since $k-s'\ge (2k-1-s)-1$, we have that, for $j=k-s'$, both stacks $(a_1,\dots,a_j)$ and $(a_k,\dots,a_{j+1})$ satisfies coordinate array $X^{v,v'}_{*}$, which is a contradiction by Lemma~\ref{lem:yes-1}.



\textbf{Case 3. $v\neq v'$ and nodes $v$ and $v'$ are not adjacent in configuration $H_{s'}$.}
In any configuration, the root node is adjacent to all other vertices, so $v$ and $v'$ must both be non-root nodes.
Suppose that in configuration $H_{s'}$, the root node is $w=\rho(H_{s'})$.
Since only leaf nodes in a configuration can be deleted, and since nodes $v$ and $v'$ are not deleted in $H_{s'},\dots,H_{s}$, we have that node $w$ exists and has degree at least two in each of $H_{s'},\dots,H_s$, and therefore must be the root node in each of $H_{s'},\dots,H_s$.
In particular, since the total order $\prec_H$ and root node of a configuration $H$ can only be changed when there are at most two vertices, no full operations from $H_{s'}$ to $H_s$ include flip operations.
Consequently, nodes $v$ and $v'$ have the same order with respect to orderings $\prec_{H_{s'}}$ and $\prec_{H_s}$

Assume without loss of generality that $v\prec_{H_{s'}} v'$ and $v\prec_{H_s} v'$ (the reverse direction is symmetric).
Let $t'$ be the largest index such that node $w$ is in configuration $H_{t'}$ ($t'\le 2k-3$ because configuration $H_{2k-2}$ only contains node $v'$). 
By maximality of $t'$, from configuration $H_{t'}$ to $H_{t'+1}$, node $w$ is deleted, so by Lemma~\ref{lem:yes-3}, $t'-s'\ge k-2$.
By Claim~\ref{lem:yes-1.6}, both $v$ and $v'$ are in $H_{s'-0.5}$.
Let $i_v$ be such that $v$ is the $i_v$th smallest node in configuration $H_{s'-0.5}$ according to $\prec_{H_{s'-0.5}}$.
Because $v\prec_{H_{s'-0.5}}v'$, and since configuration $H_{s'-0.5}$ is valid, Definition~\ref{def:edge} gives that stack $S_v(H_{s'-0.5})$ satisfies coordinate array $X^{v',w}_{v',i_v}$.
By Claim~\ref{lem:yes-2}, $(a_1,\dots,a_{k-s'})$ is a substack of $S_v(H_{s'-0.5})$, so by Lemma~\ref{lem:stack-1}, stack $(a_1,\dots,a_{k-s'})$ also satisfies coordinate array $X^{v',w}_{v',i_v}$.
On the other hand, by Claim~\ref{lem:yes-2}, $(a_k,\dots,a_{2k-1-t'})$ is a substack of $S_v(H_{t'+0.5})$.
Additionally, by Claim~\ref{lem:yes-1.6}, edge $(v',w)$ is also in $H_{t'+0.5}$, so stack $S_v(H_{t'+0.5})$, and thus stack $(a_k,\dots,a_{2k-1-t'})$, satisfies coordinate array $X^{v',w}_{v',i_v}$.
Since $k-s'\ge (2k-1-t)-1$, we have that for $j=k-s'$, stacks $(a_1,\dots,a_j)$ and $(a_k,\dots,a_{j+1})$ satisfy the same coordinate array $X^{v',w}_{v',i_v}$, which is a contradiction by Lemma~\ref{lem:yes-1}.


In all cases of $v$ and $v'$, we have shown a contradiction.
Thus, the path from configuration $H$ to configuration $H'$ in the Diameter instance $G$ cannot have length $2k-2$. 
Thus, when $A$ has $k$ orthogonal vectors, the Diameter of $G$ is at least $2k-1$.
This completes the proof.




















 


==> camera_ready/README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> old_proofsketch.tex <==
\section{Overview of the general $k$ reduction}
\label{sec:proofsketch}

We now sketch the ideas of the proof of Theorem~\ref{thm:main} for general $k$.

\subsection{The basic setup}
\label{ssec:proofsketch-0}
For our general reduction, we start with a $k$-OV instance $A\subset\{0,1\}^{\mathbb{d}}$ with size $|A|=n_{OV}$ and would like to construct a graph $G$ on $\tilde O(n_{OV}^{k-1})$ vertices and edges such that, if the set $A$ has $k$ orthogonal vectors (Yes case), the diameter of $G$ is at least $2k-1$, and otherwise (No case) the diameter of $G$ is at most $k$.
Throughout, we refer to elements of $A$ as \emph{vectors} and elements of $[\mathbb{d}]$ as \emph{coordinates}.
We may assume without loss of generality that the all ones vector $\mathbf{1}$ is in the set $A$.
We may also assume without loss of generality that no $k-1$ vectors of $A$ are orthogonal, as this can be checked in $\tilde O(n_{OV}^{k-1})$ time, and if there were then we already know we have $k$ orthogonal vectors (these assumptions help in motivating the construction).
Like in the prior constructions for $k=2,3,4$, the graph $G$ contains an ``endpoint vertex'' for each element of $A^{k-1}$, as well as some ``internal vertices'', identified by at most $k-2$ vectors in $A$, and some constant (in terms of $k$) number of \emph{coordinates} in $[\mathbb{d}]$.
Accordingly, we think each vertex of $G$ as a \emph{configuration} $H$ of vectors (in $A$) and coordinates (in $[\mathbb{d}]$).
Some configurations $H$ are \emph{valid}, meaning vectors in $H$ have 1s in specified coordinates of $H$, and there is one vertex of $G$ for each valid configuration.
Edges between vertices (configurations) of $G$ change up to one vector of a configuration and/or some of the coordinates of the configuration, and we think of edges as performing \emph{operations} on configurations.
To ensure the graph is undirected, we need to choose operations that always have an inverse operation.

\subsection{The vectors in a configuration}
\label{ssec:proofsketch-1}
The reduction graph $G$ has the property that, for any two vertices $v$ and $v'$ identified by vectors $a_1,\dots,a_s$ and $a_1',\dots,a_{s'}'$, respectively, for $s,s'\le k-1$, (and possibly some coordinates), if any subset of $k$ vectors from $a_1,\dots,a_s,a_1',\dots,a_{s'}'$ are not orthogonal (No case), then vertices $v$ and $v'$ are at distance at most $k$.
Furthermore, in the Yes case, if $a_1,\dots,a_k$ are $k$ orthogonal vectors, then the endpoint vertices $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ should be at distance $2k-1$.
Already, these requirements impose the following structure on the construction:

\paragraph{In the Yes case, a path of length at most $k-2$ from endpoint vertex $(a_1,\dots,a_{k-1})$ should not drop vector $a_1$.}
That is, after taking $k-2$ edges from the endpoint vertex $v=(a_1,\dots,a_{k-1})$, one cannot arrive at a configuration $u=(b_1,\dots,b_s, \bar x)$ of vectors $b_1,\dots,b_s$ and coordinates $\bar x$ where $a_1$ is not among vectors $b_1,\dots,b_s$.
Suppose not for contradiction, and suppose $a_1,a_2,\dots,a_k$ form the orthogonal $k$-tuple in the Yes case.
If all of the ``new'' vectors added are the all ones vector $\mathbf{1}$, then the vectors $\{b_1,\dots,b_s\}$ contain only vectors from $(a_2,\dots,a_{k-1},\mathbf{1})$.
Then among $b_1,\dots,b_s, a_k,a_{k-1},\dots,a_2,\mathbf{1}$, any $k$ vectors are orthogonal, so vertex $(b_1,\dots,b_s,\bar x)$ should be distance at most $k$ from endpoint vertex $v'=(a_k,\dots,a_2)$ by our requirement for the No case.
Hence, if $d(v,u)\le k-2$, then by the triangle inequality, we have $d(v,v')\le d(v,u)+d(u,v')\le 2k-2$, which contradicts our large diameter requirement for the Yes case.

For the same reason, a path of length at most $k-2$ from endpoint vertex $(a_k,\dots,a_2)$ should not drop vector $a_k$.
This idea leads to our next idea.

\paragraph{Using ``stacks''}
Here, stacks refer to the ``first-in-last-out'' data structure.
We identify a configuration by several ``stacks'' $S_1,\dots,S_t$, where each stack $S_i$ is simply a tuple of a nonnegative number of vectors of $A$ (the configuration may also be identified by some coordinates).
The endpoint vertices of the Diameter instance are configurations with a single stack of size $k-1$.
We think of these tuples of vectors as ``stacks'' so that operations consist of popping a vector from one stack and pushing a vector onto another stack.
In particular, an operation can only touch the ``top'' vector of any given stack.
This ensures that in the Yes case, for the endpoint vertices with stacks $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$, it takes $k-1$ operations to delete the vectors $a_1$ and $a_k$ from their respective stacks, because each operation can remove at most one vector from the top of the stack.
We point out that our constructions for $k=4$ and $k=5$ are written in this stack language.

\paragraph{More than two stacks}
For $k=4$ and $k=5$, it suffices to construct our Diameter instance with vertices that are configurations with at most two stacks, but for general $k$, more stacks seem necessary: if $k$ is large, and there were two configurations $H$ and $H'$ each with two stacks $S_1,S_2$ and $S_1',S_2'$ each of size roughly $k/2$, if one is constrained to only having two stacks, one needs around $3k/2$ vector insertion+vector deletion operations to reach configuration $S_1',S_2'$ from $S_1,S_2$, which is too much in the No case.

\paragraph{A general operation} (Definition~\ref{def:op})
For general $k$, to accommodate for more than two stacks, we define operations (edges of the Diameter instance) as follows.
Operations on configurations consist of one ``insertion'' \emph{half-operation} and one ``deletion'' half-operation.
An insertion half-operation either pushes a vector onto some stack or creates a new empty stack (along with some coordinates), and a deletion half-operation either deletes (pops) a vector from some stack or deletes an empty stack.\footnote{For technical reasons, in the final construction, we require that operations that do the insertion half-operation before the deletion half-operation, which contrasts with the $k=4$ and $k=5$ case where the deletions are done first. Roughly, this change saves a +1 in the Yes case.}\footnote{Also for technical reasons, in specific cases of the general $k$ construction, we also allow a operation to perform a ``flip'' operation between the insertion and deletion, which changes some of the ``meta-data'' of a configuration.}

Conveniently, \emph{all} edges of our generalized construction can be described by such operations.
In the $k=4$ and $k=5$ case, the edges that apply a vector insertion followed by a vector deletion cover all of the edges in the graph, except for (1) the edges from endpoint vertices with one stack to internal vertices with two stacks, and (2) the edges that change the coordinates (``coordinate change edges'').
However, for our general $k$ construction, we do not use the coordinate change edges from (2) (intuition for why is given below), this generalized definition of an operation now includes edges from (1): for example, in the $k=4$ case, the edge from $(a,b,c)\in A^3$ to $(\{(a,b),()\},x,y)\in A^2\times ([\mathbb{d}]^3)^2$ can be seen as the operation of inserting an empty stack $()$ and coordinates $x$ and $y$, and then deleting the vector $c$ from the top of the stack $(a,b,c)$.
Furthermore, these operations are invertible (e.g., a vector insertion plus stack deletion can be inverted by applying a stack insertion plus a vector deletion), so our Diameter instance is indeed undirected.


\paragraph{Size: how big are configurations?} (Definition~\ref{def:size})
We also need to specify how many vectors (and stacks) we can have in a configuration.
We note that the total number of vectors plus the total number of stacks is invariant under our defined operations: each ``insertion'' (of a vector or a stack) increases this quantity by 1, and each ``deletion'' (of a vector or a stack) decreases this quantity by 1.
Accordingly, we give this quantity a special name, calling it the \emph{size} of a configuration. 
The endpoint vertices have 1 stack and $k-1$ vectors, so the size of configurations at endpoint vertices is $k$.
Since operations preserve size, we therefore require that all configurations (vertices) in our Diameter instance have size $k$.
The size definition also has the property that, if we ignore coordinates, it is always possible to reach one size $k$ configuration from any other size $k$ configuration with $k$ operations, giving us hope that we can achieve Diameter $k$ in the No case.














\subsection{The coordinates in a configuration}
\label{ssec:proofsketch-2}
We have specified the structure of vectors in the configurations, namely, that we place them in first-in-last-out stacks so that the total size (number of stacks plus number of vectors in stacks) is $k$, and operations push and pop vectors from stacks and add and delete empty stacks.
Now, we need to specify the coordinates in the configurations.
In particular, we need to specify how the operations change the coordinates, and which coordinates constrain (need to be satisfied by) which stacks.

As argued above, we expect that for general $k$, our configurations need more than two stacks, and the main challenge that remains is specifying how the coordinates in configurations constrain the vectors in those stacks.
The constraints must be strong enough that in the Yes case, the 1-stack configurations $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ are not too close, but loose enough that any two configurations can reach each other in $k$ steps in the No case.
Conveniently for our construction, we only need to specify when configurations are valid vertices of our graph: we let an operation give a valid edge as long as the incident configurations are valid.
We now describe the additional ideas needed to specify the coordinates of configurations, starting with the most concrete ones.


\paragraph{Coordinate arrays}
A key abstraction that was implicit in prior constructions but that we explicitly use is something we call \emph{coordinate arrays}.
For a $k$-OV instance $A\subset\{0,1\}^{\mathbb{d}}$, a coordinate array is simply an element of $[\mathbb{d}]^{k-1}$ (Definition~\ref{def:coord-1}).
With this notion, we define what it means for a stack $S=(a_1,\dots,a_{|S|})$ to \emph{satisfy} a coordinate array $x$, which requries the vectors $a_1,\dots,a_{|S|}$ in the stacks have ones in certain coordinates of the array (Definition~\ref{def:coord-2}).
With these definitions, coordinate arrays become a useful primitive because of the following nice properties, which are helpful for achieving the balance we need between the Yes case having large diameter and the No case having small diameter.
\begin{enumerate}
\item (Lemma~\ref{lem:stack-2}, useful for the No case) Let $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$ be stacks with at most $k-1$ vectors such that any $k$ vectors from among $a_1,\dots,a_s,b_1,\dots,b_{s'}$ are orthogonal.
Then there exists a coordinate array satisfied by both $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$.
\item (Lemma~\ref{lem:yes-1}, useful for the Yes case) If $a_1,\dots,a_k$ are orthogonal, and $x$ is a coordinate array, then the stacks $(a_1,\dots,a_j)$ and $(a_k,\dots,a_{j+1})$ cannot satisfy $x$ simultaneously,
\end{enumerate}

At this point, we have described all of the ideas that are common to our general $k$ construction and the small case constructions for $k=4$ and $k=5$ (Section~\ref{sec:k4} and Appendix~\ref{app:k5}).
Coordinate arrays are also used as primitives in our simplified proofs for $k=4$ and $k=5$.
However, because we optimized the presentation of the $k=4$ and $k=5$ constructions for brevity and simplicity and not for generalizability, the ways the coordinate arrays constrain the stacks is slightly different from the way the coordinates constrain the stacks in the general construction.
The remaining ideas specific are to the general $k$ construction.




\paragraph{No case: Coordinate arrays constrain at most two stacks.} (See Definition~\ref{def:edge} and Table~\ref{tab:edgesatisfying})
The next two ideas may or may not be necessary but are at least convenient.
In the No case, for any two configurations $H$ and $H'$, we need to construct a path $H_0=H,H_1,\dots,H_k=H'$ from $H$ to $H'$, such that configuration $H_i$ is obtained by applying some operation to $H_{i-1}$ for all $i=1,\dots,k$.
Since configurations $H$ and $H'$ have size $k$, in each of the $k$ operations on the path, the insertion operation must add a vector or stack ``belonging to'' $H'$ and the deletion operation must delete a vector or stack ``belonging to'' $H$ (the notion that some configurations ``share'' stacks can be formalized by assigning labels to stacks, see Definition~\ref{def:configuration}).
Hence, each intermediate configuration $H_i$ contains some stacks and coordinate arrays ``belonging to'' $H$, some stacks and coordinate arrays ``belonging to'' $H'$, and possibly some additional coordinate arrays. 
However, it is possible that none of the vectors in $H$ have ones in any of the coordinates in $H'$, and vise versa.
Thus, it is important that for each $H_i$, none of the coordinate arrays ``belonging to'' $H$ constrain any of the stacks ``belonging to'' $H'$, and vise versa.
This is easiest to guarantee if at most two stacks are ever required to satisfy any coordinate array, and we found this assumption not make the Yes case much harder.
By similar reasoning, we also have the following idea.

\paragraph{No case: Require every configuration has a stack with at least $\ceil{(k-2)/2}$ vectors.} (Definition~\ref{def:valid})
Without this constraint, there could be two size-$k$ configurations $H$ and $H'$ with $\Omega(k)$ stacks of $O(1)$ vectors each such that none of the coordinate arrays from $H$ are satisfied by stacks in $H'$ and vise versa.
In the No case, these two configurations $H$ and $H'$ must be connected by a length $k$ path $H_0=H,H_1,\dots,H_k=H'$.
Then, the intermediate configuration $H_{k/2}$ must have $\Omega(k)$ stacks from $H$ and also $\Omega(k)$ stacks from $H'$.
It is easily possible that configuration $H_{k/2}$ has at least one coordinate array for every pair of stacks (in fact, below we show that having only one coordinate array for each pair of stacks is not enough for the Yes case), so we likely have $\Omega(k^2)$ coordinate arrays in $H_{k/2}$ that belong to neither $H$ or $H'$ but constrain some stack in $H$ and another stack in $H'$.
All $\Omega(k^2)$ must be all inserted and then deleted on the path from $H$ to $H'$, giving a lot of ``extra'' coordinate arrays to keep track of.

Requiring that every configuration has a stack with at least $\ceil{(k-2)/2}$ vectors means that, in the No case, we can find a path $H_0=H,H_1,\dots,H_k=H'$ between two configurations $H$ and $H'$, such that in each intermediate configuration $H_i$, there is either only \emph{one} stack from $H$ or only \emph{one} stack from $H'$, giving only $O(k)$ ``extra'' coordinate arrays to keep track of, an improvement from $\Omega(k^2)$ such coordinate arrays.
Furthermore, this requirement does not seem to affect the Yes case, and our Yes case proof does not seem to use this assumption.








\paragraph{Yes case: No coordinate change edge.}
In the $k=4$ and $k=5$ constructions in this work, at every vertex, there is an edge that changes \emph{all} the coordinates of an edge, e.g., from $(a,b,x,y)_{L_2}\in A^2\times ([\mathbb{d}]^3)^2$ to $(a,b,x',y')_{L_2}$ in the case of $k=4$.
However, these ``coordinate-change edges'' cannot exist in the general construction.
Indeed, if such edges existed, then in the Yes case, configurations $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ would be at distance only $3k/2+O(1)$.
From $(a_1,\dots,a_{k-1})$, we could (i) reach a configuration with stacks $(a_1,\dots,a_{k/2-O(1)}), (\mathbf{1},\dots,\mathbf{1})$ in roughly $k/2$ operations, (ii) apply a coordinate change edge, (iii) reach a configuration with stacks $(a_k,\dots,a_{k/2+O(1)}),(\mathbf{1},\dots,\mathbf{1})$ in roughly $k/2$ operations, (iv) apply a coordinate change edge, and (v) reach configuration $(a_k,\dots,a_{2})$ in roughly $k/2$ operations.
Indeed, the coordinate change edges divide the path into three subpaths, and in each subpath we never ``see'' all of the vectors $a_1,\dots,a_k$ in the stacks, so we can choose the coordinate arrays so that the stacks always satisfy the coordinate arrays, hence giving a valid path (we assumed without loss of generality that no $k-1$ vectors are orthogonal).
Thus, for the Yes case, changing coordinates needs to be more expensive that one edge.



\paragraph{Yes case: Remembering coordinate arrays (a.k.a. coordinate arrays constraining phantom stacks)} (See comments after Definition~\ref{def:edge})
One natural (but incorrect) way of implementing the above ideas is, in a configuration with stacks $S_1,\dots,S_t$, have $\binom{t}{2}$ coordinate arrays, $x^{i,j}$ for $1\le i<j\le t$, and require that stacks $S_i$ and $S_j$ satisfy coordinate array $x^{i,j}$.
Adding an empty stack $S_{t+1}$ to a configuration with $t$ stacks adds $t$ coordinate arrays $x^{i,t+1}$, one for each pair of stacks $(S_i,S_{t+1})$, and deleting a stack $S_{t}$ deletes the $t-1$ coordinate arrays that constrain it.
This construction does not work, because in the Yes case, as in the previous paragraph, it is again possible for the 1-stack configuration $(a_1,\dots,a_{k-1})$ to reach the 1-stack configuration $(a_k,\dots,a_2)$ in $3k/2+O(1)$ steps, by passing through the two stack configurations with stacks $(a_1,\dots,a_{k/2-O(1)}), (\mathbf{1},\dots,\mathbf{1})$ and $(a_k,\dots,a_{k/2+O(1)}),(\mathbf{1},\dots,\mathbf{1})$.

To work around this problem we have configurations $H$ ``remember'' some coordinate arrays that constrain deleted stacks.
That is, if an operation on configuration $H$ deletes a stack $S$ to obtain configuration $H'$, some of the coordinate arrays of $H$ that $S$ needed to satisfy are still coordinate arrays of configuration $H'$.
In this way, some coordinate arrays of a configuration constrain two stacks and other coordinate arrays only constrain one stack (such coordinate arrays can be thought of as constraining a real stack and a ``phantom'' stack).
This works, but one needs to be careful in how many coordinate arrays are ``remembered'', or else the No case might have large diameter.

\paragraph{Balancing the No case and Yes case: a tree and an ordering $\prec_H$ on the stacks.} (Definition~\ref{def:configuration})
The Yes case, particularly the $3k/2+O(1)$-path counterexample, encourages us to remember more constraints, but having Diameter $k$ in the No case keeps us from remembering too many constraints.
In the final construction, to help with this balance, we add two additional structures to configurations: 
\begin{enumerate}
\item Put an ordering $\prec_H$ on the stacks of a configuration $H$, so that we have a list of stacks, rather than simply a set of stacks.
Whether a stack is constrained by a certain coordinate array then depends on the location of the stack in the ordering. 

\item We place the stacks $S_1,\dots,S_t$ of a configuration $H$ at the vertices of a tree on $t$ vertices (in particular, a star graph on $t$ vertices). Coordinate arrays are attached to the edges of the tree so that a coordinate array is added to (deleted from) the configuration exactly when the corresponding edge is added to (deleted from) the configuration.
For clarity, we emphasize that there are now two types of graphs: the tree graphs $H$ that define a configuration, and the Diameter instance $G$, whose vertices are configurations $H$.

With this tree, we remember some, but not too many, coordinate arrays that constrained deleted vertices (Lemma~\ref{lem:yes-3}).
In particular, for an edge connecting stacks $S_i$ and $S_j$, we keep track of the coordinate arrays that constrain $S_i$ and some other (possibly non-existent) stack, and also the coordinate arrays that constrain $S_j$ and some other (possibly non-existent) stack.
Somewhat subtly, the coordinate arrays attached to an edge may constrain stacks not incident to the edge.
For the coordinate arrays constraining $S_i$, whether the coordinate arrays constrain another real stack or a non-existent stack depends on the ordering $\prec_H$.
\end{enumerate}














==> prior_construction/construction.tex <==
\section{Construction}

%\ryl{2/11/21 I might have a way of simplifying the whole construction. I will try writing it up and see if it works. If it doesn't I will go back to fixing up the No case.}\mina{would be amazing if you simplify it!}
%\ryl{The simplification didnt work. I will go finish up the No case.}
%\ryl{This is a new file where I am playing around with rewriting (essentially the same) construction. The old one is in construction\_old.tex}
We describe below a reduction from $k$-OV to $2k-1$ vs. $k$ Diameter with time $n^{k/(k-1)}$ on graphs with edges of weight 1 or 0.
This immediately gives a reduction from $k$-OV to $2k-1$ vs. $k$ Diameter with time $n^{k/(k-1)}$ on unweighted graphs, by contracting the edges of weight 0.
For clarity of exposition, we describe the reduction to the 0/1-weighted graph.

Let $A$ be a $k$-OV instance, meaning that $A$ is a set of $n$ vectors of length $O(\log{n})$. We create a graph $G$ using this instance. 
First we need a few definitions. 
\TODO{$[d]=\{1,\dots,d\}$ in prelims}

\subsection{Preliminaries for the construction}
Throughout the construction, fix $k'=k-\ceil{\frac{k-2}{2}}$.
A \emph{stack} $S=(a_1,\dots,a_{|S|})\in A^*$ is a vector of a nonnegative number of elements of $A^*$.
Denote $a_1$ as the \emph{bottom} element of the stack and $a_{|S|}$ as the \emph{top} element of the stack.
%Our constructions consist of stacks, where the contents of all the stacks are vectors of $A$. We show the vectors in  a stack by a tuple $(a_1,\ldots,a_{|S|})$, where the order of the elements are from left to right, $a_1$ is at the bottom of the stack, and $a_{|S|}$ is in the top. 
Given a stack $S=(a_1,\dots,a_\ell)$, a \emph{substack} $S_{\le \ell'}=(a_1,\dots,a_{\ell'})$ is given by a prefix of the bottom $\ell'$ vectors of $S$, where $\ell'\le \ell$.
The stack $popped(S)$ is the stack $(a_1,\dots,a_{\ell-1})$, i.e., the stack $S$ with the top element removed.
A \emph{stack array} $\vec S$ is a tuple of stacks $(S_{t-1},\dots,S_0)$.%\ryl{I defined this here because we use it by Definition 1.4}
The \emph{type} of a stack array $\vec S$ is $t$, the number of stacks in the stack array.
The \emph{weight} $|\vec S|$ of a stack array $\vec S$ is $t+\sum_{i=0}^{t-1} |S_i|$.
In a stack array $\vec S$, we refer to $S_0$ as the \emph{big stack}, and $S_{t-1}$ as the \emph{main stack}.
Accordingly, we sometimes denote $S_0$ by $S_{big}$ and $S_{t-1}$ by $S_{main}$.

\begin{definition}
A \emph{coordinate-array $x$} is an element of $[d]^{k-1}$.
\end{definition}
For a coordinate array $x\in[d]^{k-1}$ and an integer $\ell\in[k-1]$, let $x[\ell]$ denote the $\ell$th coordinate in the coordinate array $x$. 
Also for a coordinate $c$ and a vector $a\in A$, $a[c]$ is the $c$th coordinate of $a$. 
We index coordinate arrays by $x[\ell]$ and vectors in $A$ by $a[c]$, rather than $x_\ell$ and $a_c$ (respectively), for clarity.
\begin{definition}
%\textbf{Coordinate multi-array $X$} consists of two sections: $X^{(main)}, X^{(big)}$, each of which is decomposed into $k'-1$ subsections: $X^{(main)}$ is decomposed into $X^{(main,i)}$ for $i=1,\ldots,k'-2$ and $X^{(main,big)}$. Similarly, $X^{(big)}$ has the following subsections: $X^{(big,i)}$ for $i=1,\ldots,k'-2$ and $X^{(big,main)}$. We additionally require $X^{(big,main)}=X^{(main,big)}$. We call these subsections \textit{``coordinate arrays''} (hence a coordinate multi array consists of many coordinate arrays). Each of these coordinate arrays has $k-1$ coordinates.
A \emph{coordinate multi-array $X$} is a tuple of $2k'-2$ coordinate-arrays: $X^{(main,i)}$ for $i=big,1,\dots,k'-2$, and $X^{(big,i)}$ for $i=1,\dots,k'-2,main$. We additionally require $X^{(big,main)}=X^{(main,big)}$.
%\mina{commenting the previous comments... I think $X_{main,(main,i)}$ would be super confusing. I would say we remove the super script (indicating the node $\alpha$) of the coordinate multi arrays in the definition of nodes, and let the subsection indicators be super scripts here as it is. This is if you don't use the super script indicating the nodes in the NO case, I don't use it in the yes case.}
%\ryl{Sure that's fine. So you suggestion is just to do $X_{main}^{(main,i)}$ without $\alpha$ in the superscript. That's fine with me. You could also do $X^{main}_{(main,i)}$, so that you write your vertices of $G$ as $(S_{main},\dots,S_{big}, X^{main},\dots,X^1)$ and you index into $X^t$ by $X^t_{(main,i)}$, which feels more natural to me, but it's fine either way.}\mina{yeah i agree that it feels more natural but i feel like the indices jumping from subscript in stacks to super script coordinates might be confusing again too.}
%\ryl{What if we did $(S^{main},\dots,S^{big}, X^{main},\dots,X^1)$? }
\ryl{Also, are you sure you don't need the superscript $\alpha$? It seems pretty useful, for example, in the edge definitions, and consequently in the No case when I have to reason about the edges being valid. Maybe we should just keep the old notation?} \mina{yeah i need the $\alpha$ for the stack, i meant that i prefer the old notation.}
\ryl{Okay, let's use the old notation}
%\ryl{Are $X^{(big,main)}$ and $X^{(main,big)}$ necessarily the same?}\mina{no they are not. They can be though (wouldn't hurt the construction)}
%\mina{since we have $X_{main}^{\alpha}$ for a node $\alpha$, and then we have things like $X^{(main,i)}$, maybe it's better to have $X_{(main,i)}$ instead? less confusing?}
%\ryl{I am in favor of this change. So then you have things like $X_{main,(main,i)}$ which looks ugly but might be clearer.}\mina{having three things in the subscript is confusing to me, not sure what you mean by it. what happens to $X^{(big,i)}$?}
%\ryl{I interpretted your suggestion to mean, for coordinate multi-array $X$, we index the coordinate arrays by $X_{(main/big,i)}$ rather than $X^{(main/big,i)}$. I was saying, in that case, since we name coordinate multi-arrays $X_{main},X_{t-2},\dots,X_1$ in the construction, then we have coordinate arrays such as $X_{t-2,(main,i)}$.}

%\ryl{You might be able to simplify this with just three coordinate arrays: $X^{main,big}$, $X^{main, extra}$, and $X^{big, extra}$, where $X^{main,extra}$ is compatible with all of $S^{main}$ and $S_2,\dots,S_{s-1}$. This ``merging of $X^{main,2},\dots,X^{main,k'-2}$'' only helps the YES case, and since $S_2,S_3,\dots,S_{s-1}$ have total size at most $k/2$, you are probably okay in the NO case. \ryl{Nevermind, I'm not sure this works}}
\end{definition}
%By $X^{(i,j)}[\ell]$ we mean the $\ell$th coordinate in the $X^{(i,j)}$ coordinate array. Also for a coordinate $c$ and a vector $a\in A$, $a[c]$ is the $c$th coordinate of $a$. 
\begin{definition}[Complement of coordinate multi-array]
For a coordinate multi-array $X$, let its \emph{complement} $\bar{X}$ be the coordinate multi-array with $\bar{X}^{(main,i)}=X^{(big,i)}$ for $i=1,\dots,k-2$ and $\bar{X}^{(big,i)}=X^{(main,i)}$ for $i=1,\dots,k-2$, and with $\bar X^{(main,big)}=\bar X^{(big,main)} = X^{(big,main)}$. In other words, we switch $X^{(big)}$ and $X^{(main)}$ and call the new coordinate multi-array $\bar{X}$. 
\end{definition}

\begin{definition}[Compatibility of a stack and a coordinate array]
Let $S=(a_1,\ldots,a_{s})$ be a stack where $|S|\le k-1$, and let $x\in[d]^{k-1}$ be a coordinate array.
%Let $S=(a_1,\ldots,a_{s})$ be a stack where $|S|=s\le k-1$ %\ryl{$s\le k-1$?} 
%and $X^{(i,j)}$ be a coordinate subsection where $i\in\{main,big\}$, $j\in \{1,\ldots,t-2,main,big\}$ and $i\neq j$. 
\begin{itemize}
\item We say that $S$ and $x$ are \emph{left-compatible}, if for all $h=1,\ldots,|S|$, we have $a_h[x[\ell]]=1$ for all $\ell=1,\ldots,k-|S|$.

\item We say that $S$ and $x$ are \emph{right-compatible}, if for all $h=1,\ldots,|S|$, we have $a_h[x[\ell]]=1$ for all $\ell=|S|,\ldots,k-1$.

\item We say that $S$ and $x$ are \emph{compatible} if they are either left-compatible or right-compatible. 
\end{itemize}

\end{definition}
\vvw{In the definition above, say that empty stacks are always compatible with any coordinate array.}

\begin{table}[!htb]
      \centering
         \begin{tabular}{|c|c |c|c| c|c| c| c|} 
 \hline
 %& $X^{(i,j)}[1]$ &$X^{(i,j)}[2]$ & $\ldots$ & $X^{(i,j)}[s]$ & $\ldots$& $X^{(i,j)}[k-2]$& $X^{(i,j)}[k-1]$\\ \hline
 & $x[1]$ &$x[2]$ & $\ldots$ & $x[k-s]$ & $\ldots$& $x[k-2]$& $x[k-1]$\\ \hline
 $a_1$ & $1$ &$1$ & $\ldots$ &  $1$&$\ldots$ & $1$ & $1$ \\ \hline
 $a_2$ & $1$ &$1$ & $\ldots$ & $1$& $\ldots$ & $1$ &  \\ \hline
 $\ldots$ & $\ldots$ &$\ldots$ & $\ldots$ & $\ldots$ & $\ldots$&&\\ \hline
 $a_{s}$ & $1$&$1$ & $\ldots$  &$1$ & & & \\ \hline
\end{tabular}

    \caption{Stack $S=(a_1,\dots,a_s)$ is left-compatible with $x$}
    \label{tab:left}
\end{table}
\begin{table}[!htb]
      \centering
         \begin{tabular}{|c|c |c|c| c|c| c| c|} 
 \hline
 %& $X^{(i,j)}[1]$ &$X^{(i,j)}[2]$ & $\ldots$ & $X^{(i,j)}[s]$ & $\ldots$& $X^{(i,j)}[k-2]$& $X^{(i,j)}[k-1]$\\ \hline
 & $x[1]$ &$x[2]$ & $\ldots$ & $x[s]$ & $\ldots$& $x[k-2]$& $x[k-1]$\\ \hline
 $a_1$ & $1$ &$1$ & $\ldots$ &  $1$&$\ldots$ & $1$ & $1$ \\ \hline
 $a_2$ &  &$1$ & $\ldots$ & $1$& $\ldots$ & $1$ & $1$  \\ \hline
$\ldots$  &  && $\ldots$ & $\ldots$ & $\ldots$&$\ldots$ &$\ldots$ \\ \hline
 $a_{s}$ & & & $\ldots$  &$1$ & $1$&$1$ & $1$ \\ \hline
\end{tabular}

    \caption{Stack $S=(a_1,\dots,a_s)$ is right-compatible with $x$}
    \label{tab:right}
\end{table}
\begin{definition}[Compatibility of a stack array and a coordinate multi-array]
We say that a stack array $(S_{t-1},S_{t-2},\ldots,S_{1},S_{0})$ and a coordinate multi-array $X$ are \emph{compatible}, if the following compatibility conditions are met:
\begin{itemize}
    \item For all $i\in\{1,\ldots,k',big\}$, $S_{t-1}$ and $X^{(main,i)}$ are compatible. 
    \item For all $i=main,1,\ldots,k'$, $S_{0}$ and $X^{(big,i)}$ are compatible. 
    \item For all $i=1,\ldots,t-2$, we have $S_i$ and $X^{(main,i)}$ are compatible.%\ryl{changed $s$ to $t$ here because $t$ describes the ``type'' of a stack array and $s$ describes the length of a stack.}
\end{itemize}
%Note that $X$ sees $S_{s-1}$ as the "main" stack and $S_{0}$ as the "big" stacks. \ryl{I mention this earlier when we define stack arrays}
\end{definition}

%\begin{definition}[Type-$t$ configuration]
%A \emph{type-$t$ configuration} $\alpha$ is a tuple $(\vec S, X_{main}^\alpha,X_{t-2}^\alpha,\dots,X_1^\alpha)$, consisting of a type-$t$ stack array and $t-1$ coordinate multi-arrays, such that the stack array $\vec S$ has weight $|\vec S|=k$.\ryl{I think it may be cleaner to define the graph in terms of configurations, and then say the nodes are the set of valid configurations.}
%%$(S_{big}^{\alpha})$ where $S_{big}^{\alpha}$ is a stack of size $k-1$. A type $t$ node $\alpha$ for $t\ge 2$ is of the form $(S_{main}^{\alpha},S_{t-2}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha}, X_{main}^{\alpha},X_{t-2}^{\alpha},\ldots,X_1^{\alpha})$, 
%%where $S_i^{\alpha}$'s are stacks containing vectors and $X_i^{\alpha}$'s are coordinate multi-arrays. We have that $|S_{big}^{\alpha}|+|S_{main}^{\alpha}|+\sum_{i}|S_i^{\alpha}|=k-t$ and, 
%We say that a type-$t$ configuration is \emph{valid} if
%\begin{itemize}
%    \item The stack array $\vec S=(S_{main}^{\alpha},S_{t-2}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha})$ is compatible with the coordinate multi-array $X^{\alpha}_{main}$. 
%    \item For all $i=1,\ldots,t-2$, the stack array $(S_{i}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha})$ is compatible with the coordinate multi-array $X_{i}^{\alpha}$. 
%    \item If $t\ge 3$, then $|S_{big}^{\alpha}|\ge \ceil{\frac{k-2}{2}}$.
%\end{itemize}
%\end{definition}



\subsection{The Vertex Set}
We are now ready to define the vertices of our graph $G$.
For $1\le t\le k'$, we construct \emph{type-$t$ vertices}, defined as follows:
a \emph{type-$t$ vertex} $\alpha$ is identified by a tuple $(\vec S^{\alpha}, X_{main},X_{t-2},\dots,X_1)$, consisting of a type-$t$ stack array $\vec S^{\alpha}=(S_{main}^{\alpha},S_{t-2}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha})$ and $t-1$ coordinate multi-arrays, such that the following conditions are satisfied:
%A \emph{type $1$ vertex} $\alpha$ is of the form $(S_{big}^{\alpha})$ where $S_{big}^{\alpha}$ is a stack of size $k-1$. A type $t$ node $\alpha$ for $t\ge 2$ is of the form $(S_{main}^{\alpha},S_{t-2}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha}, X_{main}^{\alpha},X_{t-2}^{\alpha},\ldots,X_1^{\alpha})$, 
%where $S_i^{\alpha}$'s are stacks containing vectors and $X_i^{\alpha}$'s are coordinate multi-arrays. We have that $|S_{big}^{\alpha}|+|S_{main}^{\alpha}|+\sum_{i}|S_i^{\alpha}|=k-t$ and, if $t\ge 3$, then 
%$|S_{big}^{\alpha}|\ge \ceil{\frac{k-2}{2}}$. 
%\ryl{We allow this to be violated when $t=2$, but since it is required when $t\ge 3$, we can only take the stack change edges when you have $S_{big}$ has more than half the elements}.\mina{for t=2, we have $|S_{main}|+|S_{big}|=k-2$, and since $S_{big}$ is the bigger one, we have $|S_{big}^{\alpha}|\ge \ceil{\frac{k-2}{2}}$. When do we violate it?}%\ryl{We don't require $S_{big}$ to be the biggest one when $t=2$. So $\alpha=(S_{main},\emptyset,X)$ is a vertex that has a weight-0 edge to $\bar \alpha = (\emptyset,S_{main},X)$. This makes it easier to describe the edges (in particular, there is no casework based on whether $k$ is even or odd). Furthermore, the existence of vertex $\alpha$ does not cause problems, because there are no stack change edges from it, only stack change edges from $\bar \alpha$, because if $\alpha$ did a stack change to get $\gamma$ of type-3, then $S_{big}^\gamma$ would be $\emptyset$ which is a contradiction.} \mina{okay I read the swap edge definition and I see where it comes from. If it helps with the NO case, I agree that we keep it (have to change the yes case a bit to comply with this, added a note for it) .}
%\mina{hmm so in the edge definition the only type1 type2 edges are these: from $(S_{big})$ you can just add a new $S_{main}$ which is empty, and add a coordinate. (then we won't need the $\alpha$ node you are suggesting.) I feel like with not having this condition, the name "big" is confusing, and I originally thought it actually helps to have this condition for $t=2$ to help the no case. If you're saying that it's actually not helpful, then we should change the "big" name. I'll add a note to check the yes case to comply with it.}  
\begin{itemize}
    \item The stack array $\vec S$ has weight $|\vec S|=k$.
    \item If $t\ge 3$, then $|S_{big}|\ge \ceil{\frac{k-2}{2}}$.
    \item The type-$t$ stack array $(S_{main}^{\alpha},S_{t-2}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha})$ and coordinate multi-array $X_{main}$ are compatible. 
    \item For all $i=1,\ldots,t-2$, the type-$i+1$ stack array $(S_{i}^{\alpha},\ldots,S_1^{\alpha},S_{big}^{\alpha})$ and the coordinate multi-array $X_{i}$ are compatible. 
\end{itemize}
The vertices of $G$ consist of all valid type-$t$ vertices, over all $1\le t\le k'$.
%\end{definition}
%\ryl{What is the reason we index them as $(S_{main},S_{t-2},\dots,S_1,S_{big})$ rather than than $(S_{t-1},\dots,S_0)$ and $(X_{main},X_{t-2},\dots,X_1)$ rather than $(X_{t-1},\dots,X_1)$. I could see an argument for why $S_{main}$ and $S_{big}$ are useful, but in the case of the coordinate arrays $X_{main},\dots,X_1$, it seems like $X_{t-1},\dots,X_1$ would be fine?} \mina{when you go from a type-2 node to a type-2 node, $X_{main}$ is the coordinate array staying with you if you don't change coordinates. That's the only reason, but if we want to change it we should change $S_{main}$ too cause their names should match (they get created and destroyed together)}
%\ryl{I see so it helps you reason about the yes case.}
%If $\alpha$ contains the two stacks $S$ and $S'$, we say that $S$ is higher than $S'$ (in the ordering) if in the ordering of stacks of $\alpha$, $S$ appears first. 

We say that $X_i$ belongs to $S_i$, for all $i\in \{main, big, 1,\ldots,t-2\}$ \ryl{can you check whether this is well defined? See the comment on Observation 1.1}, since $X_i$ sees $S_i$ as the "main" stack. We refer to $(S_{main}^{\alpha},S_{t-2}^{\alpha},\ldots,S_1^{\alpha}, S_{big}^{\alpha})$ as the stack array of $\alpha. $ \mina{should we delete this last sentence since you added it at the beginning?} We also refer to $S_i$ as the stack in position $i$ (of the stack array). Similarly, we refer to $X_i$ as the coordinate multi-array in position $i$. 

For a fixed $k$, we have at most $k'=k-\ceil{\frac{k-2}{2}}$ layers. \ryl{Is this ``layer'' the same as the ``layer'' two sentences later?}\mina{yes, although I just changed it to reflect the swap edges.} 

We say that a type-$t$ node $\alpha$ contains a stack $S$ if $S$ is one of its stacks. 

The graph $G$ has $\floor{\frac{k}{2}+1}$ layers. Layer $i$ has all the valid type-$t$  nodes $\alpha$ for $t\ge 3$, where $|S_{big}^{\alpha}|=k-i$. Moreover, layer $i$ has all the valid type $2$ nodes $\alpha$ where either $|S_{big}^{\alpha}|=k-i$ or $|S_{main}^{\alpha}|=k-i$.
%The vectors in stacks are from $A$. \ryl{We get this in the definition of stack}







\subsection{The Edge Set}
We now define the edges of $G$.
%For a stack $S$, let $S-1$ indicate that we remove the top vector in $S$ \mina{remove cause we have $popped(S)$?}. 
%We have two kinds of edges: the edges between two nodes of the same type, and the edges between two nodes of different types. 

\begin{enumerate}
\item \textbf{Vector change edges} (Type $t$ to type $t$ for $t\ge 2$) Let $t\ge 2$. For a vertex $\gamma=(S_{t-1}, S_{t-2},\dots,S_1, S_{0}, X_{main}, X_{t-2},\dots,X_1)$, a \emph{vector change} is the operation of first deleting the top element of either stack $S_{t-1}$ or stack $S_{t-2}$, then adding a vector to either stack $S_{t-1}$ or stack $S_{t-2}$ (possibly the same one)\TODO{example?}, and keeping the coordinate arrays $X_1,\dots,X_{main}$ and rest of the stacks $S_i$ for $i<t-2$ the same.
If $\gamma'$ can be obtained by applying a vector change to $\gamma$, then we add an edge between $\gamma$ and $\gamma'$.
Note that $\gamma'$ can be reached by applying a vector change to $\gamma$ if and only if $\gamma$ can be reached by applying a vector change to $\gamma'$.

%and $\gamma'=(S_{t-1}', S_{t-2}',\dots,S_1', S_{0}', X_{main}, X_{t-2},\dots,X_1)$ such that $S_i=S_i'$ for $i<t-2$, and the pair $(S_{t-1},S_{t-2})$

%Let $\gamma$ be a node. It is attached to any other node created by removing a vector from one of the top two stacks of $\gamma$, and putting a new vector in one of the top two stacks of $\gamma$. \mina{added the following} \ryl{I see so you change $X$ to $\bar X$ when you take the edge}\ryl{And the point is that, even though $X^{big}$ and $X^{main}$ are not symmetric in general, they are symmetric when there are only two stacks.}%\ryl{For ease of exposition, it may be easier to first write this as a ``weighted'' construction, where you put a weight 0 edge between $\alpha$ and $\beta$ if $\alpha=(S_1,S_2,X)$ and $\beta=(S_2,S_1,\bar X)$. Then you analyze the weighted construction, and then contract all the weight 0 edges for the final construction.}\mina{that's a good idea I'll apply this change.}
%\mina{added the zero edge as suggested.}
%The coordinate multi-arrays are the same between $\gamma$ and $\gamma'$, except for the following two case:  

%(1) If $k$ is odd, and $\gamma,\gamma'$ are both type $2$ nodes in layer $\frac{k+1}{2}$, and $\gamma'$ is created by removing one vector from the big stack of $\gamma$ and adding a vector to the main stack of $\gamma$, then if $X$ is the coordinate multi array of $\gamma$, $\bar{X}$ is the coordinate multi-array of $\gamma'$. This is because by removing an element from the big stack of $\gamma$, it becomes the main stack of $\gamma'$, so the order of the two stacks change, and hence we should change the corresponding order in the coordinate multi-array. More formally, let $\gamma=(S_{main}^{\gamma},S_{big}^{\gamma},X)$, and let $\gamma'=(S_{main}^{\gamma'}, S_{big}^{\gamma'},Y)$. Let $S_{big}^{\gamma}-1=S_{main}^{\gamma'}$ and $S_{big}^{\gamma'}-1=S_{main}^{\gamma}$. Then we have $Y=\bar{X}$.

%(2) If $k$ is even, then for any type 2 node $\gamma=(S_{big}^{\gamma},S_{main}^{\gamma},X)$, we connect $\gamma$ to $\gamma'=(S_{main}^{\gamma},S_{big}^{\gamma},\bar{X})$ with an edge of weight zero. Note that this edges is the only weighted edge in this construction.

%This summarizes all edges between nodes of the same type. By $S=S'$ for two stacks we mean that they have the same contents. 

\item \textbf{Swap edges} (Weight 0 type 2 to type 2) Let $S$ and $T$ be stacks and $X$ be a coordinate array such that $\alpha=(S_{main}^\alpha, S_{big}^\alpha,X^\alpha)$ is valid. Let $\bar\alpha$ denote the vertex $\bar \alpha=(S_{big}^\alpha,S_{main}^\alpha,\bar X^\alpha)$.
That is, $X^\alpha$ is replaced with $\bar X^\alpha$ and $S_{big}$ is swapped with $S_{main}$.
Connect $\alpha$ and $\bar\alpha$ by an edge of weight 0.
One can check that $\alpha$ is a valid vertex if and only if $\bar \alpha$ is valid, so every type-2 vertex has exactly one swap edge. 
\TODO{Check}
%\mina{has "exactly" one swap edge right?}\ryl{yes}

\item \textbf{Stack change edges}
Now let $\gamma=(S_{main}^{\gamma},S_{t-2}^{\gamma},\ldots,S_{1}^{\gamma},S_{big}^{\gamma},X_{main}^{\gamma},X_{t-2}^{\gamma},\ldots,X_{1}^{\gamma})$ be a valid type $t$ node. 
%\mina{for $t=2$, we must have $S_{big}\ge \ceil{(k-2)/2}$ (because $\gamma'$ is valid only in this case.)}\ryl{Added this at the bottom.}
Let $\gamma'=(S_{main}^{\gamma'},S_{t-1}^{\gamma'},\ldots,S_{1}^{\gamma'},S_{big}^{\gamma'},X_{main}^{\gamma'},X_{t-1}^{\gamma'},\ldots,X_{1}^{\gamma'})$ be a valid type $t+1$ node. Vertices $\gamma$ and $\gamma'$ are connected by an edge if either of the following conditions happen:

\begin{enumerate}
    \item \textbf{Inner stack change} If $\gamma'$ is created by removing the top vector of $S_{main}^{\gamma}$, and adding an empty stack between $S_{main}^{\gamma}$ and $S_{t-2}^{\gamma}$, hence in position $t-1$. For the coordinate multi-arrays, a new multi-array $X_{t-1}^{\gamma'}$ is added between $X_{main}^{\gamma}$ and $X_{t-2}^{\gamma}$, hence in position $t-1$. More formally, $S_{main}^{\gamma'}=S_{main}^{\gamma}-1$ \mina{$S_{main}^{\gamma'}=popped(S_{main}^{\gamma})$}, $S_{t-1}^{\gamma'}=\emptyset$, $S_{i}^{\gamma'} = S_{i}^{\gamma}$ for $i=1,\ldots,t-2$, and $S_{big}^{\gamma} = S_{big}^{\gamma'} $. We also have $X_{main}^{\gamma'}=X_{main}^{\gamma}$, $X_i^{\gamma'}=X_{i}^{\gamma}$ for $i=\{1,\ldots,t-2\}$. 
    \ryl{I think we also need that $S_{main}^\gamma$ is compatible with something}
    \item \textbf{Outer stack change} If $\gamma'$ is a node created by removing the top vector of $S_{main}^{\gamma}$, and adding an empty stack in position main. For the coordinate multi-arrays, a new multi-array $X_{main}^{\gamma'}$ is added in position $main$. More formally, $S_{main}^{\gamma'}=\emptyset$, $S_{t-1}^{\gamma'}=S_{main}^{\gamma}-1$ \mina{$S_{t-1}^{\gamma'}=popped(S_{main}^{\gamma})$}, $S_{i}^{\gamma'} = S_{i}^{\gamma}$ for $i=1,\ldots,t-2$, and $S_{big}^{\gamma} = S_{big}^{\gamma'} $. We also have  $X_{t-1}^{\gamma'}=X_{main}^{\gamma}$, $X_i^{\gamma'}=X_{i}^{\gamma}$ for $i=\{1,\ldots,t-2\}$. 
    \ryl{I think we also need that $S_{main}^\gamma$ is compatible with something}\mina{it should be compatible with the new coordinate in this case, which I was implying by with $\gamma'$ being "valid".}
\end{enumerate}
    Note that the edge exists between $\gamma$ and $\gamma'$ only if both are valid vertices. In particular, when $t=2$, the type-2 vertex $\gamma$ has incident stack change edges only when $|S_{big}^\gamma|\ge \ceil{(k-2)/2}$.

\item \textbf{Pseudo outer stack change.}
Let $t\ge 1$ and let $\gamma=(S_{main}^{\gamma},S_{t-1}^{\gamma},\ldots,S_{1}^{\gamma},S_{big}^{\gamma},X_{main}^{\gamma},X_{t-1}^{\gamma},\ldots,X_{1}^{\gamma})$ be a type $t+1$-vertex with $S_{main}^\gamma$ as the empty stack.
Let $\gamma'=(S_{main}^{\gamma},S_{t-1}^{\gamma},\ldots,S_{1}^{\gamma},S_{big}^{\gamma},Y_{main},X_{t-1}^{\gamma},\ldots,X_{1}^{\gamma})$ for some $Y_{main}\neq X_{main}$.
Connect $\gamma$ and $\gamma'$ by an edge. \mina{another name suggestion: coordinate change edge? not sure if it is more confusing than useful.}\ryl{I like Pseudo-outer stack change because in the No case, the outer stack change and pseudo-outer stack change play the same role, but if there's a good reason to change it in the yes case I'm fine with that.}\mina{no it's fine now i thought i'm gonna use it a lot but turns out not that much.}

%\ryl{This is a new edge. I think we need it for the No case, because if you start with a vertex with $S_{main}=\emptyset$, it seems like you can't do the stack change you want to change $X_{main}$. This seems consistent with our 4-OV, 5-OV, 6-OV constructions, where you need a coordinate change at the highest types. Is there any way to get around this? Hopefully it doesn't affect the Yes case.}\mina{yes you're right we need it, and no it shouldn't affect the yes case, i'll check.}

\end{enumerate}

%the node created by adding a new stack between $S_{main}^{\gamma}$ and $S_{1}^{\gamma}$ (as $S_1^{\gamma'}$), removing the top vector of $S_{main}$ and by adding a corresponding coordinate between $X_{main}^{\gamma}$ and $X_1^{\gamma}$. 

%In other words let $\gamma'=(S_{main}^{\gamma}-1,S_1,S_1^{\gamma},\ldots,S_{t-2}^{\gamma},X_{main}^{\gamma}, X_1,X_1^{\gamma},\ldots,X_{t-2}^{\gamma})$.


Note that if $t=1$, then $\gamma=(S_{big})$ is attached to $\gamma'=(S_{main},S_{big}-1, X)$ where $S_{main}$ is an empty stack, and $\gamma'$ is a valid type $2$ node. Since all type $1$ nodes have one stack, we don't have any edges inside layer $1$. When going from a type $t+1$ node to a type $t$ node, we say that the stack $S_1$ ($S_{main}$ in the second case) gets "deleted". Also note that the coordinate multi-arrays belonging to any stack remains the same. So we have the following observation:
\begin{observation}
A stack and a coordinate multi-array belonging to it are created and deleted at the same time.\ryl{What happens when you have $(S_{main}, S_{big}, X)$ becomes $(S_{big}, S_{main}, \bar X)$? Then $X$ ``belongs'' to $S_{main}$ in the first case, but it ``belongs'' to $S_{big}$ in the second case, so then they may not get created and deleted at the same time. If we want to be precise about this, it may be better to write nodes as $((S_{main}, X_{main}), \cdots (S_1,X_1), S_{big})$, but that may make other parts more clumsy.}\mina{you're right, what if we say that a coordinate multi-array $X_i$ belongs to both $S_{big}$ and $S_i$. Then a coordinate multi-array is deleted if and only if one of the stacks it belongs to gets deleted. This is basically what I use in the yes case. And maybe we need a lemma for this to explain it more?}\ryl{I think this works. I agree it would be nice if we had a lemma justifying this. Also maybe you can move this to the Yes case? We don't need this observation for the No case.}
\end{observation}

%\paragraph{Dual Representation} 
%Let $k$ be even, and let $\gamma$ be a type $2$ node in layer $\frac{k}{2}+1$. Then both of the stacks of $\gamma$ have $\frac{k-2}{2}$ nodes. So in this case, for any representation of $\gamma=(S_1,S_2,X)$ which is valid, we have another equivalent representation: $(S_2,S_1,\bar{X})$. Now for any $\gamma\gamma'$ edge, depending on the big stack of $\gamma'$, one of the representations fits the definitions. \mina{not sure if this sentence helps or is more confusing. }One can think of the dual representation of a node, as two nodes being attached by a 0 weighted edge. 
%\ryl{I think it will be easier to simply state the construction with weight 0 edges, and then say afterwards we can contract them.}

%We refer to $X$ and $\bar{X}$ as the same coordinate multi-array.

%\ryl{What does this mean? Are $X$ and $\bar X$ are interchangable, so that when you say ``$(S,\dots,)$ is compatible with $X$'' you really mean ``$(S,\dots,)$ is compatible with either $X$ or $\bar X$''? If not then I am confused as to how you define this. If they are interchangable in the above sense, then I am concerned about the YES case.
%
%It would help if you included this in the definition of the edges and vertices, since I don't see where to add $\bar X$ into the definition.}\mina{this sentence is very misleading, i'll remove it. Added the switch edge for odd case above in the definition of the edges.}\ryl{Okay, it makes sense now, thanks.}


\mina{some ideas:} motivation for this construction: start from having only type 1 and type 2 nodes like previous constructions, and argue that you need type 3 nodes in the no case to go from a type 1 to a type 2 node.
\ryl{Additional motivation: need to make sure you can't drop $a_1$ or $a_k$ in less than $k-1$ steps.}
\ryl{Additional motivation: need to make sure you can't do $a_1,\dots,a_{k-1}$ to $(a_1,\dots,a_{k/2}), (1,1,\dots,1)$ to $(a_k,\dots,a_{k/2}),(1,\dots,1)$ to $(a_k,\dots,a_3)$.}
\subsection{Other Definitions\mina{moved to the yes case}}










==> prior_construction/nocase.tex <==
\section{No case \ryl{Sorta done}}
\ryl{Sorry I haven't gotten to proofreading this yet}
\ryl{I haven't gotten to this yet because I've spent much of my time trying to find a simpler construction, but many attempts have failed.}

Assume that any $k$ vectors from a set $A$ are orthogonal.
Given at most $k$ orthogonal vectors $a_1,\dots,a_k$, let $ind(a_1,\dots,a_k)$ denote some $x\in[d]$ such that $a_1[d]=\cdots=a_k[d]=1$.
We first establish some lemmas about coordinate arrays.

\begin{lemma}
  \label{lem:stack-1}
  If stack $S$ is compatible with a coordinate array $X$, then any substack of $S$ is compatible with $X$ as well.
\end{lemma}
\begin{proof}
  This follows from the definition of compatibility.
\end{proof}

\begin{lemma}
  \label{lem:stack-2}
  Let $S=(a_1,\dots,a_{|S|})$ and $S'=(b_1,\dots,b_{|S'|}$ be stacks, each with at most $k-1$ vectors from $A$.  Then there exists a coordinate array $X$ such that $S$ and $S'$ are both compatible with $X$.
\end{lemma}
\begin{proof}
  By Lemma~\ref{lem:stack-1}, it suffices to prove this in the case that $|S|=|S'|=k-1$.
  Then $S=(a_1,\dots,a_{k-1})$ and $S'=(b_1,\dots,b_{k-1})$.
  Let $X[\ell]=ind(a_1,\dots,a_{k-\ell},b_1,\dots,b_\ell)$.
  Then for all $h=1,\dots,k-1$, we have $a_h[X[\ell]]=1$ for $\ell\le k-h$, so $S$ is left-compatible with $X$.
  Additionally, for all $h=1,\dots,k-1$, we have $b_h[X[\ell]]=1$ for $\ell=h,\dots,k-1$ so $S'$ is right-compatible with $X$.
  Hence, both $S$ and $S'$ are compatible with $X.$
\end{proof}
%Since any $k$ vectors in $A$ are orthogonal, we can apply Lemma~\ref{lem:stack-2} to any stacks of at most $k-1$ vectors from $A$.
%\begin{corollary}
  %\label{cor:stack-2}
  %Let $S$ and $S'$ be stacks of vectors from $A$ with at most $k-1$ vectors each.
  %Then there exists a coordinate array $X$ compatible with each of $S$ and $S'$.
%\end{corollary}

\begin{lemma}
  Suppose that $t\ge 3$ and the stack array $(S_{t-1},S_{t-2},\dots,S_1,S_{big})$ is compatible with the coordinate multiarray $Z$, and $T$ is compatible with the coordinate multiarray $Z^{main,i}$ for $i=big,1,\dots,k'$.
  Then the stack array $(T, S_{t-3},\dots,S_1,S_{big})$ is also compatible with the coordinate multiarray $Z$.
\label{lem:stack-2.5}
\end{lemma}
\begin{proof}
  Since $(S_{t-1},S_{t-2},\dots,S_1,S_{big})$ is compatible with $Z$, we have
  \begin{itemize}
  \item For all $i=1,\dots,k',main$, $S_{big}$ and $Z^{(big,i)}$ are compatible.
  \item For all $i=1,\dots,t-2$, $S_i$ and $Z^{(main,i)}$ are compatible.
  \end{itemize}
  Additionally, we have by the lemma condition,
  \begin{itemize}
  \item For all $i=big,1,\dots,k'$, $T$ and $Z^{(main,i)}$ are compatible.
  \end{itemize}
  By definition of compatibility of a stack array and coordinate multi-array, this means that the stack array $(T,S_{t-3},\dots,S_1,S_{big})$ is also compatible with $Z$.
\end{proof}

\begin{lemma}
  Let $S'$ be a substack of stack $S$ and $T'$ be a substack of stack $T$ such that $\gamma_1=(S',T,X)$ and $\gamma_2=(S,T',X)$ are both type-2 vertices.
  Then there is a length $|S|-|S'|=|T|-|T'|$ path from $\gamma_1$ to $\gamma_2$.
  Similarly, if $\gamma_2'=(T',S,\bar X)$, there is a length $|S|-|S'|$ path from $\gamma_1$ to $\gamma_2$.
\label{lem:stack-3}
\end{lemma}
\begin{proof}
  Clearly we always have $|S'|+|T|=|S|+|T'|=k-2$ so always $|S|-|S'|=|T|-|T'|$.
  %We prove by induction on $|S|-|S'|$.
  %In the base case, $|S|-|S'|=0$, there is nothing to prove as $S'=S$ and $T'=T$.
  %Now suppose $|S|-|S'|>0$.
  Suppose that $S$ has length $\ell$ and $S'=S_{\le \ell'}$, so that $T$ has length $k-2-\ell'$ and $T'$ has length $k-2-\ell$.
  For $i=\ell',\dots,\ell$, let $\delta_i$ be the vertex $(S_{\le i}, T_{\le k-2-i},X)$, so that $\delta_i = \gamma_1$ and $\delta_\ell=\gamma_2$.
  Since $\gamma_1$ and $\gamma_2$ are vertices, we know that $S$ and $T$ are both compatible with the coordinate array $X$, so by Lemma~\ref{lem:stack-1}, all of $S_{\le i}$ and $T_{\le k-2-i}$ for $i=\ell',\dots,\ell$ are compatible with the coordinate array $X$.
  Hence, $\delta_{\ell'},\dots,\delta_{\ell}$ are all valid vertices.
  Additionally, by vector changing edges, $\delta_i$ and $\delta_{i+1}$ are adjacent for all $i=\ell',\dots,\ell-1$, so $\delta_{\ell'},\dots,\delta_\ell$ is a valid path of length $\ell-\ell'=|S|-|S'|$ from $\gamma_1$ to $\gamma_2$ as desired.
  The second part follows from the fact that $\gamma_2$ and $\gamma_2'$ are connected by a weight 0 edge.
\end{proof}
\begin{lemma}
  \label{lem:stack-4}
  Let $t\ge 1$ and let $\alpha=(S_t, S_{t-1},\dots,S_1,S_{big},Z,X_{t-1},\dots,X_1)$ be a valid type-$t+1$ vertex. \TODO{Notation, $S_t$ is $S_{main}$.}
  Let $\gamma=(T,S_{big},Z)$ be a valid type-2 vertex such that $S_t$ is a substack of $T$.
  Then the distance between vertices $\alpha$ and $\gamma$ is at most $|T|-|S_t|$.
\end{lemma}
\begin{proof}
  If $t=1$, then we must have $|S_t|=k-2-|S_{big}|$ by definition of a type-2 vertex, so $S_t=T$ and thus $\alpha=(T,S_{big}, Z)=\gamma$, so they are distance $0=|T|-|S_t|$ as desired.

  We prove by induction on $t$, and then by induction on $|S_{t-1}|$.
  The base case $t=1$ is already proven.
  Suppose $t\ge 2$, and $T=(a_1,\dots,a_{k-2-|S_{big}|})$ and $S_t = T_{\le \ell} = (a_1,\dots,a_\ell)$.
  Suppose as an inductive hypothesis that the lemma is true when for smaller values of $t$, or for the same value of $t$ but with $|S_{t-1}|$ smaller.
  There are two cases in the inductive step.
  
  \textbf{Case 1. $|S_{t-1}|=0$.}
  Let $S_{t-1}' = T_{\le \ell+1} = S_{t-1}+ a_{\ell+1}$.
  Let $\beta$ denote the type-$t$ vertex $(S_{t-1}', S_{t-2},\dots,S_1,S_{big}, Z, X_{t-2},\dots,X_1)$.

  We check that $\beta$ is a valid type-$t$ vertex. Indeed, since $\gamma$ is valid, we have $T$ is compatible with $Z^{main,i}$ for $i=big,1,\dots,k'$, so by Lemma~\ref{lem:stack-1}, $S_{t-1}'$ is compatible with $Z^{main,i}$ for $i=big,1,\dots,k'$.
  Hence, by Lemma~\ref{lem:stack-2.5}, $(T,S_{t-2},\dots,S_1,S_{big})$ is compatible with $Z$.
  We also have $(S_{t'},\dots,S_1,S_{big})$ is compatible with $X_{t'}$ for $1\le t'\le t-2$, so indeed $\beta$ is a valid vertex.

  We now claim that $\alpha$ and $\beta$ are connected by an inner stack-change edge.
  The can be done by checking the following properties of $\alpha$ and $\beta$.
  \begin{itemize}
  \item $\alpha$ is a valid type-$t+1$ vertex (by the lemma's hypothesis)
  \item $\beta$ is a valid type-$t$ vertex by the previous paragraph
  \item $S_{t-1}^\alpha=\emptyset$.
  \item $S_{main}^\alpha = popped(S_{main}^\beta)$.
  \item $S_i^\alpha = S_i^\beta$ for $i=big, 1,\dots,t-2$.
  \item $X_{main}^\alpha =X_{main}^{\beta}=Z$.
  \item $X_i^\alpha=X_i^\beta$ for $i=1,\dots,t-2$.
  \end{itemize}

  Since $S_{t-1}'$, which is $S_{main}^\beta$, is a substack of $T$, and $\beta$ is a valid vertex, we have $\beta$ satisfies the setup of the Lemma with a $t$-parameter of $t-1$.
  Hence, we may apply the inductive hypothesis to obtain that the distance from $\beta$ to $\gamma$ is at most $d(\beta,\gamma)\le |T|-|S_{t-1}'| = |T|-|S_t|-1$.
  We showed that $\alpha$ and $\beta$ are adjacent by an inner stack-change edge, so $d(\alpha,\beta)=1$.
  Hence,  $d(\alpha,\gamma)\le |T|-|S_t|-1+1=|T|-|S_t|$, as desired.

  \textbf{Case 2. $|S_{t-1}|>0$}.
  Let $S_t'=T_{\le \ell+1}=T_{\le \ell}+a_{\ell+1}$ and $S_{t-1}'=popped(S_{t-1})$.
  Let $\beta$ denote the type-$t+1$ vertex $(S_t',S_{t-1}',S_{t-2},\dots,S_1,S_{big},Z,X_{t-1},\dots,X_1)$.
  We can check that $\beta$ is a valid vertex. We first check that $S_{t-1}'$ is compatible with coordinate arrays $X_{t-1}^{main,i}$ for $i=big,1,\dots,k'$, which is true by Lemma~\ref{lem:stack-1} since $S_{t-1}'$ is a substack of $S_{t-1}$ and stack $S_{t-1}$ is compatible with coordinate arrays $X_{t-1}^{main,i}$ for $i=big,1,\dots,k'$.
  We then check that $S_{t}'$ is compatible with coordinate arrays $Z^{main,i}$ for $i=big,1,\dots,k'$, which is true by Lemma~\ref{lem:stack-1} because $T$ is compatible with all such coordinate arrays since $\gamma$ is a valid vertex, and $S_t'$ is a substack of $T$.
  We also know that $\alpha$ and $\beta$ are adjacent by a vector-change edge.

  Also $S_t'$, which is $S_{main}^\beta$, is a substack of $T$, and $\beta$ is a valid vertex, we have that $\beta$ satisfies the setup of the lemma with $|S_{t-1}'|<|S_{t-1}|$.
  Hence, we may apply the inductive hypothesis to obtain that the distance from $\beta$ to $\gamma$ is at most $d(\beta,\gamma)\le |T|-|S_t'| = |T|-|S_t|-1$.
  We showed that $\alpha$ and $\beta$ are adjacent by an vector-change edge, so $d(\alpha,\beta)=1$.
  Hence,  $d(\alpha,\gamma)\le |T|-|S_t|-1+1=|T|-|S_t|$, as desired.

  This covers all cases, proving the inductive step, and completing the induction, proving Lemma~\ref{lem:stack-4}.
\end{proof}


\begin{lemma}
  Let $t\ge 2$ and let $\alpha=(S_{t-1},\dots,S_1, S_{big},X_{main},X_{t-2},\dots,X_1)$ be a type-$t$ vertex, and let $T$ be a stack of size $k-2-|S_{big}|$, and let $Z$ be a coordinate array such that $\gamma=(T,S_{big},Z)$ is a valid type-2 vertex, and such that $Z^{main,i}$ is compatible with $S_i$ for $i=1,\dots,t-1$.
  Then $\alpha$ is at distance $|T|+1$ from the vertex $\gamma=(T,S_{big},Z)$.
  \label{lem:stack-6}
\end{lemma}
\begin{proof}
  We consider two cases based on $S_{t-1}$.

  \textbf{Case 1.} $S_{t-1}=\emptyset$.
  Let $\alpha'$ denote the vertex $\alpha'=(S_{t-1},\dots,S_1,S_{big}, Z, X_{t-2},\dots,X_1)$, which has the same stacks as $\alpha$ and the same coordinate arrays as $\alpha$ except for $X_{main}^{\alpha'}$, which is $Z$.
  We have that $\alpha'$ is a valid vertex, because $\alpha$ is valid and because $Z$ is compatible with the stack array $(S_{t-1},\dots,S_1,S_{big})$ (recall $S_{t-1}$ is empty).
  We have that $\alpha'$ and $\alpha$ are adjacent by a pseudo-outer-stack change edge.
  Then we have that $\alpha'$ and $\gamma$ satisfy the setup of Lemma~\ref{lem:stack-4}, as $S_{t-1}$, an empty stack, is trivially a substack of $T$, and by this lemma's assumptions we have $\gamma$ is a valid vertex.
  Hence, by Lemma~\ref{lem:stack-4}, we have $d(\alpha',\gamma)\le |T|$, so by the triangle inequality $d(\alpha,\gamma)\le d(\alpha,\alpha') + d(\alpha',\gamma) \le |T|+1$.

  \textbf{Case 2.} $S_{t-1}$ is nonempty.
  Let $\alpha'$ denote the vertex $\alpha'=(\emptyset, popped(S_{t-1}),S_{t-2},\dots,S_1,S_{big}, Z, X_{main},X_{t-2},\dots,X_1)$, which has the same stacks as $\alpha$ and the same coordinate arrays as $\alpha$ except for $X_{main}^{\alpha'}$, which is $Z$.
  We have that $\alpha'$ is a valid vertex because $\alpha$ is and because $Z$ is compatible with the stack array $(\emptyset, popped(S_{t-1}),S_{t-2},\dots,S_1,S_{big})$: the ``main'' stack is empty and $Z^{main,i}$ is compatible with $S_i$ for $i=1,\dots,t-1$.\TODO{}

  We can also check that that $\alpha'$ and $\alpha$ are adjacent by an outer-stack change edge. Indeed $S_{main}^{\alpha'}=\emptyset$, $S_{t-1}^{\alpha'} = popped(S_{t-1}^{\alpha})$, and $S_i^{\alpha'}=S_i^{\alpha}$ for $i=big, 1,\dots,t-2$.  We also have $X_{t-1}^{\alpha'}=X_{main}^{\alpha}$ and $X_i^{\alpha'}=X_i^{\alpha}$ for $i=1,\dots,t-2$.
  And we just showed that $\alpha'$ is a valid type-$t+1$ vertex.

  Now we have that $\alpha'$ and $\gamma$ satisfy the setup of Lemma~\ref{lem:stack-4}, as $S_t^{\alpha'}$, an empty stack, is trivially a substack of $T$, and by this lemma's assumptions we have $\gamma$ is a valid vertex.
  Hence, by Lemma~\ref{lem:stack-4}, we have $d(\alpha',\gamma)\le |T|$, so by the triangle inequality $d(\alpha,\gamma)\le d(\alpha,\alpha') + d(\alpha',\gamma) \le |T|+1$.
\end{proof}

Let $\alpha$ and $\beta$ be vertices of type $t_\alpha$ and $t_\beta$ respectively.
Then $\alpha=(S_{t_\alpha-1}, S_{t_\alpha-2},\dots,S_1, S_{big}, X_{t-1},\cdots,X_1)$ and $\beta=(T_{t_\beta-1},T_{t_\beta-2},\dots,T_1, Y_{main},\dots, Y_1)$.
Note that if $\alpha$ is type-1, then $\alpha$ is simply a stack $(S_{big})$, and if $\beta$ is type-1, then $\beta$ is simply a stack $T_{big}$.

By construction $|S_{big}|,|T_{big}|\ge \frac{k-2}{2}$.
Let $S_{big}'$ be the size-$k-2-|T_{big}|$ substack of $S_{big}$, and let $T_{big}'$ be the size $k-2-|S_{big}|$ substack of $T_{big}$.


\textbf{Defining $Z$.}
We first describe a coordinate multiarray $Z$ that is important to the path from $\alpha$ to $\beta$, by specifying the individual coordinate arrays $Z^{main,i}$ and $Z^{big,i}$.
We specify these coordinate arrays by repeatedly applying Lemma~\ref{lem:stack-2}. 
\begin{enumerate}
\item Let $Z^{main,big}=Z^{big,main}$ be the coordinate array compatible with $S_{big}$ and $T_{big}$.
\item For $i=1,\dots,k'-2$, $Z^{main,i}$ be the coordinate array compatible with $T_{big}$ and, if $S_i$ exists, with $S_i$.
\item For $i=1,\dots,k'-2$, $Z^{big,i}$ be the coordinate array compatible with $S_{big}$ and, if $T_i$ exists, with $T_i$.
\end{enumerate}
\TODO{compatibility diagram, which stacks are compatible with which coordinates}

\begin{lemma}
  If $t_\alpha\ge 2$, there exists a type-2 vertex $\gamma_1=(T_{big}', S_{big}, Z)$ such that $T_{big}'$ is a substack of $T_{big}$, and the distance from $\alpha$ to $\gamma_1$ is $|T_{big}'|+1$. 
\label{lem:stack-7}
\end{lemma}
\begin{proof}
  Let $T_{big}'$ denote the bottom $k-2-|S_{big}|$ elements of $T_{big}$.
  Then $\alpha$ and $\gamma_1$ satisfy the setup of Lemma~\ref{lem:stack-6}, so $d(\alpha,\gamma_1)=|T_{big}'|+1$.
%
  %Let $\gamma$ denote the type-$t+1$ vertex $(S_{t_\alpha}',S_{t_\alpha-1}',\dots,S_1',S_{big},Z, X_{t-1}, X_{t-2},\dots,X_1)$, where $X_{t-1},\dots,X_1$ \ryl{TODO, indexing problems if $t_\alpha=1$} are the same as in vertex $\alpha$,where $S_{t_\alpha}$ is an empty stack, $S_{t_\alpha-1}=popped(S_{t_\alpha-1})$, where $S_{t'}'=S_{t'}$ for $0\le t'\le t_\alpha-2$, and where $Z$ is the coordinate array defined above.
%
  %Let $\alpha'$ denote the vertex $(T_{big}', S_{big}, Z)$.
%
  %\TODO{Check that $\gamma$ and $\alpha'$ are valid vertices.}
%
  %\begin{enumerate}
  %\item The total size of the stacks in $\gamma_1$ is $|S_{big}'|+|T_{big}| = k-2$. Similarly, the total size of the stacks in $\gamma_2$ is $k-2$.
  %\item Since $T_{big}'$ is a substack of $T_{big}$ and $T_{big}$ is compatible with $Z^{main,i}$ for all $i$ by definition of $Z$, we have by Lemma~\ref{lem:stack-1} that $T_{big}'$ is compatible with $Z^{main,i}$ for all $i\in\{big,1,\dots,k'-2\}$. 
  %\item Additionally $S_{big}$ is compatible with $Z^{big,i}$ for all $i\in\{main, 1,\dots,k'-2\}$.
  %\item We conclude $(T_{big}', S_{big})$ is compatible with coordinate multi-array $Z$, so $\gamma_1$ is a valid vertex.
  %\item Since $S_{big}'$ is a substack of $S_{big}$ and $S_{big}$ is compatible with $Z^{big,i}$, and thus $\bar Z^{main,i}$ for all $i$ by definition of $Z$, we have by Lemma~\ref{lem:stack-1} that $S_{big}'$ is compatible with $\bar Z^{main,i}$ for all $i$.
  %\item Additionally, $T_{big}$ is compatible with $Z^{main,i}$ for all $i=big,1,\dots,k'-2$, and thus $Z^{big,i}$ for all $i=main,1,\dots,k'-2$.
  %\item We conclude that $(S_{big}', T_{big})$ is compatible with coordinate multi-array $Z$, so $\gamma_2$ is a valid vertex.
  %\end{enumerate}
%
  %\TODO{verify that $\alpha$ is adjacent to $\gamma$}
%
  %\TODO{Apply Lemma~\ref{lem:stack-4}}
\end{proof}
\begin{lemma}
  If $t_\beta\ge 2$, there exists a type-2 vertex $\gamma_2=(S_{big}', T_{big}, \bar Z)$ such that $S_{big}'$ is a substack of $S_{big}$, and the distance from $\beta$ to $\gamma_2$ is $|S_{big}'|+1$.
\label{lem:stack-8}
\end{lemma}
\begin{proof}
  Let $S_{big}'$ denote the bottom $k-2-|T_{big}|$ elements of $S_{big}$.
  We have that $\gamma_2$ is a valid vertex by definition of $Z$.
  We also have by definition of $Z$ that for $i=1,\dots,t-2$, the coordinate array $\bar Z^{main,i}=Z^{big,i}$ is compatible with $S_i$.
  Then $\beta$ and $\gamma_2$ satisfy the setup of Lemma~\ref{lem:stack-6}, so $d(\beta,\gamma_2)=|S_{big}'|+1$.
%
%
%Let $\gamma$ denote the type-$t+1$ vertex $(T_{t_\beta},pop(T_{t_\beta-1}), T_{t_\beta-2},\dots,T_1,T_{big},Z, Y_{t-1}, Y_{t-2},\dots,Y_1)$, where $T_{t_{\beta}-1},\dots,T_1,T_{big},Y_{t-1},\dots,Y_1$ are the same as in vertex $\beta$, where $T_{t_\beta}$ is an empty stack, and where $Z$ is the coordinate array defined above.
%
  %Let $\beta'$ denote the vertex $(S_{big}',T_{big}, \bar Z)$.
%
  %\TODO{Check that $\gamma$ and $\beta'$ are valid vertices.}
%
  %\TODO{verify that $\beta$ is adjacent to $\gamma$}
%
  %\TODO{Apply Lemma~\ref{lem:stack-4}}
\end{proof}

%\textbf{Validity of $\alpha',\beta',\gamma_1,\gamma_2$.}
%We check that $\alpha', \beta'$, $\gamma_1$, and $\gamma_2$ are valid vertices:


%\textbf{Verifying $\alpha$ ($\beta$) is adjacent to $\alpha'$ ($\beta'$).}
%We now check that $\alpha$ is adjacent to $\alpha'$ and $\beta$ is adjacent to $\beta'$.
%\TODO{Do we need to be careful about stating type-1 to type-2 edges.}


If $t_\alpha\ge 2$, let $\alpha'=(T_{big}',S_{big},Z)$ be as in Lemma~\ref{lem:stack-7}.
Otherwise, let $\alpha'=(T_{big}', popped(S_{big}), Z)$ where $T_{big}'$ is the empty stack. 
If $t_\beta\ge 2$, let $\beta'=(S_{big}',T_{big}, Z)$ be as in Lemma~\ref{lem:stack-8}.
Otherwise, let $\beta'=(S_{big}', popped(T_{big}), \bar Z)$, where $S_{big}'$ is the empty stack.

We now finish the proof by showing there is a path from $\alpha$ to $\beta$ through $\alpha',\beta'$.
We consider four cases.

\textbf{Case 1. $t_\alpha,t_\beta\ge 2$}
By Lemma~\ref{lem:stack-3}, we have that the distance from $\alpha'$ to $\beta'$ satisfies
\begin{align}
  d(\alpha',\beta') \le |S_{big}|-|S_{big}'|.
\label{lem:no-dist-1}
\end{align}
Additionally, by Lemma~\ref{lem:stack-7} and Lemma~\ref{lem:stack-6}, we have
\begin{align}
  d(\alpha,\alpha')&\le |T_{big}'|+1, \nonumber\\
  d(\beta,\beta')&\le |S_{big}'|+1.
\end{align}
By the triangle inequality,
\begin{align}
  d(\alpha,\beta)
  \ &\le \ d(\alpha,\alpha')+d(\alpha',\beta')+d(\beta',\beta) \nonumber\\ 
  \ &\le \ (|S_{big}'|+1) + (|S_{big}|-|S_{big}'|) + (|T_{big}'|+1)\nonumber\\
  \ &= \  2+|S_{big}'| + |T_{big}| = k.
\end{align}

\textbf{Case 2. $t_\alpha=1, t_\beta\ge 2$.}
We have $\alpha' = (\emptyset, popped(S_{big}), Z)$ and $\beta'=(S_{big}', T_{big},\bar Z)$.
We have $\alpha$ and $\alpha'$ are adjacent by an outer-stack-change edge.
By Lemma~\ref{lem:stack-3}, we have that the distance from $\alpha'$ to $\beta'$ satisfies
\begin{align}
  d(\alpha',\beta') \le |popped(S_{big})|-|S_{big}'| = k-2-|S_{big}'|
\end{align}
Additionally, by Lemma~\ref{lem:stack-8}, we have
\begin{align}
  d(\beta,\beta')&\le |S_{big}'|+1.
\end{align}
By the triangle inequality,
\begin{align}
  d(\alpha,\beta)
  \ &\le \ d(\alpha,\alpha')+d(\alpha',\beta')+d(\beta',\beta) \nonumber\\ 
  \ &\le \ 1 + (k-2-|S_{big}'|) + (|S_{big}'|+1) = k.
\end{align}

\textbf{Case 3. $t_\alpha=2, t_\beta\ge 1$.} Analogous to previous one

\textbf{Case 4. $t_\alpha= t_\beta= 1$.}
We have $\alpha' = (\emptyset, popped(S_{big}), Z)$ and $\beta'=(\emptyset, popped(T_{big}),\bar Z)$.
We have $\alpha$ and $\alpha'$ are adjacent by an outer-stack-change edge.
We also have $\beta$ and $\beta'$ are adjacent by an outer-stack-change edge.
\begin{align}
  d(\alpha',\beta') \le |popped(S_{big})|-|\emptyset| = k-2.
\end{align}
By the triangle inequality,
\begin{align}
  d(\alpha,\beta) &\le  
  d(\alpha,\alpha')+d(\alpha',\beta')+d(\beta',\beta) \le 1 + (k-2) + 1 = k. 
\label{}
\end{align}

This covers all cases of vertices $(\alpha,\beta)$, so for any two vertices $\alpha,\beta$ we have $d(\alpha,\beta)\le k$, so the diameter is at most $k$. This proves that when $A$ does not have $k$ orthogonal vectors, the diameter of the constructed graph $G$ is at most $k$.

%Vertices $\alpha'=(S_t',\dots,S_1',S_{big}',Z,X_{t-1},\dots,X_1)$ and $\gamma_1=(T_{big}',S_{big},Z)$ satisfy the setup of Lemma~\ref{lem:stack-4}, as they are both valid vertices, verified above, and $S_t'$ is the empty stack and thus trivially a substack of $T_{big}'$.
%Then by Lemma~\ref{lem:stack-4}, we have that the distance from $\alpha'$ to $\gamma_1$ satisfies.
%\begin{align}
  %d(\alpha',\gamma_1)\le |T_{big}'|-|S_t'| = |T_{big}'|.
%\end{align}
%Similarly, vertices $\beta'=(T_t',\dots,T_1',T_{big}',Z,Y_{t-1},\dots,Y_1)$ and $\gamma_1=(S_{big}',T_{big},Z)$ satisfy the setup of Lemma~\ref{lem:stack-4}, as they are both valid vertices, verified above, and $S_t'$ is the empty stack and thus trivially a substack of $T_{big}'$.



%To prove that $\alpha$ and $\beta$ are distance at most $k$, it suffices to prove the following claim.
%\begin{claim}
  %The vertex $\alpha$ is distance $k-1-|S_{big}|$ from $\gamma_1$.
  %The vertex $\beta$ is distance $k-1-|T_{big}|$ from $\gamma_2$.
  %There exists a coordinate multiarray $Z$ such that the vertex $\gamma=(S_{big}', T_{big}', Z)$ is distance $1+\floor{(k-2)/2}$ from $\alpha$ and distance at most $1+\ceil{(k-2)/2}$ from $\beta$. In $\gamma$, $S_{big}'$ is the ``main'' stack and $T_{big}'$ is the ``big'' stack.
%\end{claim}
%\begin{proof}
  %Let $r_1$
%\end{proof}









==> prior_construction/yescase.tex <==

\section{Yes case } 
%\mina{todo: make it compatible with having a zero weight edge instead of dual representation.}
%\mina{todo: apply $X^{main,big}=X^{big,main}$}
%\mina{todo:check pseudo outer stack change: you delete a stack, or you empty it and do pseudo outer stack change: same cost.}
\mina{todo: check "belonging" parts }\mina{todo: use the substack notation.} Suppose that $A$ is a YES $k$-OV instance, where $a_1,\ldots,a_k$ are orthogonal. We are going to argue that $\alpha=(C_0)$ and $\beta=(C_1)$ are at least $2k-1$ far, where $C_0=(a_1,\ldots,a_{k-1})$ and $C_1 = (a_k,\ldots,a_2)$. Let $P$ be a $\alpha\beta$ shortest path, where $V(P)$ denotes the vertex set of $P$. By $P[\gamma,\gamma']$ for two nodes $\gamma,\gamma'$ on $P$, we mean the subpath between $\gamma$ and $\gamma'$ on $P$, and we show the size of this subpath by $|P[\gamma,\gamma']|$. First we give some intuition on the following definitions. For a node $\gamma\in V(P)$ and an edge $e$ attached to it on the path, we think of the edge $e$ as an operation on the stacks and coordinate multi-arrays of the node $\gamma$: we might swap the order of the stacks, remove the top element of an stack, delete an empty stack and a coordinate multi-array, etc. 


%\mina{check the new "big" stack constraints/relaxations: say that the path is partitioned into (1) inner subpaths and (2) subpaths with all nodes of type 1 or 2. In this second type of subpaths, I can always assume that $S_{big}$ is the biggest stack, otherwise I just use a 0 weight edge to make it the biggest. Then if I start with a node $\gamma$ and end with $\gamma'$, if the biggest stack of $\gamma$ is the same as the biggest stack of $\gamma'$, coordinate doesn't change. If not, coordinate switches.}


% \mina{can assume that we only use a switch edge in layer $\floor{k/2}+1$. So for any node in a layer $j<\floor{k/2}+1$, can assume that the big stack is actually big. For $k$ even, this is still sort of true. For odd, there is only one vertex that violates this, by one.}

%\mina{todo: when considering edges, specify the type of the edge.}




\begin{definition}
Let $\alpha',\beta'\in V(P)$. Let $S$ be a stack in the stack array of $\alpha'$. We say that $S$ and $S_{\beta'}^{i}$ are the same stack for some $i\in \{big, main, 1,\ldots,t-2\}$, and show it by $S\equiv S_{\beta'}^{i}$, if throughout the $P[\alpha',\beta']$ path, the stack $S$ never gets deleted and only its content changes and it ends up at position $i$ in the stack array of $\beta$. %We may just write $S\equiv S_{\beta'}^{i}$ if the path is clear. 

Moreover, if $\gamma\gamma'$ is a pseudo outer stack change edge in $P$, we assume that $S_{main}^{\gamma}\not\equiv S_{main}^{\gamma'}$. In other words, a pseudo outer stack change edge in a path simultaneously deletes the main stack and creates a new main stack.
\end{definition}



\begin{definition}
For two stacks $S$ and $S'$, let $|S\cap S'|$ be the maximum $j$ such that the contents of the substacks of size $j$ of $S$ and $S'$ are the same. 
\end{definition}
\begin{definition}
For two stacks $S$ and $S'$ where $S$ belongs to the stack array of some node $\gamma\in V(P)$ and $S'$ belongs to the stack array of some node $\gamma'\in V(P)$, we say that $S=S'$ if $S\equiv S'$ and $|S\cap S'|=|S|=|S'|$.
\end{definition}

\begin{observation}
\label{obs:type2edge}
Any edge that is between two different layers must be a vector-change edge, and has type $2$ endpoints. If the coordinate multi array of one is $X$, coordinate multi array of the other is $X$ as well. Moreover, for any $\gamma\gamma'$ stack change edge, $S_{big}^{\gamma}$ and $S_{big}^{\gamma'}$ are the same stacks with the same contents; i.e. $S_{big}^{\gamma}=S_{big}^{\gamma'}$.
\end{observation}
\begin{observation}
 Throughout a path, the coordinate belonging to a stack doesn't change as long as the stack is not deleted or replaced. In other words, a coordinate multi-array changes if and only if the stack belonging to it changes.\mina{todo: needs adjustment}
\end{observation}
%\mina{an observation saying that a coordinate multiarray changes if and only if the stack belonging to it changes.}

\begin{definition}
\textbf{Inner subpath.} Let $\gamma$ be a type $t$ node in layer $j$ on the $\alpha-\beta$ path where $t>2$. Then it is on a subpath of $P$ with all nodes in layer $j$,  endpoints of type 2, and all other nodes of type $>2$. We call this subpath the ``inner subpath" containing $\gamma$.

More generally, an \textit{``inner subpath"} is a subpath with all nodes in the same layer, endpoints of type $2$ and other nodes of type $>2$. We consider a pseudo outer stack change edge an inner subpath as well. 
%This is because as long as $S_{big}$ does not change, we are in the same layer, and it only can change through a type 2 node.
\end{definition} 


We call the vertices of a path that are not endpoints, the inner vertices of the path. If a path has only type $2$ inner vertices with type $1$ or type $2$ endpoints, we call it a an ``outer" subpath. The path $P$ can be decomposed into inner subpaths and outer subpaths, sharing endpoints. \mina{todo: make a figure for this.} From the definition of inner subpath, we know that if $\gamma=(S_{main}^{\gamma},S_{big}^{\gamma},X)$ and $\gamma'=(S_{main}^{\gamma'},S_{big}^{\gamma'},Y)$ are the endpoints of an inner subpath, then $|S_{big}^{\gamma}|,|S_{big}^{\gamma'}|\ge \ceil{\frac{k-2}{2}}$; they are actually the ``big" stacks. Since the endpoints of outer subpaths are either the endpoints of an inner subpath or a type $1$ node, we have that their big stack is at least as big as their main stack. 

For outer subpaths, we know that the edges are swap edges or vector change edges; except for when the first (last) endpoint is a type $1$ node then the first (last) edge is a stack change edge.

Each vector change edge removes a vector from one stack and adds a vector to either of the stacks, and a swap edge swaps the order of the stacks, but doesn't change their contents. So the order of these edges does not matter in an outer subpath. Moreover, we can assume a stronger structure on the nodes of this outer subpath: for any node $\gamma$ in layer $j<\floor{\frac{k}{2}}+1$, we can assume that $|S_{big}^{\gamma}|\ge |S_{main}^{\gamma}|$, hence $|S_{big}^{\gamma}|\ge\ceil{\frac{k-2}{2}}$. 

To see this, start from an endpoint. If the endpoint is a type $1$ node, start from the type $2$ node right after it. This node has its big stack at least as big as its main stack, since it is attached to a stack change edge. Now apply vector change edges (skipping swap edges) until the first node $\gamma_1$ where its big stack is at most the size of the main stack; i.e $|S_{big}^{\gamma_1}|\le |S_{main}^{\gamma_1}|$. This node must be in layer $\floor{\frac{k}{2}}+1$.%, as in the previous node the big stack was bigger than the main stack. 
 Now if $|S_{big}^{\gamma_1}|<|S_{main}^{\gamma_1}|$ we must have that $k$ is odd, and the previous edge was a vector change edge inside layer $\floor{\frac{k}{2}}+1$. In this case, add a swap edge right after $\gamma_1$ so that the next vertex has a big stack bigger than its main stack. Start from this vertex, and do the process again. Note that in this case, the swap edge is always attached to a vector change edge both in layer $\floor{\frac{k}{2}}+1$.

If $|S_{big}^{\gamma_1}|=|S_{main}^{\gamma_1}|$, consider the next vector change edge. If it removes a vertex from $S_{big}^{\gamma_1}$, do a swap edge. If it removes a vertex from $S_{main}^{\gamma_1}$, don't add a swap edge. This way, the next edge always removes an element from the main stack, so the next vertex has its big stack bigger than its main stack. Again, starting from this vertex, we can continue this process.
Note that since the other endpoint has its big stack at least as big as its main stack, we won't need any swap edges at the end. Except when $k$ is even and the other endpoint is at layer $\floor{\frac{k}{2}}+1$, then we might need a swap edge at the end. So we have the following observation.

%Moreover we can assume a stronger structure on these outer subpaths: All vector change edges must be removing an element from the same stack $S$, and adding an element to the same stack $S'$, otherwise we can shorten this subpath while preserving the endpoints. To prove this, suppose that the two endpoints of our outer subpath are $\gamma$ and $\gamma'$, and suppose that the their two stacks are $S$ and $S'$ (with possibly different contents for each). If the contents of one of the stacks is the same for both endpoints, it means that we remove and add vectors to the same stack at each edge. 



%\begin{claim}
%If an outer subpath does not pass layer $\floor{\frac{k}{2}}+1$, it has even number of swap edges, hence we can remove all these swap edges.
%\end{claim}
%\begin{proof}
% We know that in this subpath no stacks are created or deleted. Now if $S$ is the big stack of one endpoint, it is the big stack of the other endpoint as well. Because otherwise there is a node with stacks of size $\floor{\frac{k-2}{2}}$ and $\ceil{\frac{k-2}{2}}$, which belongs to layer $\floor{\frac{k}{2}}+1$. 
%\end{proof}
%So the only outer subpath that have swap edges pass layer $\floor{\frac{k}{2}}+1$, hence we can assume that swap edges only appear in this layer in $P$. 
\begin{observation}
\label{obs:swapedge}
We can assume that swap edges only appear in layer $\floor{\frac{k}{2}}+1$. Moreover, for any vertex $\gamma$ in layer $j<\floor{\frac{k}{2}}+1$, we can assume that $|S_{big}^{\gamma}|\ge \ceil{\frac{k-2}{2}}\ge |S_{main}^{\gamma}|$. 
\end{observation}


For a node $\gamma$, if $|S_{big}^{\gamma}|\ge \ceil{\frac{k-2}{2}}\ge |S_{main}^{\gamma}|$, we call $\gamma$ a \textit{well-ordered} node. Note that by observation \ref{obs:swapedge}, if $k$ is even, all the nodes on $P$ are well-ordered. If $k$ is odd, only layer $\floor{\frac{k}{2}}+1$ might have nodes that are not well-ordered. If $\gamma$ is a well-ordered node in layer $j$, then $|S_{big}^{\gamma}|=k-j$ and $|S_{main}^{\gamma}|=j-2$.


\begin{lemma}
\label{lem:different-main-stack}
Let $\gamma,\gamma'\in V(P)$ be two type 2 well-ordered nodes in layer $j$. Suppose that $S_{main}^{\gamma}\not\equiv S_{main}^{\gamma'}$ and $S_{main}^{\gamma}\not \equiv S_{big}^{\gamma'}$. Then $|P[\gamma,\gamma']|\ge j-1$. 
\end{lemma}
\begin{proof}
Through the path, we must empty $S_{main}^{\gamma}$ and delete it. This takes at least $(j-2)+1$, since $|S_{main}^{\gamma}|=j-2$.
\end{proof}

\begin{corollary}\label{lem:coordinate-change}
If $\gamma,\gamma'\in V(P)$ are two type 2 well-ordered nodes in layer $j$ with different coordinate multi-arrays, then $|P[\gamma,\gamma']|\ge j-1$. 
\end{corollary}
%\begin{proof}
%If $S_{main}^{\gamma}\not \equiv S_{main}^{\gamma'}$, then by Lemma \ref{lem:different-main-stack} $|P[\gamma,\gamma']|\ge j-1$. If $S_{main}^{\gamma} \equiv S_{main}^{\gamma'}$, the only way we can change coordinate multi-array belonging to this stack is to empty the stack and take a pseudo outer stack change edge. Again, this adds up to $j-1$ cost, since $|S_{main}^{\gamma}|=j-2$.
%\end{proof}


\begin{lemma}
\label{lem:lay1-jdist}
Let $\alpha'\in V(P)$ be a well-ordered node in layer $i\ge 1$ and let $\gamma=(S_{main}^{\gamma},S_{big}^{\gamma},X)\in V(P)$ be a well-ordered node in layer $j$. If $S_{big}^{\gamma}\equiv S_{big}^{\alpha'}$, and $|S_{big}^{\gamma}\cap S_{big}^{\alpha'}|=t$, then $|P[\alpha',\gamma]|\ge k-i-t+k-j-t$. If $S_{main}^{\gamma}\equiv S_{big}^{\alpha'}$ and  $|S_{main}^{\gamma}\cap S_{big}^{\alpha'}|=t'$, then $|P[\alpha',\gamma]|\ge k-i-t'+j-2-t'$.
\end{lemma}

\begin{proof}
First suppose $S_{big}^{\gamma}\equiv S_{big}^{\alpha'}$. Then to go from $\alpha'$ to $\gamma$, one should empty the top $k-i-t$ vectors of $S_{big}^{\alpha'}$, and add the $k-j-t$ top vectors of $S_{big}^{\gamma}$. Similarly, if $S_{main}^{\gamma}\equiv S_{big}^{\alpha'}$, then one should remove the first $k-i-t'$ top vectors of $S_{big}^{\alpha'}$, and add the first $j-2-t'$ top vectors of $S_{main}^{\gamma}$.
\end{proof}

%\mina{what if one of them is in the last layer? (so big stack not big). otherwise, what if we have k odd? correction: for our purposes, we can assume $S_{big}$ is the big stack in both.}
\begin{lemma}
\label{lem:basicdist}
Let $\alpha'\in V(P)$ be a well-ordered node in layer $i\ge 1$. Let $\gamma=(S_{main}^{\gamma},S_{big}^{\gamma},X)\in V(P)$ be a well-ordered node in layer $j$. If $S_{big}^{\gamma}\not\equiv S_{big}^{\alpha'}$, we have that $|P[\alpha',\gamma]|\ge k-j-i+2$.
\end{lemma}
\begin{proof}
%\mina{todo} using the above lemma basically.
This is because if we want the big stack to change to another stack, we have to go to layer $\floor{k/2}+1$ as it is the only layer with a swap edge by Observation \ref{obs:swapedge}. So if $k$ is even, we have $|P[\alpha',\gamma]|\ge (k/2-i+1)+(k/2-j+1)=k-i-j+2$. We have to take a vector change edge in this layer, so we have $|P[\alpha',\gamma]|\ge ((k-1)/2-i+1)+1+((k-1)/2-j+1)=k-i-j+2$.
\end{proof}
\begin{lemma}
\label{lem:toomanyvectors}
Suppose that $S$ and $S'$ are two stacks that are both compatible with a coordinate array $X^{(i,j)}$, and that $|S|+|S'|\ge k$. Then for any $t\le\min(k,|S|)$, there is a coordinate that all vectors in $S[1..t]\cup S'[1..k-t]$ are $1$ in that coordinate.
\end{lemma}
\begin{proof}
If both $S$ and $S'$ are right-compatible, all vectors in $S\cup S'$ share coordinate $X^{(i,j)}[1]$. Similarly if both stacks are left-compatible, all vectors share coordinate $X^{(i,j)}[k-1]$. Suppose WLOG that $S$ is right-compatible and $S'$ is left-compatible. Then all vectors in $S[1..t]\cup S'[1..k-t]$ share coordinate $X^{(i,j)}[t]$.
\end{proof}
\begin{lemma}
\label{lem:switch}
Let $\gamma=(S_{main}^{\gamma}, S_{big}^{\gamma}, X)$ and $\gamma'=(S_{main}^{\gamma'}, S_{big}^{\gamma'}, Y)$ be two well-ordered nodes in $V(P)$ 
where $S_{big}^{\gamma}\equiv S_{main}^{\gamma'}$ and $S_{big}^{\gamma'}\equiv S_{main}^{\gamma}$. Then we have that $Y=\bar{X}$ 
\end{lemma}
\begin{proof}

%\mina{todo} basically because the stacks don't change so the coordinate doesn't change, but it switches so the coordinate switches as well.
%First suppose that $X\neq \bar{Y}$ or $X\neq Y$. Then we must have change $X$, without changing the stack it belongs to. This is only possible if we empty the main stack and take a pseudo outer stack change edge

The $\gamma\gamma'$ path consists of inner and outer subpaths, and all nodes have $S_{main}^{\gamma}$ and $S_{big}^{\gamma}$ among their stacks.
So any inner subpath has endpoints with the same coordinate multi-array, because none of their stacks change. Moreover, the outer subpaths consist of only type 2 vertices, and by Observation \ref{obs:type2edge}, any edge between type 2 nodes keeps the coordinate multi-array (vector change edge) or switches it (swap edge). Now since with every swap edge, stacks swap, from $\gamma$ to $\gamma'$ we must have an odd number of swap edges, so $Y=\bar{X}$.
\end{proof}

\begin{definition}\textbf{Incompatibility number.}
For a stack $S$ and a coordinate multi-array $X$, we say that the \textit{incompatibility number} of $S$ and $X$ is $j$, if $j$ is the smallest number, such that $S[1\ldots j]$ and $X^{(main,i)}$ are not compatible for any $i$. We use the notation $Inc(S,X)=j$. If no such number exists, we say $Inc(S,X)=|S|+1$.
\end{definition}

\begin{lemma}
\label{lem:inner_subpath}
Let $\gamma=( S,S_{big}, X)$ and $\gamma'=(S',S_{big},X')$ be two well-ordered nodes in layer $i$, where $X\neq X'$ and $S\not\equiv S'$. Then we have $d(\gamma,\gamma')\ge 2i-2-(\max{(Inc(S,X'),Inc(S',X),1)})$.
\end{lemma}
\begin{proof}
%First suppose that $S$ and $S'$ are same stack (with potentially different vectors in them). Then in order to change the coordinate multi-array belonging to $S$, we need to empty the stack, change coordinate using a pseudo outer stack change edge, and then load the contents of $S'$. This takes $2(i-2)+1$.% because the coordinate multi-arrays corresponding to them are different. \mina{psudo} So when $X$ is being deleted, the stack corresponding to it ($S$) is being deleted as well. 

First suppose that there is no node in the $\gamma \gamma'$ path that has both stacks $S$ and $S'$. We also know that throughout this path, $S$ is being emptied and destroyed, and $S'$ is being created and loaded from empty. Since $|S|=|S'|=i-2$, loading and de-loading each takes $i-2$, and destroying $S$ and creating $S'$ takes at least $1$, so $d(\gamma,\gamma')\ge 2i-3$.

Now suppose that there is a node $\mu$ in the $\gamma\gamma'$ path that has both stacks $S$ and $S'$. WLOG, suppose that $S$ appears first in the stack array of $\mu$. Note that the coordinate multi-arrays belonging to $S$ and $S'$ are $X$ and $X'$. So $S'$ and $X^{(main,i)}$ are compatible for some $i$. Since $S'$ remains in the stack-array in the $\mu\gamma'$ path and $S$ gets deleted somewhere in this path, there is a node $\mu'$ for which $S$ is empty. So $d(\gamma,\mu')\ge i-2$. Since $S'$ and $X^{(main,i)}$ are compatible, we know that $S'$ has at most $Inc(S',X)-1$ (of its original) vectors in it. So $d(\mu',\gamma')\ge i-2-(Inc(S',X)-1)$. So $d(\gamma,\gamma')\ge 2i-2-Inc(S',X)$. 
\end{proof}

Now we prove the YES case. Recall that $\alpha=(C_0)$ and $\beta=(C_1)$ where $C_0=(a_1,\ldots,a_{k-1})$, $C_1=(a_k,\ldots,a_2)$, and $a_1,\ldots,a_k$ are orthogonal vectors. First we go through two simple cases.
Suppose that $C_0$ and $C_1$ are the same stacks. This means that through the $\alpha\beta$ path, we empty $C_0$, and then we add the vectors of $C_1$. This takes at least $2k-2$. \mina{argue the +1 remaining cost: coordinate change probably.} So we assume that $C_0$ and $C_1$ are not the same stack. Let $P_0$ be part of $P$ that has $C_0$ in all nodes, and $P_1$ be part of $P$ that has $C_1$ in all nodes.

Now suppose that there is no node that contains both $C_0$ and $C_1$ among its stacks. So $P_0$ and $P_1$ don't have any nodes in common, and since we have to empty $C_0$, $|P_0|\ge k-1$ (size of the path is the number of its edges). Similarly, $|P_1|\ge k-1$. There is also an edge between $P_0$ and $P_1$, so $|P|\ge 2k-1$. 

So we assume that there is a node $\gamma$ with both $C_0$ and $C_1$ among its stacks. We can assume that $\gamma$ is the ``first'' node on the $\alpha\beta$ path that has both stacks. So $\gamma\in P_0\cap P_1$, and in fact $\gamma$ is the first node in $P_1$. So $C_1$ is empty in $\gamma$. Furthermore, we must have that $\gamma$ is a well-ordered node. This is because the only nodes that are not well-ordered are type 2 and in layer $\floor{\frac{k}{2}}+1$, so none of their stacks are empty.
Now we have two cases:
\begin{itemize}
    \item Case 1: $S_{big}^\gamma\equiv C_0$.
    \item Case 2: $S_{big}^\gamma\not \equiv C_0$.
\end{itemize}
\subsection{Case 1}
Suppose that $S_{big}^\gamma\sequiv{P} C_0$. Recall that $P_0$ is the subpath of $P$ containing $C_0$, and $P_1$ is the subpath of $P$ containing $C_1$. Let the endpoints of the inner subpath containing $\gamma$ be $\gamma_1'$ and $\gamma_1$, where $\gamma_1'$ is in $P[\alpha,\gamma]$ and $\gamma_1\in P[\gamma,\beta]$. So $S_{big}^{\gamma}=S_{big}^{\gamma_1'}=S_{big}^{\gamma_1}\equiv C_0$. Moreover, since $\gamma_1\in P_1$ and $\gamma_1'\notin P_1$, we have that $S_{main}^{\gamma_1}\equiv C_1$ and $S_{main}^{\gamma_1'}\not \equiv C_1$. 
Let the coordinate multi-array of $\gamma_1$ be $X$.%, so $\gamma_1=(S_{big}^\gamma\equiv C_0, S_{main}^{\gamma}\equiv C_1, Y)$. Let the last type 2 node on $\alpha\gamma$ path be $\gamma_1'$. Note that since $\gamma_1'$ must have the same big stack as $\gamma$, and it doesn't have $C_1$ among its stacks (since $\gamma$ was the first node on the path having both $C_0$ and $C_1$).

 

%Let $P'$ be the subpath in the intersection of $P_0$ and $P_1$. We argue that the coordinate multi-array on all type-2 nodes on $P'$ are the same, and as a result it is $Y$. This is because all these nodes have $C_1$ and $C_0$ as their $S_{big}$ and $S_{main}$. If a coordinate changes in a layer, the $S_{main}$ changes. \mina{better explanation?}

Symmetrically, let the last node containing $C_0$ be $\gamma'$. Suppose that the endpoints of the inner subpath containing $\gamma'$ are $\gamma_2$ and $\gamma_2'$, where $\gamma_2\in P[\alpha,\gamma']$ and $\gamma_2'\in P[\gamma',\beta]$. Since $\gamma_2\in P_0\cup P_1$, $\gamma_2'\notin P_0$ and $S_{big}^{\gamma_2}=S_{big}^{\gamma_2'}$, we have that $C_1\equiv S_{big}^{\gamma_2}=S_{big}^{\gamma_2'}=S_{big}^{\gamma}$. Moreover, $S_{main}^{\gamma_2}\equiv C_0$ and $S_{main}^{\gamma_2'}\not \equiv C_0$. Let the coordinate multi-array of $\gamma_2$ be $Y$. By Lemma \ref{lem:switch} we have $X=\bar{Y}$.



%in Let the last type 2 node on the $\alpha\gamma'$ path be $\gamma_2$, and let the first type 2 node on the $\gamma'\beta$ path be $\gamma_2'$. See Figure \ref{fig:case1}. Note that $S_{big}^{\gamma_2}=S_{big}^{\gamma_2'}$, and $\gamma_2\in P_0\cap P_1$ and $\gamma_2\in P_1$. So we must have that $\gamma_2=(S_{big}^{\gamma_2}\equiv C_1, S_{main}^{\gamma_2}\equiv C_0, X)$.  %Let the first type-2 node in $\gamma'\beta$ path be $\gamma_2'$. Note that $\gamma_2'$ doesn't have $C_0$ among its stacks, and has $C_1$ as its big stack.



\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{case1.pdf}
    \caption{Case 1. Purple stack indicates $C_0$ and Blue stack indicates $C_1$.\mina{todo: change the order of stacks.}}
    \label{fig:case1}
\end{figure}

%So let the last type-2 node on $P'$ be $\gamma_2$. Since the type-2 node after $\gamma_2$ preserves $S_{big}$ in $\gamma_2$ as one of its stacks, it should be that $S_{big}$ in $\gamma_2$ is $C_1$. So $S_{main}$ is $C_0$. 

Let $t=|S_{big}^{\gamma_1}\cap S_{big}^{\alpha}|=|S_{big}^{\gamma_1'}\cap S_{big}^{\alpha}|$. Similarly, let $t'=|S_{big}^{\gamma_2}\cap S_{big}^{\beta}|=|S_{big}^{\gamma_2'}\cap S_{big}^{\beta}|$. 
Suppose that $\gamma_1$ and $\gamma_1'$ are in layer $j$, and $\gamma_2$ and $\gamma_2'$ are in layer $j'$. Note that $\gamma_1,\gamma_1',\gamma_2$ and $\gamma_2'$ are all well-ordered nodes since they are endpoints of inner subpaths. We have:
\begin{align*}
    &|P[\alpha,\gamma_1']| \ge k-1-t+k-j-t \text{ by Lemma \ref{lem:lay1-jdist}}\\
    &|P[\gamma_1',\gamma_1]|\ge j-1\text{ since $S_{main}^{\gamma_1}\not\equiv S_{main}^{\gamma_1'}$, by Lemma \ref{lem:different-main-stack}}\\
    &|P[\gamma_1,\gamma_2]|\ge  k-j-j'+2 \text{ since $S_{big}^{\gamma_1}\not\equiv S_{big}^{\gamma_2}$ by Lemma \ref{lem:basicdist}}\\
    &|P[\gamma_2,\gamma_2']|\ge j'-1\text{ since $S_{main}^{\gamma_2}\not\equiv S_{main}^{\gamma_2'}$, by Lemma \ref{lem:different-main-stack}} \\
    &|P[\gamma_2',\beta]|\ge k-1-t'+k-j'-t'\text{ by Lemma \ref{lem:lay1-jdist}}
\end{align*}
All these distances add up to $|P|\ge 5k-2(t+t'+1)-(j+j')$. 
We have two subcases:

We just need to show that $t+t'\le k-1$. This is because then we have that $|P|\ge 3k-(j+j')$. We know that $j,j'\le \floor{\frac{k}{2}}+1$. Unless $j=j'=k/2+1$ for even $k$, we have $|P|\ge 2k-1$. If $j=j'=k/2+1$, then since $\frac{k}{2}-1\ge |S_{big}^{\gamma_1}|\ge t$ and $\frac{k}{2}-1\ge |S_{big}^{\gamma_2}|\ge t'$, we have $t+t'\le k-2$, and so $|P|\ge 2k-1$.

Now we show that $t+t'\le k-1$. Note that $X^{(main,big)}=Y^{(main,big)}$ and it is compatible with $S_{big}^{\gamma_1}$ and $S_{big}^{\gamma_2}$. If $t+t'>k$, then since $S_{big}^{\gamma_1}[1..t]=(a_1,\ldots,a_t)$ and $S_{big}^{\gamma_2}[1,\ldots,k-t]=(a_k,\ldots,a_{t+1})$, by Lemma \ref{lem:toomanyvectors}, $\{a_1,\ldots,a_k\}$ share a coordinate which is a contradiction. 
%\paragraph{subcase 1b. not complete yet.}\mina{not needed: just say that when you do pseudo edge, you change the stack to another empty stack.} Suppose that $t+t'\ge k$. We are going to measure the $\gamma_1-\gamma_2$ distance more carefully. Note that in this case we have $X\notin \{Y,\bar{Y}\}$. This is because otherwise, $X^{(main,big)}=Y^{(main,big)}$ and it is compatible with $S_{big}^{\gamma_1}[1..t]=(a_1,\ldots,a_t)$ and $S_{big}^{\gamma_2}[1,\ldots,k-t]=(a_k,\ldots,a_{t+1})$, and so by Lemma \ref{lem:toomanyvectors}, $\{a_1,\ldots,a_k\}$ have a coordinate in common. Now since both $C_0$ and $C_1$ are in the stack array of all the nodes on the $P[\gamma_1,\gamma_2]$ subpath, the only way to change the main coordinate multi-array is through a pseudo outer stack change edge. 
%Let $\eta_1\eta_2$ be this edge, where coordinate multi-array $X$ is changed. The stack belonging to $X$ in $\eta$ is either $C_0$ or $C_1$, if $\eta_1'$ is the endpoint of the inner subpath containing $\eta_1'$ that is on $P[\gamma_1,\eta_1]$ subpath, it has either of $C_0$ or $C_1$ as its main stack, so $X$ belongs to this stack throughout the inner subpath. 

%First suppose that $X$ belongs to $C_1$ in $\eta_1$. This means that $C_1$ is empty in $\eta_1$. We show that in this case we can shorten $P$, and hence get a contradiction.  Instead of going to $\eta_1$ through $\gamma_1$, we use a node $\tilde{\gamma_1}=(S_{big}^{\gamma_1},S*,X)$, where $S*\equiv C_1$ is the stack of size $j-2$ with all-one vectors. First note that $\tilde{\gamma_1}$ is a valid node, because $S*$ is compatible with any coordinate array. Moreover, we can simulate the $P[\gamma_1,\eta_1]$ path to have a path of the same size from $\tilde{\gamma_1}$ to $\eta_1$: for any vertex in the $P[\gamma_1,\eta_1]$ path, replace all the vectors of $C_1$ in this vertex with the all-one vectors.\mina{more explanation maybe?}. Now we show that there is a path from $\alpha$ to $\tilde{\gamma_1}$ which is shorter than $|P[\alpha,\gamma_1]| = 2k-2t-2$. In fact, since $S_{big}^{\alpha}\cap S_{big}^{\tilde{\gamma_1}}=t$, by Lemma \mina{easy, todo} there is a path of length \mina{to complete}



 %\mina{this might be a lemma in the no case?}


%  So there are two nodes $\eta$ and $\eta'$ in layer $2$, where $\eta\eta'$ is a pseudo outer stack change edge which changes the coordinate multi array of $\eta$ to $Y$. 


%Note that $S_{big}^{\alpha}\equiv C_0$ and $S_{big}^\beta \equiv C_1$.
%Suppose in $\gamma_1$ and $\gamma_1'$, $t$ is the biggest number such that $S_{main}[1..t]=C_0[1..t]$. Similarly, suppose that $t'$ is the biggest number such that in $\gamma_2$ and $\gamma_2'$, $S_{main}[1..t']=C_1[1..t']$.
%Since $S_{big}^{\gamma_1}[1..t]=\{a_1,\ldots,a_t\}$ and $Y^{(main,big)}$ are compatible, and $S_{big}^{\gamma_2}[1..t']=\{a_k,\ldots,a_{k-t'+1}\}$ and $\bar{Y}^{(main,big)}=\bar{Y}^{(big,main)}=Y^{(main,big)}$ are also compatible, we have that $t+t'\le k-1$, because otherwise by Lemma \ref{lem:toomanyvectors}, $S_{big}^{\gamma_1}[1..t]\cup S_{big}^{\gamma_2}[1..k-t]=\{a_1,\ldots,a_k\}$ share a coordinate.

%Now we are ready to compute the length of the path $P$ from $\alpha$ to $\beta$.

%By Lemma \ref{lem:lay1-jdist} we have that $d(\alpha,\gamma_1') \ge k-1-t+k-j-t$. Since the main stack changes from $\gamma_1'$ to $\gamma_1$, we have that $d(\gamma_1',\gamma_1)\ge j-1$. Since the main stack and the big stack switch form   $\gamma_1$ and $\gamma_2$, we must have that $d(\gamma_1,\gamma_2)\ge k-(j-1+j'-1)$. This is because we must have visited layer $\floor{k/2}+1$, and if $k$ is odd we must have an edge inside this layer that switches the two stacks.

%Similarly we have that $d(\gamma_2,\gamma_2')\ge j'-1$, and $d(\gamma_2',\beta)\ge k-1-t'+k-j'-t'$. 




\subsection{Case 2}
Suppose that $C_1$ and $C_0$ are among the stacks of the node $\gamma$ in layer $j$, and $S_{big}^{\gamma}\not \equiv C_0$. Note that $S_{big}^{\gamma}\not \equiv C_1$, since $C_1$ is empty at $\gamma$ and $\gamma$ is well-ordered. We are going to consider a few extra well-ordered nodes on the $\alpha\beta$ path and state a few observations about them. See Figure \ref{fig:case2}.


\begin{itemize}
    \item Let $\gamma_2$ and $\gamma_3$ be the endpoints of the inner subpath containing $\gamma$. Let the only coordinate multi-array of $\gamma_2$ be $X$ and the only coordinate multi-array of $\gamma_3$ be $Y$. Note that $\gamma_2$ and $\gamma_3$ are well-ordered.
    \item Let $\gamma_1$ be the first type-2 node with $X$ or $\bar{X}$ as its coordinate multi-array. If $\gamma_1$ is attached to a type $1$ node, we let $\gamma_1$ be that type 1 node. Suppose $\gamma_1$ is in layer $j_1$.
    \item Similarly, let $\gamma_4$ be the last type-2 node with $Y$ or $\bar{Y}$ as its coordinate multi-array. Suppose that $\gamma_4$ is in layer $j_4$. 
    \item Let $\gamma_1'$ be the last type 2 node on $\alpha\gamma_1$ path excluding $\gamma_1$, and let $\gamma_4'$ be the first node on the $\gamma_4\beta$ path excluding $\gamma_4$. Note that $\gamma_1'$ has a different coordinate multi array than $X$ or $\bar{X}$. If $\gamma_1$ is a type $1$ node, we let $\gamma_1'=\gamma_1$. Similarly, if $\gamma_4$ is a type 1 node, we let $\gamma_4'=\gamma_4$.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{case2.pdf}
    \caption{Case 2. Purple stack indicates $C_0$ and Blue stack indicates $C_1$.\mina{todo: change order of the stacks.}}
    \label{fig:case2}
\end{figure}

Now we state some observations about these nodes:
\begin{enumerate}
    \item \label{fact1} Since $\alpha\gamma$ subpath is part of $P_0$ and $S_{big}^{\gamma_2}=S_{big}^{\gamma}\not\equiv C_0$, we must have that $S_{main}^{\gamma_2}\equiv C_0$. Similarly, since $\gamma\beta$ subpath is part of $P_1$, we have that $S_{main}^{\gamma_3}\equiv C_1$. Also note that $S_{big}^{\gamma_2}=S_{big}^{\gamma}=S_{big}^{\gamma_3}$ and they are neither $C_0$ nor $C_1$. 
    \item \label{fact:samelayer}$\gamma_1'$ is in layer $j_1$ (same layer as $\gamma_1$). This is because if the last edge in $\alpha\gamma_1$ path is a stack change edge, then $\gamma_1'$ and  $\gamma_1$ are the endpoints of an inner subpath, hence they are in the same layer. If this edge is not a stack change edge, then it is either a swap edge or a vector change edge. This cannot happen because then the other endpoint of this edge (other than $\gamma_1$) has $\bar{X}$ or $X$ as its coordinate multi-array.  
    \item $\gamma_4'$ is in layer $j_4$ (same layer as $\gamma_4$). The reasoning is similar to above.
    \item $S_{big}^{\gamma_1'}=S_{big}^{\gamma_1}$. This is because by observation \ref{fact:samelayer}, $\gamma_1$ and $\gamma_1'$ are either the endpoints of an inner subpath, or they are both the same vertex in layer $1$. Note that by this observation we have $\gamma_1$ and $\gamma_1'$ are well-ordered. 
    \item $S_{big}^{\gamma_4'}=S_{big}^{\gamma_4}$. Similar as above. Note that by this observation we have $\gamma_4$ and $\gamma_4'$ are well-ordered. 
   % \item \label{fact:differentmain} $|P[\gamma_1,\gamma_1']|\ge j_1-1$. This is because  $S_{main}^{\gamma_1'}\not\equiv S_{main}^{\gamma_1}$. This is because $\gamma_1$ and $\gamma_1'$ have different coordinate multi arrays. Similarly, $S_{main}^{\gamma_4'}\not\equiv S_{main}^{\gamma_4}$. \mina{quasi edge affects this, if main stack is empty. Replace with their distance.} 
    \item We can assume $S_{big}^{\gamma_1}\equiv C_0$.  Suppose that this is not true. Then $S_{main}^{\gamma_1}\equiv C_0$ as $\gamma_1$ is in $P_0$. We have that $\gamma_1'$ is also in layer $j_1$ and $S_{big}^{\gamma_1'}=S_{big}^{\gamma_1}\not\equiv C_0$ so by Lemma \ref{lem:basicdist} we have $d(\alpha,\gamma_1')\ge k-j+1$, and since the main stack changes from $\gamma_1'$ to $\gamma_1$, by Lemma \ref{lem:different-main-stack} we have $d(\gamma_1',\gamma_1)\ge j-1$. So $d(\alpha,\gamma_1)\ge k$. With similar reasoning, $d(\gamma_1,\gamma_2)\ge j-1$ and by Lemma \ref{lem:basicdist} $d(\gamma_2,\beta)\ge k-j+1$. So $|P|\ge 2k$.
    \item  We can assume $S_{big}^{\gamma_4} \equiv C_1 $. Similar as above.
    
\end{enumerate}

 



%First we argue that $S_{big}^{\gamma_1}$ is $C_0$. Suppose that this is not true. Then $S_{main}^{\gamma_1}\equiv C_0$ as $\gamma_1$ is in $P_0$. We have that $\gamma_1'$ is also in layer $j_1$ and $S_{big}^{\gamma_1'}=S_{big}^{\gamma_1}\not\equiv C_0$ So by Lemma \ref{lem:basicdist} we have $d(\alpha,\gamma_1')\ge k-j+1$, and since the main stack changes from $\gamma_1'$ to $\gamma_1$, we have $d(\gamma_1',\gamma_1)\ge j-1$. So $d(\alpha,\gamma_1)\ge k$. With similar reasoning, $d(\gamma_2,\gamma_2)\ge j-1$ and by Lemma \ref{lem:basicdist} $d(\gamma_2,\beta)\ge k-j+1$. So $|P|\ge 2k$.
%Then since $d(\gamma_2,\beta)\ge j-1+k-j+1$, we have $|P|\ge 2k$. 

Now since all $\gamma_i$ and $\gamma_i'$ nodes are well-ordered, we have that the following:
\begin{observation}
\label{obs:distances-case2}
Using the above observations, we have the following distances. Note that $\gamma_1$ and $\gamma_1'$ either have different coordinate multi-arrays, or are the same vertex and in layer $1$ ($\gamma_4$ and $\gamma_4'$ are similar).
\begin{align*}
    &|P[\alpha,\gamma_1']|\ge j_1-1 \text{ minimum distance from layer $1$ to $j_1$} \\
    &|P[\gamma_1',\gamma_1]|\ge j_1-1 \text{ by Corollary \ref{lem:coordinate-change}} \\
    &|P[\gamma_1,\gamma_2]|\ge k-j_1-j+2 \text{ by Lemma \ref{lem:basicdist}, since } S_{big}^{\gamma_1}\not\equiv S_{big}^{\gamma_2}\\
    &|P[\gamma_2,\gamma_3]|\ge j-1 \text{ by Lemma \ref{lem:different-main-stack}, since} S_{main}^{\gamma_2}\not\equiv S_{main}^{\gamma_3}\\
    &|P[\gamma_3,\gamma_4]|\ge k-j_4-j+2 \text{ by Lemma \ref{lem:basicdist}, since } S_{big}^{\gamma_3}\not\equiv S_{big}^{\gamma_4}\\
    &|P[\gamma_4,\gamma_4']|\ge j_4-1 \text{ by Corollary \ref{lem:coordinate-change}} \\
    &|P[\gamma_4',\beta]|\ge j_4-1 
\end{align*}
\end{observation}
    


Summing the above distances, we have $|P|\ge 2k+j_1+j_4-j-1$. So if we have $j_1+j_4\ge j$, we are done. So suppose that $j_1+j_4\le j-1$

Now we estimate the above distances more accurately. 
Define the following parameters: $t_1 = |S_{big}^{\gamma_1}\cap S_{big}^{\alpha}|$, $t_2 = |S_{main}^{\gamma_2}\cap S_{big}^{\alpha}|$, $t_3 = |S_{main}^{\gamma_3}\cap S_{big}^{\beta}|$, $t_4 = |S_{big}^{\gamma_4}\cap S_{big}^{\beta}|$. Recall that $S_{big}^{\alpha}=(a_1,\ldots,a_{k-1})$ and $S_{big}^{\beta}=(a_k,\ldots,a_2)$.

We have the following:
\begin{align} \label{eq:gamma1gamma4}
    &|P[\alpha,\gamma_1]| \ge |P[\alpha,\gamma_1']|+|P[\gamma_1',\gamma_1]| \ge (k-1-t_1+k-j_1-t_1)+(j_1-1). \text{ by lemma \ref{lem:lay1-jdist}}\\
    &|P[\gamma_4,\beta]|\ge |P[\gamma_4,\gamma_4']|+|P[\gamma_4',\beta]| \ge (j_4-1)+(k-1-t_4+k-j_4-t_4).
\end{align}
\begin{claim}\label{claim:dist}
We have the following distances.
\begin{align}
    &|P[\alpha,\gamma_2]|\ge (k-1-t_2+j-2-t_2)+(j_1-1)\\
    &|P[\gamma_3,\beta]|\ge (k-1-t_3+j-2-t_3)+(j_4-1)
\end{align}
\end{claim} 
\begin{proof}
We only prove the second inequality. The first one is similar. If $t_3=t_4$, then 
\begin{align*}
    |P[\gamma_3,\beta]|&\ge |P[\gamma_4,\beta]|\\
    &\ge |P[(\gamma_4,\gamma_4']|+|P[\gamma_4',\beta]|\\
    &\ge (j_4-1)+(k-1-t_3+k-j_4-t_3)\\ 
    &\ge(j_4-1)+(k-1-t_3+j-2-t_3)
\end{align*}
    Where for the last inequality we use $j-2=|S_{main}^{\gamma_2}|\le \floor{k/2}-1\le |S_{big}^{\gamma_4}|= k-j_4$.
    
If $t_3\neq t_4$, then we have that $|S_{big}^{\gamma_3}\cap S_{big}^{\gamma_4}|=\min(t_3,t_4)$. Let $t'=\min(t_3,t_4)$, so  
\begin{align*}
    |P[\gamma_3,\beta]|&\ge |P[\gamma_3,\gamma_4]|+|P[\gamma_4,\gamma_4']|+|P[\gamma_4',\beta]|\\
    &\ge (k-j_4-t'+j-2-t')+(j_4-1)+(k-1-t_4+k-j_4-t_4)\\
    &\ge (k-j_4-t_3+j-2-t_3)+(j_4-1)+(k-1-t_4)\\
    &= (k-1-t_3+j-2-t_3)+(j_4-1) + (k-j_4-t_4)
\end{align*}
Note that $t_4\le k-j_4$ from the definition of $t_4$. We use Lemma \ref{lem:lay1-jdist} to bound $|P[\gamma_3,\gamma_4]|$ and $|P[\gamma_4',\beta]|$.
\end{proof}

We have two subcases. 


\paragraph{subcase 2a.} $t_1+t_3\le k-1$ or $t_2+t_4\le k-1$. WLOG assume the first happens. We divide $P$ into four subpath using $\gamma_1,\gamma_2$ and $\gamma_3$.
%$|P|\ge d(\alpha,\gamma_1)+d(\gamma_1,\gamma_2)+d(\gamma_2,\gamma_3)+|P[\gamma_3,\beta]|$, where for the first distance we use Equation \ref{eq:gamma1gamma4} and for the last distance we use Claim \ref{claim:dist}.
Summing these distances, we have the following:
\begin{align*}
    |P|&\ge |P[\alpha,\gamma_1]|+|P[\gamma_1,\gamma_2]|+|P[\gamma_2,\gamma_3]|+|P[\gamma_3,\beta]|\\
    &\ge (k-1-t_1+k-j_1-t_1)+(j_1-1) \text{  by Equation \ref{eq:gamma1gamma4}}\\
    &+(k-j_1-j+2) \text{ by Observation \ref{obs:distances-case2}}\\
    &+(j-1)\text{ by Observation \ref{obs:distances-case2}}\\
    &+(k-1-t_3+j-2-t_3)+(j_4-1) \text{ by Claim \ref{claim:dist}}\\
    &=4k-2t_1-2t_3-5+j+j_4-j_1\\
    &=(2k-1)+2(k-t_1-t_3-1)+(j-j_1-1)+(j_4-1)\\
    &\ge 2k-1
\end{align*}

%By Lemma \ref{lem:lay1-jdist} we have that the distance from $\alpha$ to the type-2 node before $\gamma_1$ is at least $k-1-t_1+k-j_1-t_1$ \mina{more explanation}, and hence $d(\alpha,\gamma_1)\ge k-1-t_1+k-j_1-t_1 + j_1-1$. We have $d(\gamma_1,\gamma_2)\ge k-j_1-j+2$, $d(\gamma_2,\gamma_3)\ge j-1$, $d(\gamma_3,\beta)\ge k-1-t_3+k-j-t_3$, and the coordinate change at $j_4$ costs $j_4-1$. \mina{explain why it doesn't intefere with $\gamma_3\beta$ path}. All these distances add up to $|P|\ge 5k-1-2t_1-2t_3-j_1-j+j_4$. Now since $t_1+t_3\le k-1$, $j_1<j\le k/2+1$, we have $|P|\ge 2k$.

\paragraph{subcase 2b.} $t_1+t_3\ge k$ and $t_2+t_4\ge k$. Note that in this case, $Inc(S_{main}^{\gamma_2},Y)\le k-t_4$. Suppose that this is not true and $S_{main}^{\gamma_2}[1..k-t_4],Y^{(main,big)}$ are compatible. From $\gamma_4$ we know that $S_{big}^{\gamma_4},Y^{(main,big)}$ are compatible. Now since $|S_{main}^{\gamma_2}\cap S_{big}^{\alpha}|=t_2\ge k-t_4$, we have that $S_{main}^{\gamma_2}[1..k-t_4]=\{a_1,\ldots,a_{k-t_4}\}$. On the other hand, we have that $S_{big}^{\gamma_4}[1..t_4]=\{a_k,\ldots,a_{k-t_4+1}\}$. So by Lemma \ref{lem:toomanyvectors}, we have that the vectors in $S_{main}^{\gamma_2}[1..k-t_4]\cup S_{big}^{\gamma_4}[1..t_4]=\{a_1,\ldots,a_k\}$ have a coordinate in common, a contradiction. Similarly, we have that $Inc(S_{main}^{\gamma_3},X)\le k-t_1$.

We divide $P$ into five subpaths using $\gamma_1,\gamma_2,\gamma_3$ and $\gamma_4$. Summing the distances, we have the following. %Using Equation \ref{eq:gamma1gamma4} to bound $d(\alpha,\gamma_1)$ and $d(\gamma_4,\beta)$, and we use Lemma \ref{lem:inner_subpath} $d(\gamma_2,\gamma_3)\ge(2j-2-\max\{k-t_4,k-t_1\})$. We have 
\begin{align*}
    |P|&\ge |P[\alpha,\gamma_1]|+|P[\gamma_1,\gamma_2]|+|P[\gamma_2,\gamma_3]|+|P[\gamma_3,\gamma_4]|+|P[\gamma_4,\beta]|\\
    &\ge (k-1-t_1+k-j_1-t_1)+(j_1-1) \text{ by Equation \ref{eq:gamma1gamma4}}\\
    &+(k-j_1-j+2) \text{ by Observation \ref{obs:distances-case2}}\\
    &+(2j-2-\max\{k-t_4,k-t_1,1\}) \text{ by Lemma \ref{lem:inner_subpath}}\\
    &+(k-j_4-j+2) \text{ by Observation \ref{obs:distances-case2}}\\
    &+(k-1-t_4+k-j_4-t_4)+(j_4-1) \text{ by Equation \ref{eq:gamma1gamma4}}\\
    &\ge 6k-2-2t_1-2t_4-j_1-j_4-\max\{k-t_4,k-t_1\}
\end{align*}
WLOG suppose $t_1\ge t_4$, and note that $k-t_4,k-t_1\ge 1$. So we have $|P|\ge 5k-2-t_1-2t_4-j_1-j_4$. Now since  $t_1\le|S_{big}^{\gamma_1}|= k-j_1$, $t_4\le |S_{big}^{\gamma_4}|=k-j_4$ and $t_4\le k-1$, we have $|P|\ge 2k-1$.% Otherwise, we have $t_1=t_4=k-1$, so basically $\gamma_1$ is the same as $\alpha$.\mina{todo: remaining +1 cost} 

%If $j_4=1$ \mina{we need a +1}.
%$d(\alpha,\gamma_1)\ge k-1-t_1+k-j_1-t_1+j_1-1$, $d(\gamma_1,\gamma_2)\le k-j_1-j+2$, by lemma ?? $d(\gamma_2,\gamma_3)\ge 2j-3-\max\{k-t_4,k-t_1\}$. We also have $d(\gamma_3,\gamma_4)\ge k-j_4-j+2$, and $d(\gamma_4,\beta)\ge k-1-t_4+k-j_4-t_4+j_4-1$. Summing these distances up, we have that $|P|\ge 6k-3-2t_1-2t_4-j_1-j_4-\max\{k-t_4,k-t_1\}$. WLOG suppose $t_1\ge t_4$, so we have $|P|\ge 5k-t_1-2t_4-j_1-j_4$. Now since $t_1\le k-j_1$, $t_4\le j_4-t_4$, and $t_4\le k-2$ \mina{what if $j_1=1$?}, we have that $|P|\ge 2k-1$.




==> proofsketch-long.tex <==
\section{Overview of the general $k$ reduction}
\label{sec:proofsketch}
%- Give an overview of the construction (start from OV, get a k vs. 2k-1 gap)
%- Vertices are “configurations” of vectors and coordinates, and operations, add/delete vectors and coordinates. In the No case, if any k vectors are orthogonal, then any two configurations are at most k operations apart. For the Yes case, we can find two configurations that are at least 2k-1.
%- Describe the configurations. As usual, each has vectors and coordinates. The vectors are ordered list of stacks S_1,…,S_t, and coordinates constraining the stacks. We require every vertex to have size (#stacks+#vectors)=k and |S_1|>=ceil{k-1/2). A vertex is valid if the vectors satisfy the coordinates in a certain way. The graph only has valid configurations as vertices.
%- The coordinates, the way they constrain the vectors, and how they change with the operations, are very delicate to define. We use primitive of coordinate-arrays (define coordinate arrays, and their key properties). At a high level, configurations have several coordinate arrays, each of which constrains one or two stacks. If the configuration has t stacks, S_1,..,S_t of vectors, we imagine a star graph whose vertices are S_1,..,S_t, with edges between S_1 and S_i for i=2,..,t. Each edge S_1S_i is identified by several coordinate arrays:, each of which constrains one of S_1 or S_i, and possibly some other stack.
%    - Each edge S_1S_i is identified by several coordinate arrays: X_*, which constraints S_1 and S_i, X_{1,j} for j=1,…,k, which constraints S_1 (there are many for a reason to be described later), and , each of which constrains one of S_1 or S_i, and possibly some other stack (. An operation 
%- Describe the edges, the operations on configurations (each operation has an insertion and deletion). The edge exists if the endpoints (and midpoint) are valid configurations. We need the operations to be invertible to get an undirected graph, and one can check that they are. Note operations preserve size, hence the definition of size. (Also, if there are two stacks S_1,S_2, we can flip S_1 and S_2, keeping the coordinate arrays but adjusting their labels.
%-  
%
%- In the No case, every k-tuple is orthogonal, we need every two configurations to be at distance k. If we ignore the coordinates and satisfying requirements, any two size-k configurations can reach each other in k steps: (delete the vector and stacks of one and build the vector and stacks of another). (Note more than two stacks is essential here)
%- In the Yes case, we want (ak,…,a2) and (a1,…,a_{k-1}) to be distance 2k-1. We need to use the coordinates to make this path length at least 2k-1. Note: stacks help this definition, we can’t drop the bottom vector too quickly, or else there is a short path by the NO case.
%- Coordinate change needs to be expensive, no coordinate-change edge. (all 1s vector).
We now sketch the ideas of the proof of Theorem~\ref{thm:main} for general $k$.

\subsection{The basic setup}
\label{ssec:proofsketch-0}
For our general reduction, we start with a $k$-OV instance $A\subset\{0,1\}^{\mathbb{d}}$ with size $|A|=n_{OV}$ and would like to construct a graph $G$ on $\tilde O(n_{OV}^{k-1})$ vertices and edges such that, if the set $A$ has $k$ orthogonal vectors (Yes case), the diameter of $G$ is at least $2k-1$, and otherwise (No case) the diameter of $G$ is at most $k$.
Throughout, we refer to elements of $A$ as \emph{vectors} and elements of $[\mathbb{d}]$ as \emph{coordinates}.
We may assume without loss of generality that the all ones vector $\mathbf{1}$ is in the set $A$.
We may also assume without loss of generality that no $k-1$ vectors of $A$ are orthogonal, as this can be checked in $\tilde O(n_{OV}^{k-1})$ time, and if there were then we already know we have $k$ orthogonal vectors.
%Like in the prior constructions for $k=2,3,4$, the graph $G$ contains an ``endpoint vertex'' for each element of $A^{k-1}$, as well as some ``internal vertices'', identified by at most $k-2$ vectors in $A$, and some constant (in terms of $k$) number of \emph{coordinates} in $[\mathbb{d}]$.
Each vertex of $G$ is identified by a \emph{configuration}, which contains vectors (in $A$) and coordinates (in $[\mathbb{d}]$), along with some meta-data.
Some configurations $H$ are \emph{valid}, meaning vectors in $H$ have 1s in specified coordinates of $H$, and there is one vertex of $G$ for each valid configuration.
Edges between vertices (configurations) of $G$ change up to one vector of a configuration and/or some of the coordinates of the configuration, and we think of edges as performing \emph{operations} on configurations.
The main challenge is making the graph is undirected, which we ensure by choose operations that always have an inverse operation.

\subsection{Configurations}
\begin{wrapfigure}{r}{8cm}
\begin{center}
\includegraphics{proofsketch-0.pdf}
\end{center}
\caption{Stacks satisfying coordinate arrays when $k=5$. Blue squares indicate a coordinate that must be 1. From left to right: Stack $a$ satisfies coordinate array $x$, Lemma~\ref{lem:stack-2}, Lemma~\ref{lem:yes-1}.}
\end{wrapfigure}
We now sketch the definitions of configurations and operations, which define the vertices and edges, respectively, of the Diameter instance.
We for clarity of exposition, we omit some technical details of the constructions that are not relevant for this high-level overview.
\paragraph{Configurations}
A \emph{configuration} $H$ is identified by the following:
\begin{enumerate}
%\item A parameter $t\in{1,\dots,k}$
%\item A sequence of $t$ lists of vectors $S_1,\dots,S_t$ (which we call \emph{stacks}) that have a total of $k-t$ vectors
\item An positive integer $t$ and a sequence of $t$ lists of vectors $S_1,\dots,S_t$, which we call \emph{stacks}.
List $S_1$ is special and is called the \emph{root}, and we require $S_1$ to have at least $(k-2)/2$ vectors.
%\item 
%\item An undirected (star) graph with vertices at $S_1,\dots,S_t$ and with edges $S_1,S_i$ for all $i=2,\dots,t$.
\item A set of $O_k(1)$ elements of $[d]^{k-1}$, which we call \emph{coordinate arrays}, which are each labeled by one or two stacks.
%attached to each edge.
\end{enumerate}
We define the \emph{size} of a configuration to be the number of stacks plus the total number of vectors in stacks.
The vertices of our Diameter instance $G$ correspond to the valid (defined below) size-$k$ configurations.

\paragraph{Valid configurations}
A configuration is \emph{valid} if its vectors satisfy a number of constraints, specified by the configuration's coordinate arrays.
These constraints are specified using the following definition (see Figure~\ref{fig:stack}), which was implicit in prior constructions \cite{BRSVW18, DW21,Li21}:
Stack $S=(a_1,\dots,a_s)$ \emph{satisfies} coordinate array $x$ if there exists sets $[k-1]= I_1\supset\cdots\supset I_s$ such that, for all $h=1,\dots,s$, we have $|I_h| = k-h$ and $a_h[x[i]] = 1$ for all $i\in I_h$.
%\begin{definition}[Stacks satisfying coordinate arrays]
%Let $S=(a_1,\ldots,a_{s})$ be a stack and let $x$ be a coordinate array.
%Stack $S=(a_1,\dots,a_s)$ \emph{satisfies} $x$ if there exists sets $[k-1]= I_1\supset\cdots\supset I_s$ such that, for all $h=1,\dots,s$, we have $|I_h| = k-h$ and $a_h[x[i]] = 1$ for all $i\in I_h$.
%\end{definition}
This definition has two key properties, which are easy to check (see Figure~\ref{fig:stack})
\begin{enumerate}
\item (Lemma~\ref{lem:stack-2}, useful for the No case) Let $S$ and $S'$ be stacks such that any $k$ vectors among the elements of $S$ and $S'$ are orthogonal. Then $S$ and $S'$ satisfy a common coordinate array.
%Let $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$ be stacks with at most $k-1$ vectors such that any $k$ vectors from among $a_1,\dots,a_s,b_1,\dots,b_{s'}$ are orthogonal.
%Then there exists a coordinate array satisfied by both $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$.
\item (Lemma~\ref{lem:yes-1}, useful for the Yes case) If $a_1,\dots,a_k$ are orthogonal, and $x$ is a coordinate array, then the stacks $(a_1,\dots,a_j)$ and $(a_k,\dots,a_{j+1})$ cannot both satisfy $x$.
\end{enumerate}
Each coordinate array $x$ in a configuration is labeled by one or two stacks, and a configuration is \emph{valid} if every coordinate array is satisfied by its one or two labeled stacks.
The actual list of coordinate arrays and their labeled stacks is omitted in this overview.
%For each edge $S_1S_i$, we include the following coordinate arrays:
%\begin{itemize}
%\item $X_*$ satisfied by $S_1$ and $S_i$,
%\item for $j=2,\dots,k$, a coordinate array $X_{i,j}$ satisfied by $S_i$ and, if $j<i$, by $S_j$.
%\item for $j=2,\dots,k$, a coordinate array $X_{1,j}$ satisfied by $S_1$.
%\end{itemize}

%It may seem redundant that there are several coordinate arrays that need only be satisfied by $S_1$ and several that are only satisfied by $S_i$.

\paragraph{Operations}
Operations are composed of half-operations.
A \emph{half-operation} on a configuration is one of the following.
\begin{enumerate}
\item (Vector insertion) insert a vector at the end of a stack
\item (Vector deletion) delete the last vector of a stack
\item (Node\footnote{We say ``Node insertion'' instead of ``stack insertion'' because in the actual construction, we place the stacks at vertices of a graph.} insertion) insert an empty non-root stack $S'$ (a list of zero vectors).
%any of positions $2,\dots, t+1$, and add an edge from $S'$ to $S_1$ with associated coordinate arrays.
\item (Node deletion) delete an empty non-root stack.\footnote{In the real construction, we require that the deleted stack is either $S_{t-1}$ or $S_t$, and require an analogous condition for node insertions. The proof holds without this requirement, but it is a notational convenience in the proof of Lemma~\ref{lem:op-4}.}
%and delete the corresponding edge and coordinate arrays.
\item (Flip) if $t=2$, and the two stacks $S_1$ and $S_2$ are the same size, we can switch $S_1$ and $S_2$, so that $S_2$ is the new root.
\end{enumerate}
Note that vectors are inserted and deleted in a ``First in First out'' fashion, hence the term ``stack''.
\begin{figure}
\begin{center}
\includegraphics{proofsketch-1a.pdf}
\end{center}
\caption{Operation on configuration}
\end{figure}

In the node insertion and deletions, we also insert and delete, respectively, coordinate arrays from the configuration.
A significant challenge is specifying how to insert and delete these coordinate arrays.
At a high level, we associate with each configuration a star graph having vertices $S_1,\dots,S_t$ and edges $S_1S_i$ for $i=2,\dots,t$.
We attach coordinate arrays to each edge, and coordinate arrays are inserted and deleted together with their corresponding edge (note: the coordinate arrays attached to an edge may not be labeled by the endpoints of that edge. e.g., a coordinate array constraining $S_i$ and $S_2$ could be attached to edge $S_1S_i$).
%For clarity, we emphasize there are now two types of graphs: the Diameter instance, whose vertices are configurations, and the star graphs in configurations, who nodes are stacks.


%With the node insertion/deletion and flip operations, the indices of the stacks change, so one needs to carefully to relabel the coordinate arrays so that they still constrain the same stack(s) (for example, in the flip, we swap $X_{2,j}$ with $X_{1,j}$).
%In practice, we avoid this relabelling by assigning separate, non-index labels to the stacks, that do not change with an operation, and index the coordinate arrays by these separate labels.

%\TODO{Need to specify how coordinate arrays are deleted and inserted with node insertions/deletions, }

A \emph{(full) operation} consists of two half-operations: a vector insertion or node insertion followed by a vector deletion or node deletion.
We also allow operations to include a flip operation in-between or after the half-operations.
To ensure there are only $\tilde O(n_{OV}^{k-1})$ edges, we do not allow operations between two configurations with one stack ($t=1$).
An operation is \emph{valid} if the starting and ending configuration are valid.
(We also require validity of intermediate configurations resulting from one of the two half-operations. In the Yes case, this gives the extra +1 in proving the diameter is $2k-1$, rather than $2k-2$).

The edges of the Diameter instance go between edges $H$ and $H'$ such that $H'$ can be obtained by applying a valid operation to $H$.

\subsection{Correctness}

\paragraph{Basic properties}
We check a few basic properties of the construction.
\begin{itemize}
\item Operations leave the size (number of stacks plus number of vectors) of a configuration invariant.
The graph vertices are all valid configurations of size $k$, applying any valid operation to a vertex gives the configuration of another vertex, so the edges are well-defined.
\item Since the Diameter instance deals with size $k$ configurations, each configuration has at most $k-1$ vectors, so there are at most $O(n_{OV}^{k-1}d^{O_k(1)})$ vertices. Similarly, one can check that there are $O(n_{OV}^{k-1}d^{O_k(1)})$ edges, and that the graph can be constructed in $O(n_{OV}^{k-1}d^{O_k(1)})$ time.
\item We can also check that (at least under these informal definitions) operations are invertible. A vector insertion inverts a vector deletion, and a node insertion inverts a node deletion, and two flips leave the configuration unchanged.
Hence, for example, a vector insertion/node deletion can be inverted by a node insertion/vector deletion.
Thus, the graph is undirected.
\end{itemize}

\paragraph{No case}
We sketch the proof that, when any $k$ vectors are orthogonal, any two valid configurations of size $k$ are at distance $k$.
We can easily reach any configuration $H'$ from any other configuration $H$ with $k$ not-necessarily-valid operations: 
insert the nodes and vectors of $H'$ while deleting the vectors and nodes from $H$.
We need $k$ deletions to remove $H$ (because it has size $k$), and $k$ insertions to build $H'$, so we pair the insertions and deletions to get from $H$ to $H'$ in $k$ full operations.

In the real proof, these operations may not all be valid, so the order in which we apply the insertions and deletions must be carefully chosen.
%The root stack and its requirement to have $(k-2)/2$ vectors, play a key role here.
The root stack plays a key role in choosing the path.
Let $S_1$ and $S_1'$ be the root stacks of $H$ and $H'$.
Because $S_1$ and $S_1'$ each have at least $(k-2)/2$ vectors (by definition), it is possible to choose a path from $H$ to $H'$ that first deletes all the non-root stacks of $H$ while only adding stack $S_1'$ and its vectors.
Then when $S_1'$ and $S_1$ have the same number of vectors, we apply a flip operation, so that $S_1'$ is the new root, and we build the remainder of $H'$ while deleting stack $S_1$.
\TODO{Picture, just $H$, $H_{mid}$, $H_{mid}'$ and $H'$.}

This path is chosen to avoid conflicts with ``auxiliary'' coordinate arrays.
As we delete $H$ and insert $H'$, we introduce auxiliary coordinate arrays that are not a part of configurations $H$ or $H'$ but are inserted during a node insertion, and we need to delete these coordinate arrays before we reach the final configuration $H$.
The above path ensures that \emph{all} of the auxiliary coordinate arrays are attached to the edge (of the star graph) between stacks $S_1$ and $S_1'$, so the coordinate arrays are only inserted at the first step of the path (when stack $S_1'$ is inserted), and they are all deleted after the last step of the path (when stack $S_1$ is deleted).

Orthogonality is used in choosing auxiliary coordinate arrays. Orthogonality, together with Lemma~\ref{lem:stack-2} ensures we can choose auxiliary coordinate arrays that make a valid path.

%Some of the coordinate arrays of $H$ may not be satisfied by stacks of $H'$, and vice-versa.
%As we delete $H$ and insert $H'$, we introduce ``auxiliary'' coordinate arrays, that are not a part of $H'$ but are inserted (and later deleted) during a node insertion. 
%Lemma~\ref{lem:stack-2} guarantees that such coordinate arrays can be chosen to be appropriately satisfied by stacks.
%every time we insert a node of $H'$ and need to add an ``auxiliary'' coordinate array that is not part of $H'$, we can always choose a coordinate array that is satisfied in the relevant configurations.
%the only coordinate arrays that can constrain stacks from both $H$ and $H'$ are auxiliary coordinate arrays that are added. \TODO{Picture, orange?}
%Furthermore, 
%The real proof carefully chooses a path such that only auxiliary coordinate





\paragraph{Yes case}
We also show that, if there are $k$ orthogonal vectors, then the diameter is at least $2k-1$.
Here, we outline how to prove the diameter is at least $2k-2$, and an extra $+1$ is gained in the real proof using a stronger definition of valid operation.

Suppose that there are $k$ orthogonal vectors $a_1,\dots,a_k$.
Let $H_0$ be the configuration with one stack $S_1=(a_1,\dots,a_{k-1})$, and let $H_{2k-3}$ be the configuration with one stack $S_1'=(a_k,\dots,a_2)$.
%Our proof shows that there are no paths of length $2k-3$ between $H_0$ and $H_{2k-3}$.
Suppose for contradiction there is a path $H_0,H_1,\dots,H_{2k-3}$ consisting of full operations.
%If stack $S_1$ is never deleted, then the path deletes all vectors of $S_1$ and then inserts all vectors of $S_1'$, using $2k-2$ operations, which is a contradiction.
%Thus we assume $i < 2k-2$ and $j<$<++>
%First if $i=2k-2$ and $j=0$, i.e., the stack $S_1$ never gets deleted and just becomes $S_1'$, then we must first use $k-1$ vector deletions to $S_1$ to get the empty stack, and then $k-1$ vector insertions to build $S_1'$. Since full operations always apply the ``insertion'' half-operation before the ``deletion'' half-operation, these insertions and deletions are part of different half operations, so we must have at least $2k-2$ full operations, so the path must have length at least $2k-2$, contradiction.but


The key is to find a coordinate array $x$ that appears in some configurations $H_i,H_{i+1}\dots,H_{i+k-1}$ such that in $H_i$, what is remains in stack $S_1$ satisfies $x$, and in $H_{i+k-1}$, what has been added to stack $S_1'$ also satisfies $x$.
Then, in $H_i$, stack $S_1$ must have a prefix of $(a_1,\dots,a_{k-i-1})$, which thus satisfies $x$ (since at most $i$ deletions were applied to $(a_1,\dots,a_{k-1})$).
In $H_{i+k-1}$, stack $S_1'$ must have a prefix of $(a_k,\dots,a_{k-i})$, which also satisfies $x$ (since applying at most $(2k-3)-(i+k-1)$ insertions gives $(a_k,\dots,a_2)$).
Hence stacks $(a_1,\dots,a_{k-i-1})$ and $(a_k,\dots,a_{k-i})$ satisfy a common coordinate array, contradicting Lemma~\ref{lem:yes-1}.

Finding such a coordinate array $x$ involves several cases, and we describe an illustrative case here.
Let $i$ be the smallest index such that configurations $H_i,H_{i+1},\dots,H_{2k-3}$ all ``contain'' stack $S_1'$.
It is easy to check that $i\le k-2$ so $H_i$ also contains stack $S_1$.
Here, consider the case where $S_1$ and $S_1'$ are adjacent in the configuration's star graph.
%(The case where $S_1=S_1'$ is easy, and the nonadjacent case is deferred to the main proof).
%Let $H_i'$ be the configuration $H_i$ with node $S_1'$ deleted.
%Then $S_1'$ is an empty stack in $H_i$, so $H_i'$ has size $k-1$.
Since the star graph is a tree, and valid operations can only delete leaf nodes, stack $S_1$ can only be deleted by deleting all of $H_i$ minus stack $S_1$, which takes $k-1$ operations (see Lemma~\ref{lem:yes-3}).
Thus, configurations $H_i,\dots,H_{i+k-1}$ all contain stacks $S_1$ and $S_1'$ and the edge between them.
That edge contains a coordinate array that must be satisfied by $S_1$ and $S_1'$ in each of $H_i,\dots,H_{i+k-1}$, as desired.

%The other case, where $S_1$ and $S_1'$ are nonadjacent, is handled in the main proof.
%
%Let $i$ be the largest index such that configuration $H_i$ ``contains'' stack $S_1$, and $j$ be the smallest index such that configuration $H_j$ ``contains'' stack $S_1'$. Since $S_1$ and $S_1'$ start with $k-1$ vectors, we have $j \le k-2 < k-1 \le i$.



\paragraph{Technical challenges}
We now highlight two important issues that our construction avoids. 
These two issues were very helpful in discovering the final construction.
\begin{enumerate}
\item (Don't drop the bottom vector) 
\item (
\end{enumerate}

\TODO{Highlight the ``not drop bottom vector'' subtlety and the $k/2$ all 1s subtelty. 
``We highlight two basic sanity checks that were helpful in coming up with this construction''}



%Since one needs $k$ deletion operations ($k-1$ vector deletions followed by 1 node deletion) to delete stack $S_1$, we have $k-1\le i$, and since one needs $k$ insertion operations to build stack $S_1'$, we have $j\le k-1$, so $j\le i$.



%\TODO{Tree implies $j-i\ge k-1$.}





 



%\subsection{The vectors in a configuration}
%\label{ssec:proofsketch-1}
%The reduction graph $G$ has the property that, for any two vertices $v$ and $v'$ identified by vectors $a_1,\dots,a_s$ and $a_1',\dots,a_{s'}'$, respectively, for $s,s'\le k-1$, (and possibly some coordinates), if any subset of $k$ vectors from $a_1,\dots,a_s,a_1',\dots,a_{s'}'$ are not orthogonal (No case), then vertices $v$ and $v'$ are at distance at most $k$.
%Furthermore, in the Yes case, if $a_1,\dots,a_k$ are $k$ orthogonal vectors, then the endpoint vertices $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ should be at distance $2k-1$.
%Already, these requirements impose the following structure on the construction:
%
%\paragraph{In the Yes case, a path of length at most $k-2$ from endpoint vertex $(a_1,\dots,a_{k-1})$ should not drop vector $a_1$.}
%That is, after taking $k-2$ edges from the endpoint vertex $v=(a_1,\dots,a_{k-1})$, one cannot arrive at a configuration $u=(b_1,\dots,b_s, \bar x)$ of vectors $b_1,\dots,b_s$ and coordinates $\bar x$ where $a_1$ is not among vectors $b_1,\dots,b_s$.
%Suppose not for contradiction, and suppose $a_1,a_2,\dots,a_k$ form the orthogonal $k$-tuple in the Yes case.
%If all of the ``new'' vectors added are the all ones vector $\mathbf{1}$, then the vectors $\{b_1,\dots,b_s\}$ contain only vectors from $(a_2,\dots,a_{k-1},\mathbf{1})$.
%Then among $b_1,\dots,b_s, a_k,a_{k-1},\dots,a_2,\mathbf{1}$, any $k$ vectors are orthogonal, so vertex $(b_1,\dots,b_s,\bar x)$ should be distance at most $k$ from endpoint vertex $v'=(a_k,\dots,a_2)$ by our requirement for the No case.
%Hence, if $d(v,u)\le k-2$, then by the triangle inequality, we have $d(v,v')\le d(v,u)+d(u,v')\le 2k-2$, which contradicts our large diameter requirement for the Yes case.
%
%For the same reason, a path of length at most $k-2$ from endpoint vertex $(a_k,\dots,a_2)$ should not drop vector $a_k$.
%This idea leads to our next idea.
%
%\paragraph{Using ``stacks''}
%Here, stacks refer to the ``first-in-last-out'' data structure.
%We identify a configuration by several ``stacks'' $S_1,\dots,S_t$, where each stack $S_i$ is simply a tuple of a nonnegative number of vectors of $A$ (the configuration may also be identified by some coordinates).
%The endpoint vertices of the Diameter instance are configurations with a single stack of size $k-1$.
%We think of these tuples of vectors as ``stacks'' so that operations consist of popping a vector from one stack and pushing a vector onto another stack.
%In particular, an operation can only touch the ``top'' vector of any given stack.
%This ensures that in the Yes case, for the endpoint vertices with stacks $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$, it takes $k-1$ operations to delete the vectors $a_1$ and $a_k$ from their respective stacks, because each operation can remove at most one vector from the top of the stack.
%We point out that our constructions for $k=4$ and $k=5$ are written in this stack language.
%
%\paragraph{More than two stacks}
%For $k=4$ and $k=5$, it suffices to construct our Diameter instance with vertices that are configurations with at most two stacks, but for general $k$, more stacks seem necessary: if $k$ is large, and there were two configurations $H$ and $H'$ each with two stacks $S_1,S_2$ and $S_1',S_2'$ each of size roughly $k/2$, if one is constrained to only having two stacks, one needs around $3k/2$ vector insertion+vector deletion operations to reach configuration $S_1',S_2'$ from $S_1,S_2$, which is too much in the No case.
%
%\paragraph{A general operation} (Definition~\ref{def:op})
%For general $k$, to accommodate for more than two stacks, we define operations (edges of the Diameter instance) as follows.
%Operations on configurations consist of one ``insertion'' \emph{half-operation} and one ``deletion'' half-operation.
%An insertion half-operation either pushes a vector onto some stack or creates a new empty stack (along with some coordinates), and a deletion half-operation either deletes (pops) a vector from some stack or deletes an empty stack.\footnote{For technical reasons, in the final construction, we require that operations that do the insertion half-operation before the deletion half-operation, which contrasts with the $k=4$ and $k=5$ case where the deletions are done first. Roughly, this change saves a +1 in the Yes case.}\footnote{Also for technical reasons, in specific cases of the general $k$ construction, we also allow a operation to perform a ``flip'' operation between the insertion and deletion, which changes some of the ``meta-data'' of a configuration.}
%
%Conveniently, \emph{all} edges of our generalized construction can be described by such operations.
%In the $k=4$ and $k=5$ case, the edges that apply a vector insertion followed by a vector deletion cover all of the edges in the graph, except for (1) the edges from endpoint vertices with one stack to internal vertices with two stacks, and (2) the edges that change the coordinates (``coordinate change edges'').
%However, for our general $k$ construction, we do not use the coordinate change edges from (2) (intuition for why is given below), this generalized definition of an operation now includes edges from (1): for example, in the $k=4$ case, the edge from $(a,b,c)\in A^3$ to $(\{(a,b),()\},x,y)\in A^2\times ([\mathbb{d}]^3)^2$ can be seen as the operation of inserting an empty stack $()$ and coordinates $x$ and $y$, and then deleting the vector $c$ from the top of the stack $(a,b,c)$.
%Furthermore, these operations are invertible (e.g., a vector insertion plus stack deletion can be inverted by applying a stack insertion plus a vector deletion), so our Diameter instance is indeed undirected.
%
%
%\paragraph{Size: how big are configurations?} (Definition~\ref{def:size})
%We also need to specify how many vectors (and stacks) we can have in a configuration.
%We note that the total number of vectors plus the total number of stacks is invariant under our defined operations: each ``insertion'' (of a vector or a stack) increases this quantity by 1, and each ``deletion'' (of a vector or a stack) decreases this quantity by 1.
%Accordingly, we give this quantity a special name, calling it the \emph{size} of a configuration. 
%The endpoint vertices have 1 stack and $k-1$ vectors, so the size of configurations at endpoint vertices is $k$.
%Since operations preserve size, we therefore require that all configurations (vertices) in our Diameter instance have size $k$.
%The size definition also has the property that, if we ignore coordinates, it is always possible to reach one size $k$ configuration from any other size $k$ configuration with $k$ operations, giving us hope that we can achieve Diameter $k$ in the No case.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%\subsection{The coordinates in a configuration}
%\label{ssec:proofsketch-2}
%We have specified the structure of vectors in the configurations, namely, that we place them in first-in-last-out stacks so that the total size (number of stacks plus number of vectors in stacks) is $k$, and operations push and pop vectors from stacks and add and delete empty stacks.
%Now, we need to specify the coordinates in the configurations.
%In particular, we need to specify how the operations change the coordinates, and which coordinates constrain (need to be satisfied by) which stacks.
%
%As argued above, we expect that for general $k$, our configurations need more than two stacks, and the main challenge that remains is specifying how the coordinates in configurations constrain the vectors in those stacks.
%The constraints must be strong enough that in the Yes case, the 1-stack configurations $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ are not too close, but loose enough that any two configurations can reach each other in $k$ steps in the No case.
%Conveniently for our construction, we only need to specify when configurations are valid vertices of our graph: we let an operation give a valid edge as long as the incident configurations are valid.
%We now describe the additional ideas needed to specify the coordinates of configurations, starting with the most concrete ones.
%
%
%\paragraph{Coordinate arrays}
%A key abstraction that was implicit in prior constructions but that we explicitly use is something we call \emph{coordinate arrays}.
%For a $k$-OV instance $A\subset\{0,1\}^{\mathbb{d}}$, a coordinate array is simply an element of $[\mathbb{d}]^{k-1}$ (Definition~\ref{def:coord-1}).
%With this notion, we define what it means for a stack $S=(a_1,\dots,a_{|S|})$ to \emph{satisfy} a coordinate array $x$, which requries the vectors $a_1,\dots,a_{|S|}$ in the stacks have ones in certain coordinates of the array (Definition~\ref{def:coord-2}).
%With these definitions, coordinate arrays become a useful primitive because of the following nice properties, which are helpful for achieving the balance we need between the Yes case having large diameter and the No case having small diameter.
%\begin{enumerate}
%\item (Lemma~\ref{lem:stack-2}, useful for the No case) Let $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$ be stacks with at most $k-1$ vectors such that any $k$ vectors from among $a_1,\dots,a_s,b_1,\dots,b_{s'}$ are orthogonal.
%Then there exists a coordinate array satisfied by both $(a_1,\dots,a_s)$ and $(b_1,\dots,b_{s'})$.
%\item (Lemma~\ref{lem:yes-1}, useful for the Yes case) If $a_1,\dots,a_k$ are orthogonal, and $x$ is a coordinate array, then the stacks $(a_1,\dots,a_j)$ and $(a_k,\dots,a_{j+1})$ cannot satisfy $x$ simultaneously,
%\end{enumerate}
%
%At this point, we have described all of the ideas that are common to our general $k$ construction and the small case constructions for $k=4$ and $k=5$ (Section~\ref{sec:k4} and Appendix~\ref{app:k5}).
%Coordinate arrays are also used as primitives in our simplified proofs for $k=4$ and $k=5$.
%However, because we optimized the presentation of the $k=4$ and $k=5$ constructions for brevity and simplicity and not for generalizability, the ways the coordinate arrays constrain the stacks is slightly different from the way the coordinates constrain the stacks in the general construction.
%The remaining ideas specific are to the general $k$ construction.
%
%
%
%
%\paragraph{No case: Coordinate arrays constrain at most two stacks.} (See Definition~\ref{def:edge} and Table~\ref{tab:edgesatisfying})
%The next two ideas may or may not be necessary but are at least convenient.
%In the No case, for any two configurations $H$ and $H'$, we need to construct a path $H_0=H,H_1,\dots,H_k=H'$ from $H$ to $H'$, such that configuration $H_i$ is obtained by applying some operation to $H_{i-1}$ for all $i=1,\dots,k$.
%Since configurations $H$ and $H'$ have size $k$, in each of the $k$ operations on the path, the insertion operation must add a vector or stack ``belonging to'' $H'$ and the deletion operation must delete a vector or stack ``belonging to'' $H$ (the notion that some configurations ``share'' stacks can be formalized by assigning labels to stacks, see Definition~\ref{def:configuration}).
%Hence, each intermediate configuration $H_i$ contains some stacks and coordinate arrays ``belonging to'' $H$, some stacks and coordinate arrays ``belonging to'' $H'$, and possibly some additional coordinate arrays. 
%However, it is possible that none of the vectors in $H$ have ones in any of the coordinates in $H'$, and vise versa.
%Thus, it is important that for each $H_i$, none of the coordinate arrays ``belonging to'' $H$ constrain any of the stacks ``belonging to'' $H'$, and vise versa.
%This is easiest to guarantee if at most two stacks are ever required to satisfy any coordinate array, and we found this assumption not make the Yes case much harder.
%By similar reasoning, we also have the following idea.
%
%\paragraph{No case: Require every configuration has a stack with at least $\ceil{(k-2)/2}$ vectors.} (Definition~\ref{def:valid})
%Without this constraint, there could be two size-$k$ configurations $H$ and $H'$ with $\Omega(k)$ stacks of $O(1)$ vectors each such that none of the coordinate arrays from $H$ are satisfied by stacks in $H'$ and vise versa.
%In the No case, these two configurations $H$ and $H'$ must be connected by a length $k$ path $H_0=H,H_1,\dots,H_k=H'$.
%Then, the intermediate configuration $H_{k/2}$ must have $\Omega(k)$ stacks from $H$ and also $\Omega(k)$ stacks from $H'$.
%It is easily possible that configuration $H_{k/2}$ has at least one coordinate array for every pair of stacks (in fact, below we show that having only one coordinate array for each pair of stacks is not enough for the Yes case), so we likely have $\Omega(k^2)$ coordinate arrays in $H_{k/2}$ that belong to neither $H$ or $H'$ but constrain some stack in $H$ and another stack in $H'$.
%All $\Omega(k^2)$ must be all inserted and then deleted on the path from $H$ to $H'$, giving a lot of ``extra'' coordinate arrays to keep track of.
%
%Requiring that every configuration has a stack with at least $\ceil{(k-2)/2}$ vectors means that, in the No case, we can find a path $H_0=H,H_1,\dots,H_k=H'$ between two configurations $H$ and $H'$, such that in each intermediate configuration $H_i$, there is either only \emph{one} stack from $H$ or only \emph{one} stack from $H'$, giving only $O(k)$ ``extra'' coordinate arrays to keep track of, an improvement from $\Omega(k^2)$ such coordinate arrays.
%Furthermore, this requirement does not seem to affect the Yes case, and our Yes case proof does not seem to use this assumption.
%
%
%
%
%
%
%
%
%\paragraph{Yes case: No coordinate change edge.}
%In the $k=4$ and $k=5$ constructions in this work, at every vertex, there is an edge that changes \emph{all} the coordinates of an edge, e.g., from $(a,b,x,y)_{L_2}\in A^2\times ([\mathbb{d}]^3)^2$ to $(a,b,x',y')_{L_2}$ in the case of $k=4$.
%However, these ``coordinate-change edges'' cannot exist in the general construction.
%Indeed, if such edges existed, then in the Yes case, configurations $(a_1,\dots,a_{k-1})$ and $(a_k,\dots,a_2)$ would be at distance only $3k/2+O(1)$.
%From $(a_1,\dots,a_{k-1})$, we could (i) reach a configuration with stacks $(a_1,\dots,a_{k/2-O(1)}), (\mathbf{1},\dots,\mathbf{1})$ in roughly $k/2$ operations, (ii) apply a coordinate change edge, (iii) reach a configuration with stacks $(a_k,\dots,a_{k/2+O(1)}),(\mathbf{1},\dots,\mathbf{1})$ in roughly $k/2$ operations, (iv) apply a coordinate change edge, and (v) reach configuration $(a_k,\dots,a_{2})$ in roughly $k/2$ operations.
%Indeed, the coordinate change edges divide the path into three subpaths, and in each subpath we never ``see'' all of the vectors $a_1,\dots,a_k$ in the stacks, so we can choose the coordinate arrays so that the stacks always satisfy the coordinate arrays, hence giving a valid path (we assumed without loss of generality that no $k-1$ vectors are orthogonal).
%Thus, for the Yes case, changing coordinates needs to be more expensive that one edge.
%
%
%
%\paragraph{Yes case: Remembering coordinate arrays (a.k.a. coordinate arrays constraining phantom stacks)} (See comments after Definition~\ref{def:edge})
%One natural (but incorrect) way of implementing the above ideas is, in a configuration with stacks $S_1,\dots,S_t$, have $\binom{t}{2}$ coordinate arrays, $x^{i,j}$ for $1\le i<j\le t$, and require that stacks $S_i$ and $S_j$ satisfy coordinate array $x^{i,j}$.
%Adding an empty stack $S_{t+1}$ to a configuration with $t$ stacks adds $t$ coordinate arrays $x^{i,t+1}$, one for each pair of stacks $(S_i,S_{t+1})$, and deleting a stack $S_{t}$ deletes the $t-1$ coordinate arrays that constrain it.
%This construction does not work, because in the Yes case, as in the previous paragraph, it is again possible for the 1-stack configuration $(a_1,\dots,a_{k-1})$ to reach the 1-stack configuration $(a_k,\dots,a_2)$ in $3k/2+O(1)$ steps, by passing through the two stack configurations with stacks $(a_1,\dots,a_{k/2-O(1)}), (\mathbf{1},\dots,\mathbf{1})$ and $(a_k,\dots,a_{k/2+O(1)}),(\mathbf{1},\dots,\mathbf{1})$.
%
%To work around this problem we have configurations $H$ ``remember'' some coordinate arrays that constrain deleted stacks.
%That is, if an operation on configuration $H$ deletes a stack $S$ to obtain configuration $H'$, some of the coordinate arrays of $H$ that $S$ needed to satisfy are still coordinate arrays of configuration $H'$.
%In this way, some coordinate arrays of a configuration constrain two stacks and other coordinate arrays only constrain one stack (such coordinate arrays can be thought of as constraining a real stack and a ``phantom'' stack).
%This works, but one needs to be careful in how many coordinate arrays are ``remembered'', or else the No case might have large diameter.
%
%\paragraph{Balancing the No case and Yes case: a tree and an ordering $\prec_H$ on the stacks.} (Definition~\ref{def:configuration})
%The Yes case, particularly the $3k/2+O(1)$-path counterexample, encourages us to remember more constraints, but having Diameter $k$ in the No case keeps us from remembering too many constraints.
%In the final construction, to help with this balance, we add two additional structures to configurations: 
%\begin{enumerate}
%\item Put an ordering $\prec_H$ on the stacks of a configuration $H$, so that we have a list of stacks, rather than simply a set of stacks.
%Whether a stack is constrained by a certain coordinate array then depends on the location of the stack in the ordering. 
%
%\item We place the stacks $S_1,\dots,S_t$ of a configuration $H$ at the vertices of a tree on $t$ vertices (in particular, a star graph on $t$ vertices). Coordinate arrays are attached to the edges of the tree so that a coordinate array is added to (deleted from) the configuration exactly when the corresponding edge is added to (deleted from) the configuration.
%For clarity, we emphasize that there are now two types of graphs: the tree graphs $H$ that define a configuration, and the Diameter instance $G$, whose vertices are configurations $H$.
%
%With this tree, we remember some, but not too many, coordinate arrays that constrained deleted vertices (Lemma~\ref{lem:yes-3}).
%In particular, for an edge connecting stacks $S_i$ and $S_j$, we keep track of the coordinate arrays that constrain $S_i$ and some other (possibly non-existent) stack, and also the coordinate arrays that constrain $S_j$ and some other (possibly non-existent) stack.
%Somewhat subtly, the coordinate arrays attached to an edge may constrain stacks not incident to the edge.
%For the coordinate arrays constraining $S_i$, whether the coordinate arrays constrain another real stack or a non-existent stack depends on the ordering $\prec_H$.
%\end{enumerate}
%












